Adversarial Domain Adaptation for Metal Cutting Sound Detection: Leveraging Abundant Lab Data for Scarce Industry Data

Cutting state monitoring in the milling process is crucial for improving manufacturing efficiency and tool life. Cutting sound detection using machine learning (ML) models, inspired by experienced machinists, can be employed as a cost-effective and non-intrusive monitoring method in a complex manufacturing environment. However, labeling industry data for training is costly and time-consuming. Moreover, industry data is often scarce. In this study, we propose a novel adversarial domain adaptation (DA) approach to leverage abundant lab data to learn from scarce industry data, both labeled, for training a cutting-sound detection model. Rather than adapting the features from separate domains directly, we project them first into two separate latent spaces that jointly work as the feature space for learning domain-independent representations. We also analyze two different mechanisms for adversarial learning where the discriminator works as an adversary and a critic in separate settings, enabling our model to learn expressive domain-invariant and domain-ingrained features, respectively. We collected cutting sound data from multiple sensors in different locations, prepared datasets from lab and industry domain, and evaluated our learning models on them. Experiments showed that our models outperformed the multi-layer perceptron based vanilla domain adaptation models in labeling tasks on the curated datasets, achieving near 92%, 82% and 85% accuracy respectively for three different sensors installed in industry settings.

==> Results.tex <==
\begin{document}

\begin{tabular}{|c|c|c|c|c|c|c|c|}
 & Source Labeled Data Size & Target Labeled Data Size & Target Test Accuracy Mean VanillaBaselineSingleModel & Target Test Accuracy Mean VanillaBaselineMultiModel & Target Test Accuracy Mean VanillaBaselineFineTunedModel & Target Test Accuracy Mean ICIT-ADV-DA & Target Test Accuracy Mean modified-ICIT-ADV-DA \\
0 & 2000 & 50 & 0.459 & 0.446 & 0.513 & 0.773 & \font-weightbold 0.791 \\
1 & 2000 & 200 & 0.439 & 0.440 & 0.448 & 0.865 & \font-weightbold 0.867 \\
2 & 2000 & 500 & 0.447 & 0.458 & 0.501 & \font-weightbold 0.881 & 0.874 \\
3 & 2000 & 1000 & 0.452 & 0.524 & 0.545 & \font-weightbold 0.889 & 0.851 \\
4 & 2000 & 4000 & 0.451 & 0.501 & 0.565 & \font-weightbold 0.913 & 0.890 \\
5 & 2000 & 10000 & 0.453 & 0.563 & 0.563 & \font-weightbold 0.930 & 0.913 \\
6 & 2000 & 16000 & 0.455 & 0.563 & 0.563 & \font-weightbold 0.925 & 0.916 \\
7 & 5000 & 50 & 0.488 & 0.428 & 0.476 & \font-weightbold 0.805 & 0.784 \\
8 & 5000 & 200 & 0.420 & 0.452 & 0.470 & 0.856 & \font-weightbold 0.876 \\
9 & 5000 & 500 & 0.503 & 0.430 & 0.491 & 0.876 & \font-weightbold 0.884 \\
10 & 5000 & 1000 & 0.492 & 0.452 & 0.563 & 0.892 & \font-weightbold 0.897 \\
11 & 5000 & 4000 & 0.445 & 0.502 & 0.563 & 0.906 & \font-weightbold 0.911 \\
12 & 5000 & 10000 & 0.474 & 0.537 & 0.563 & \font-weightbold 0.928 & 0.916 \\
13 & 5000 & 16000 & 0.499 & 0.498 & 0.563 & \font-weightbold 0.930 & 0.913 \\
14 & 8000 & 50 & 0.445 & 0.407 & 0.461 & 0.788 & \font-weightbold 0.798 \\
15 & 8000 & 200 & 0.442 & 0.461 & 0.461 & 0.851 & \font-weightbold 0.874 \\
16 & 8000 & 500 & 0.452 & 0.480 & 0.497 & 0.871 & \font-weightbold 0.892 \\
17 & 8000 & 1000 & 0.418 & 0.441 & 0.563 & \font-weightbold 0.900 & 0.898 \\
18 & 8000 & 4000 & 0.442 & 0.478 & 0.565 & \font-weightbold 0.924 & 0.912 \\
19 & 8000 & 10000 & 0.447 & 0.497 & 0.563 & \font-weightbold 0.930 & 0.916 \\
20 & 8000 & 16000 & 0.434 & 0.537 & 0.563 & \font-weightbold 0.925 & 0.919 \\
21 & 10000 & 50 & 0.432 & 0.435 & 0.445 & 0.788 & \font-weightbold 0.799 \\
22 & 10000 & 200 & 0.475 & 0.477 & 0.444 & 0.840 & \font-weightbold 0.874 \\
23 & 10000 & 500 & 0.497 & 0.457 & 0.521 & 0.868 & \font-weightbold 0.887 \\
24 & 10000 & 1000 & 0.434 & 0.445 & 0.563 & \font-weightbold 0.901 & \font-weightbold 0.901 \\
25 & 10000 & 4000 & 0.482 & 0.505 & 0.563 & 0.888 & \font-weightbold 0.920 \\
26 & 10000 & 10000 & 0.436 & 0.478 & 0.563 & 0.905 & \font-weightbold 0.924 \\
27 & 10000 & 16000 & 0.450 & 0.516 & 0.563 & 0.904 & \font-weightbold 0.919 \\
28 & 16000 & 50 & 0.450 & 0.418 & 0.505 & 0.797 & \font-weightbold 0.798 \\
29 & 16000 & 200 & 0.448 & 0.490 & 0.486 & \font-weightbold 0.876 & 0.874 \\
30 & 16000 & 500 & 0.437 & 0.442 & 0.519 & 0.879 & \font-weightbold 0.893 \\
31 & 16000 & 1000 & 0.435 & 0.448 & 0.563 & 0.897 & \font-weightbold 0.899 \\
32 & 16000 & 4000 & 0.439 & 0.457 & 0.565 & 0.914 & \font-weightbold 0.916 \\
33 & 16000 & 10000 & 0.448 & 0.519 & 0.563 & 0.912 & \font-weightbold 0.922 \\
34 & 16000 & 16000 & 0.443 & 0.521 & 0.565 & 0.901 & \font-weightbold 0.913 \\
\end{tabular}
\end{document}


==> draft_dataset_preparation.tex <==
\section{Dataset Preparation} \label{sec:datprep}
For both the \imi{} and \kirby{} datasets, we collected separate sound files of cutting processes. Each sound file ranges from 1 minute to 6.5 minute in length and has several time intervals where the machine cutting sounds are heard. \imi{} and \kirby{} have, respectively, 18 and 1 sound files for each sensor, with a total duration of 2789.97 \& 130.27 seconds respectively. Each sound file was sampled with 48 kHz rate, with the help of the Librosa~\cite{mcfee2015librosa} library. After that, these samples were transformed into Fourier domain using Fast Fourier Transformation (FFT)~\cite{nussbaumer1982fast}, with frequency windows set to $\mathit{n_{fft} = 2048}$, in Librosa \cite{mcfee2015librosa}. FFT returns $\mathit{1 + \frac{n_{fft}}{2}}$ frequency beans, hence each sample has $1 + \frac{2048}{2} = 1025$ frequency beans. Each frequency bean value was squared to get the intensity value, and then they converted to Decibels (dB). So, per data sample has 1025 intensities as features. The number of samples in Librosa \cite{mcfee2015librosa} conversion is defined as $\frac{4 \times \text{sampling rate} \times \text{time} }{n_{fft}}$, hence there are $\frac{4 \times 48000 \times 2789.97}{2048} \approx $ 261560 samples in \imi{} and $\frac{4 \times 48000 \times 130.27}{2048} \approx $ 12213 samples in \kirby{}, per sensor. Also, per sensor, the number of cut (non-cut) sample frames are- for \imi{}, 97312 (164248) and for \kirby{}, 5405 (6805).

==> draft_experiment.tex <==
\section{Experiments} \label{sec:exp}

\subsection{Experiment settings}
We implemented all our models using 
Tensorflow~\cite{tensorflow2015-whitepaper}, and Librosa~\cite{mcfee2015librosa}. The models were run on an NVIDIA GeForce RTX 3090 GPU with Cuda 12.2 support. For experiments, we randomly split our datasets in (70-10-20)\% ratio for train, validation, and test set for each sensor. 
\subsection{RQ1 Experiment}
%The motivation behind our RQ1 experiment is to find out whether we need to perform any transformation on the source and target domain data before passing them to the model. Our hypothesis is: as the source and target domain feature distributions are different, if a prior-transformation can improve the single domain classification (same source and domain) performance without the introduction of more deep layers to capture the domain invariant and dependent features, then we can use these transformed features as direct input to the transfer learning task, rather than using the original features as the direct input, which would then require introducing more deep layers. This would help us to learn the smaller number of parameters to perform the transfer learning task optimally. 
The motivation behind our RQ1 experiment is to determine if we need to transform the source and target domain data before passing them to the model. Our hypothesis is that the feature distributions of the source and target domains differ. If a prior transformation can improve single-domain classification performance without adding more deep layers, we can use these transformed features directly for transfer learning. This approach helps us avoid introducing more layers, thus learning fewer parameters and optimizing the transfer learning process.
For this, we introduce a simple binary classification model comprising of a \textbf{MLP} with a single hidden dense layer with 512 neurons. We use sigmoid and softmax as the activation functions in the hidden and output layers respectively. We ran the model for 20 epochs, with the batch size set as 128. We also used the same splits as before, and reported our results on the validation set instead of the test set, as the validation set results reflect more on the model’s generalizablity. Better accuracy in validation ensures that these transformations will also work better for transfer learning task. We loaded all \imi{} data and ran the model. The model was simpler and hence it did not take much memory, thereby we could load the whole data in memory. The evaluated transformations are: (i) Identity ($idx$), (ii) Standardization ($stanx$), (iii) Log ($logx$), (iv) Sigmoid ($sigmoidx$) and, (v) Gamma ($gammax$). In the second column of \Cref{tab:rq1_merged2}, we have described the transformation formulas for the feature value $x$.  
%\begin{align}idx(x) = x\end{align} 
%\begin{align}stanx(x) = \frac{x-\min(x)}{\max(x)-\min(x)}\end{align} \begin{align}logx(x) = 255(\frac{\log{(81+x)}}{\log{(81+\max{(x)})}})
%\end{align} 
%\begin{align}sigmoid(x) = 255(\frac{e^{x+41}}{1+ e^{x+41}})
%\end{align} 
%\begin{align}gammax(x) = 255(\frac{81+x}{81+\max{(x)}})^\gamma\end{align} where $\gamma$ is an arbitrary constant.

%\input{tables/RQ1_result_merged}
%\mir{FIX PERCENTAGE, AND TABLE}

%\eunseob{Use percentage unit for RQ1 table.}
%\noindent(i) Identity: $idx(x) = x$ \noindent(ii) Standardization: $standardx(x) = \frac{x - \text{min}(x)}{\text{max}(x) - \text{min}(x)}$ \noindent(iii) Log: $logx(x) = 255(\frac{\text{log}(81 + x)}{\text{log}(81 + \text{max}(x)})$ \noindent(iv) Sigmoid: $sigmoid(x) = 255(\frac{e^{x + 41}}{1 + e^{x + 41}})$ \noindent(v) Gamma: $gamma(x) = 255(\frac{81 + x}{81 + \text{max}(x)})^{\gamma}$

%\noindent(i) Identity: \begin{align}idx(x) = x\end{align} (ii) Standardization: \begin{align}stanx(x) = \frac{x-\min(x)}{\max(x)-\min(x)}\end{align}(iii) Log: \begin{align}logx(x) = 255(\frac{\log{(81+x)}}{\log{(81+\max{(x)})}})\end{align} (iv) Sigmoid: \begin{align}sigmoid(x) = 255(\frac{e^{x+41}}{1+ e^{x+41}})\end{align} (v) Gamma: \begin{align}gammax(x) = 255(\frac{81+x}{81+\max{(x)}})^\gamma\end{align} where $\gamma$ is an arbitrary constant. 
From \Cref{tab:rq1_merged2}, we can see that for all sensors of both datasets, $gammax$ transformation outperforms all others in validation accuracy, thus being the representation with the greater generalization ability. $stanx$ has the best performance for training accuracy in \imi{} ($gammax$ is not very far). Overall, $gammax$ with $\gamma=4.2$ proves to be the best choice for data pre-processing transformation. 
%\textbf{We used this transformation before running the models for the next experiments}.
\textbf{In RQ2 experiments, models are trained on Gamma-transformed features}.
\input{tables/RQ1_result_merged_2}
%\adrian{To further save the space, we can skip the train accuracy in both tables and merge table 2 and 3 as one table.}
%\eunseob{Done.}

%\input{tables/RQ1_results} \eunseob{I will merge two table (II and III)}

\input{tables/RQ2_imi_sensor_0_reduced}

\subsection{RQ2 Experiment}
%\eunseob{I will be updating the RQ2 table}
In this experiment, we compared our adversarial DA models with baseline models, for classifying unlabeled target data by learning on large labeled source domain data and small labeled target domain data. We ran experiments on nine combinations: from all three sensors of the source domain (\imi{}) to all three sensors of domain (\kirby{}). We compared five models: three vanilla baselines (single, multi and fine-tuned), and two adversarial DA models (\icit{}, \icitmod{}). For brevity, we refer to the \textbf{Vanilla} \textbf{B}aseline \textbf{S}ingle, \textbf{M}ulti and \textbf{F}ine Tuned \textbf{M}odels respectively as \vbs{}, \vbm{} and \vbf{}. For space constraint, we only report the results of three combinations- \imi{} sensor 0 to all \kirby{} sensors.

All the vanilla baselines are \textbf{MLP}s with two hidden layers of 512 and 200 nodes. Both of these have ReLU as activation, and dropout layers with $p=0.2$. In final layer, Softmax is applied. The difference among them is in how they are trained: \vbs{} is trained and validated with source domain data; \vbm{} is trained and validated with both source and target domain data; and finally, \vbf{} is at first trained and validated on source domain data, and later, the last dense and output layers are fine-tuned with target domain data, while the first dense layer weights remain frozen. For the vanilla baselines, we have used cross-entropy loss with the Adam optimizer \cite{kingma2014adam}, with learning rate 0.001 and $\beta_1 =$ 0.9.

For the \icit{}  and \icitmod{} models, we train and validate on both source and target domain (train and validation split respectively) data, using Adam optimizer~\cite{kingma2014adam} for all components with the same learning rate (=0.0002) and $\beta_1$(=0.5). The values of loss weights $\beta, \gamma$, and $\lambda$ are all set to 1 after trial and error over different ranges.   
%\eunseob{Normally in academic writing, don't use "please".}
Batch size and learning epoch were set to 128 and 20, respectively. Moreover, for \icit{} \& \icitmod{}, in each epoch, we iterated over the entire training data for both domains at least once. 
%Thus for one entire training of the source domain, the target domain data was used multiple times. In each epoch, we calculated the number of steps to iterate over entire source domain data, and 
In each epoch, after a fixed number of batch steps (=40) iteratively, we performed validation and saved the model with best target validation accuracy. We iterated over the pairing of source training data size = 
\{
2000, 
%5000, 
8,000, 
%10000, 
16,000\} 
and target training data size = 
\{50, 
%200, 
500, 
%1000, 
4,000, 
%10000, 
%16,000
12,213\} 
and ran each combination with all models, for three times with fixed seeds, and reported the average accuracy. For the model architectures, refer to the \Cref{sec:mod:arch}. 

%\input{tables/RQ2_imi_sensor_0_all}
%\input{tables/RQ2_imi_sensor_1_all}
%\input{tables/RQ2_imi_sensor_2_all}

%\adrian{I don't think we have space for 2 tables, also the table is quite large. I suggest we just chose one table and trim it down to a few rows with most interesting results. And in the text we can say, we only report partial results with sensor 0 due to space limit, full results on sensor 0 as well as the experiment results with sensor 1 will be provided in the final version. } \eunseob{I agree with that. Table V, VI will be removed and the Table IV will be shortened.}
\Cref{tab:rq2sens0_reduced} shows the performances of the different models, %all three sensor data separately of \imi{} as source and data of sensor $0,1,2$ of \kirby{} respectively, as target. 
from \imi{} sensor 0 to \kirby{} sensors. 
From the results, we can see that: \textbf{(1)} \icit{} and \icitmod{} outperform all the vanilla baseline models by a considerable margin, with accuracy values ranging over $72\%$ at least, whereas even the best accuracy of the vanilla baselines are $56\%$ at most- proving our models' effectiveness; \textbf{(2)} Also, for each data size combination, our models showed their best performances for \kirby{} sensor 0 data - it is to be noted that this was the case for \imi{} sensor 1 and 2 too - which indicates that \kirby{} sensor 0, the very sensor in the closest proximity to the cutting machine, captures the sound information best.
%\endinput
%\eunseob{I'd like to suggest to remove this section below (Demonstration~) due to the page limitation. The result is obvious. We could show this in the presentation or include the following journal paper submission including real-time implementation part.}

%\subsection{Demonstration on a proper-time ordered sound file}
%For the previous experiments, we constructed the sound frames by sampling the sound files on a given rate, and later performing training, validation and testing batches from them after permutations. A question is whether from these permuted sound frames we can reconstruct the prediction for a full sound file. Also, as we ran the experiments for 16000 source and 4000 target sound frames, it remains to see whether we can choose two source sound files (namely Exp1-2 and Exp2-1 from \imi{}) containing around 16000 frames in total, and 4000 sampled frames from \kirby{}, and train on them to predict the cutting-non cut sound for the entire time frame. 
%\elisa{There is a logical disconnection between the previous text and the one below. The reader would expect some sentences talking about the experiments you did to reply to this question.} \eunseob{This subsection will be revised.}
%The results are shown in
%\Cref{fig:demo} shows the results. In the figure, the blue sound wave denotes the real cut (1) - non cut (0) frames, and the red line is the predicted one. We can see that the rate of true positives and negatives are quite high; but the rates of false ones could be reduced by training on more diverse dataset. 
%\begin{figure}[htbp]
%\centerline{\includegraphics[scale=0.6]{images/RQ5.png}}
%\caption{Comparison of ground truth labels and \icitmod{}-inferred labels in a clipped \kirby{} sound file }\label{fig:demo}
%\label{fig}
%\end{figure}


==> draft_industrial_background.tex <==
\section{Industrial Background} \label{sec:indback}


\adrian{The initial submission is up to 6 pages including references and figures. We might need to remove this section and merge it into the introduction.}

Optimizing equipment utilization and enhancing productivity are key factors in improving manufacturing competitiveness. Monitoring machine operations plays a pivotal role in enhancing manufacturing production by providing essential information that improves efficiency on 
factory floors~\cite{bueno2020smart}. Accordingly, manufacturing equipment nowadays features Information and Communication Technology (ICT) and Internet of Things (IoT) capabilities, facilitating data exchange of machine operation and the adoption of Artificial Intelligence (AI) solutions~\cite{maier2017big}. MTConnect which is a CNC machine tool data integration standard provides information of events, samples, and conditions from 
controller~\cite{liu2019cyber}. However, MTConnect does not provides exact cutting times. Additionally, many CNC machines estimate cutting time based on the accumulated cutting motion commands (e.g., G01, G02, G03, etc.) in G-Code, which can be inaccurate because it includes air-cutting. Monitoring the cutting state is also challenging when the machine is manually operated by a machinist. Accurate real-time cutting state monitoring can significantly improve factory floor operations.

On top of that, in situations where many legacy machines are still functioning well and widely used for production in real factory settings, it is crucial to digitize the operational information of these machines, which often lack hardware or software interfaces~\cite{guerreiro2018definition}. However, manufacturing companies, particularly Small and Medium-sized Enterprises (SMEs), are often reluctant to invest significantly in retrofitting these machines to gather operational data. Additionally, many SMEs prefer to maintain their existing manufacturing setup and avoid interrupting production for intrusive equipment monitoring, as this can lead to undesirable downtime and changes in production configurations. While machine sound monitoring could be a viable alternative with advances in ML, it faces challenges such as vulnerability to noise and the lack of solutions for various machines and situations. The high cost and labor-intensive process of labeling and gathering data are significant barriers to its adoption. Therefore, effective DA techniques and the development of more generalized models could greatly impact the adoption of machine sound monitoring in the industry.




==> draft_introduction.tex <==
\section{Introduction}
%\eunseob{I re-organized Intro. However, still it should be more concise by cutting off.}
Machine sound monitoring is a low-cost and non-intrusive method that converts acoustic signals into machine operational information. Manufacturing machines emit sounds that contain ample process information as they operate. However, the intricate interactions between components of manufacturing equipment and the complex nature of vibration and sound propagation make modeling sound emission challenging in the unpredictably noisy environment of a real-world factory floor~\cite{wegener2021noise}. In the metal cutting industry, continuous monitoring of the cutting state is crucial for evaluating process efficiency ~\cite{liu2018real} and estimating cutting tool life \cite{benkedjouh2015health}.
%As an operator understands machine sounds through experience and learning, machine learning (ML) approaches adopting principles from Automatic Speech Recognition (ASR) have been utilized for machine sound monitoring~\cite{kim2021multiple}. In the metal cutting industry, continuous monitoring of the cutting state is crucial for evaluating process efficiency ~\cite{liu2018real} and estimating cutting tool life \cite{benkedjouh2015health}. 
%It is not surprising that experienced machinists can detect cutting sounds by listening, even in noisy environments with various equipment. In wet cutting conditions where visual observation is impossible due to coolant fluid, they can still discern the cutting state by sound. A machinist familiar with a specific Computer Numerical Control (CNC) milling machine can recognize its cutting sounds and quickly adapt to identifying sounds from different machines in new locations. This ability exemplifies the flexible auditory sensing capabilities of human experts in the manufacturing industry.

%Optimizing equipment utilization and enhancing productivity are crucial for manufacturing competitiveness. Monitoring machine operations improves factory efficiency by providing essential data ~\cite{bueno2020smart}. Modern manufacturing equipment incorporates Information and Communication Technology (ICT) and Internet of Things (IoT) capabilities for data exchange and Artificial Intelligence (AI) adoption ~\cite{maier2017big}. However CNC machine tool data integration standard standards such as MTConnect lack precise cutting time information ~\cite{liu2019cyber}. CNC machines often inaccurately estimate cutting time, and manual operation further complicates real-time monitoring. Moreover, legacy machines, still prevalent in production, require digitization, yet SMEs hesitate to invest in retrofitting due to costs and production disruptions. Machine sound monitoring, a potential solution, faces challenges like noise vulnerability and high data labeling costs. Effective domain adaptation techniques and generalized models are needed to advance machine sound monitoring in the industry.

 Machine learning (ML) techniques have been applied to the detection of cutting sounds~\cite{kothuru2018application,chu2022research,peng2021sound,kim2023real-time,kim2023sound}. However, previous detectors have overlooked several critical factors, such as the numerous combinations of operational conditions, including machine type, tool, cutting parameters, and environmental factors. Moreover, the type and placement of sound sensors impact the prediction performance of ML models in machine sound monitoring~\cite{kim2023sound, kim2024operation}. In a controlled laboratory setting, collecting and labeling diverse cutting data for a Computer Numerical Control (CNC) machine tool can be automated~\cite{kim2024online}. However, in a real industrial setting, data collection and labeling are costly and time-consuming. This raises an interesting question: {\em Can lab data be useful for training a model that predicts real-world data?} An ML model simply trained on lab data is typically unable to make accurate predictions on real industry data due to distinct sound emission characteristics between different machines and settings. Therefore, to effectively train the model, it is crucial to consider the different domains created by varying machine types, cutting conditions, and sensor types and placements.

One approach to train an effective ML-based sound detector despite domain differences is through Domain Adaptation (DA)~\cite{ganin2016domain, tzeng2017adversarial, li2023building}. This method typically involves learning a common latent representation from two different domains, referred to as source and target domains. These domains are related but distinct; the source domain has a large training dataset, whereas the target domain has few labeled data obtained from the actual deployment environment of the equipment.
A classifier is then trained using such latent common representation, also referred to as {\em domain-independent representation} or {\em domain-invariant representation}. Because the representation is domain-invariant, the classifier can be ``transferred'' to make predictions in the target domain. For our research problem, the lab data is the labeled source domain and the industrial data is the target domain.
%, where \textbf{all} data are labeled.

In this work, we collected the cutting sound datasets in both lab and industry settings with various sensor types and placements. 
%These datasets were gathered from three sound sensors placed at different locations. The machines in the lab and industrial settings vary in configuration and size. The dataset collected in the lab setting is abundant, while the one collected in the industrial setting is scarce. 
Our work on designing a suitable DA approach to train a cutting detection model for deployment in a real factory floor, answers the following Research  Questions (RQs):

\newlist{researchquestions}{enumerate}{1}
\setlist[researchquestions,1]{
    label=RQ\arabic*),
    left=10pt,
    leftmargin=*,
    labelsep=0.5em,
    listparindent=1em,
    align=left
}

\begin{researchquestions}
    \item Which type of transformation for the sound features improves learning performances?
    \item How good is DA for learning on adequate source and inadequate target labeled data, and performing inference on unlabeled target domain data?
    %\item What is the relation between the sizes of provided source and target labeled training data in terms of accuracy performance?
\end{researchquestions}
To answer the first question, we have experimentally evaluated single domain classification on both lab and industry data for separate sensors, after transforming their features in different ways. 
%We show that, compared with other feature transformations, the Gamma transformation has the best performance on training and validation performance. 
For the second research question, we compare two models: one has been developed by Li et al.~\cite{li2023building} but applied only the image data; the other is a modification of the first approach and our novel contribution. We refer the first model as \icit{} (\icitfull{})- as it fools (``flummoxes'') the adversarial discriminator by adapting through the mixing (``amalgamation'') of separate latent space representations for both domains. We refer to the second model as \icitmod{} (\icitmodfull{})- as in this methodology the generator will receive feedback from the discriminator more as a critic than as an adversary, to ingrain domain identity information in the shared representation space.

In \Cref{sec:relwork}, we provide background about ML-based sound monitoring techniques, and domain adaptation. Later, in \Cref{sec:datcol}, we discuss our process for lab and industry data collection and pre-processing for our DA task, %and how we  preproces them for learning. 
Then, in \Cref{sec:method}, we formulate our research problem, and provide details about \icit{} and \icitmod{}. Finally, in \Cref{sec:exp}, we report the results of our evaluations with respect to our two research questions, by comparing different transformations and domain adaptation models. 
%We also give a demonstration of our model on a short cutting-sound file.




==> draft_methodology.tex <==
\section{Methodology} \label{sec:method}

Our approach is based on the methodology by Li et al.~\cite{li2023building}, which uses DA along with data augmentation for training a target model from minimal and imbalanced training data from two domains (e.g., source and target). This model is able to infer classes for samples from the target domains. We first give our problem statement in \Cref{sec:probstate}, followed by a description of the \icit{} model in \Cref{sec:icit}, and our new approach \icitmod{} in \Cref{sec:icitmod}.

\subsection{Problem Statement} \label{sec:probstate}
%\adrian{This section can be reduced. For example, we don't need to state the research problems in three ways. We can just keep the use case one and maybe the math one.}
\textbf{In words}, our research problem can be stated as follows: 
\vspace{0.5\baselineskip}

\emph{``Given a large labeled dataset from a source domain, and a way smaller labeled dataset from a target domain, can we train a model which can classify samples
%an unlabeled dataset 
from the target domain, by learning domain dependent and domain independent features from source and target domains?''}\\
%\vspace{0.5\baselineskip}

Formally, {let $\mathcal{D}_s = \{(\mathbf{x}_s^{(i)}, y_s^{(i)})\}_{i=1}^{n_s}$, be a labeled dataset of size $n_s$, where sample data $\mathbf{x}_s^{(i)} \in \mathbf{S}$ -- the source domain. Also, let another labelled dataset be $\mathcal{D}_t= \{(\mathbf{x}_t^{(i)}, y_t^{(i)})\}_{i=1}^{n_t}$, of size $n_t$, where sample data $\mathbf{x}_t^{(i)} \in \mathbf{T}$ -- the target domain. Moreover, $y_s^{(i)}, y_t^{(i)} \in \{0,1\}$ are class labels for each sample irrespective of their domain. It is assumed that $n_s \gg n_t$.} Let $f_{dep}(.; \phi)$ \& $f_{indep}(.;\psi)$ be two models which learn domain dependent and independent features respectively ($\phi, \psi$ are learnable parameters). In other words, for any domain 
$\mathbf{\zeta}$ $\in \{\mathbf{S}, \mathbf{T}\}$, $ \forall_{\mathbf{x} \in \zeta } f_{indep}(\mathbf{x}| \mathbf{x} \in \mathbf{S};\psi ) = f_{indep}(\mathbf{x}| \mathbf{x} \in \mathbf{T};\psi )$ \& $ \exists_{\mathbf{x} \in \zeta } f_{dep}(\mathbf{x}| \mathbf{x} \in \mathbf{S};\phi ) \neq f_{dep}(\mathbf{x}| \mathbf{x} \in \mathbf{T};\phi )$. Let $f(.; \theta)$ be a binary-classification model with learnable parameters $\theta$. For brevity, we denote $f_{indep}(\mathbf{x};\psi )$ \& $f_{dep}(\mathbf{x}|\mathbf{x} \in \zeta;\phi )$ as $f_{\psi}(\mathbf{x})$ \& $f_{\phi}(\mathbf{x}, \mathbf{\zeta})$. \textbf{In terms of mathematical notations}, our problem can be stated as: 
\vspace{0.5\baselineskip}

\emph{``Can we learn a classification model $f(.; \theta)$, and feature learning models $f_{\psi}(.), f_{\phi}(.)$ from labeled dataset $\mathcal{D}_s$ of size $n_s$ from source domain $\mathbf{S}$ and labeled dataset $\mathcal{D}_t$ of size $n_t$ from target domain $\mathbf{T}$ (where $n_s \gg n_t$), such that for a target data sample $\mathbf{x_t} \in \mathbf{T}$, $f( \mathbf{x_t}, f_{\psi}(\mathbf{x_t}) , f_{\phi}(\mathbf{x_t},\mathbf{T}); \theta)$ can predict the associated class label $\mathbf{y_t} \in \{0,1\}$?''}.

%In terms of \textbf{our use case}, we can state the problem as follows:\\

%\emph{``Given labeled sound samples from laboratory data and a few labeled sound samples from industry data, can we label unlabeled sound samples from industry data? Here, labelling means finding whether a sound sample is a cut sound or non-cut sound.''}

%In literature, classification models usually refer to single domain classification models, where we learn from samples from a particular domain, and predict the label from samples in the same domain. For example, if we are training on images of animals in sunlight, to predict whether an image is of a cat or of a dog, this kind of model can predict another image of a cat or a dog in sunlight; but not if the picture is taken in dark. If we intend to learn from the pictures of animals in sunlight but predict animals in the dark, we have to use domain adaptation classification models, which can learn to classify on a domain and infer classes in another domain. Another way to improve the classification performance is to learn from both the domains, for example, animals in both sunlight and darkness- so that we can learn domain-dependent (sunlight or dark) and domain-independent (cat or dog) features. Then, if we are given an image of a dog in darkness, the learning model can predict correctly. One way to learn by this way is \emph{Adversarial Domain Adaptation}, where we try to fool a discriminator so that it cannot distinguish from which domain the query image is, and simultaneously learn the classifier. This way, we learn both kinds of features- one that fools the discriminator (leading to domain-independent features), and one that helps to train the classifier (leading to domain-dependent features).  So, For our problem, as we have data available from both the source (lab) and target (industry) domain, we will follow the adversarial domain adaptation approach. We will mostly base our work on \cite{li2023building}, which has used this method of training along with data augmentation to learn from minimal and imbalanced training data from two domains, and infer classes from target domains. We will describe their model, and a modification of it in the later sections. 

\subsection{\icit{}- Flummoxing-Amalgam Representation Adaptation with Discriminator as Adversary} \label{sec:icit}
%At an abstract level, the heart of 
Similar to other adversarial training frameworks, \icit{} also consists of generator(s) and a discriminator (see Figure~\ref{fig:icit}).
%\eunseob{I revised this sentence.}On an abstract level, at the heart of this architecture (see Figure~\ref{fig:icit}), like any other adversarial training, are generator(s) and a discriminator. 
The goal of the adversarial training here is to generate features so that the discriminator cannot distinguish from which domain the features are. The model has two \textit{private} generators for source and target domains separately, $G_S$ and $G_T$, respectively. The corresponding generator takes input sample from a domain and is trained to generate private or domain-dependent features. It also has a \textit{shared} generator $G$ that takes those features as input, for both source and target domain, and generates domain-independent features. This generator directly tries to fool the discriminator $D$ and hence gets feedback in the form of loss propagation to learn how to generate domain-independent features. Practically, the \textit{shared} generator ensures that the classifier $C$ does not require domain information for inference; it only needs to obtain shared feature representations. In a sense, the classifier $C$ learns exclusively from domain-independent features, as the domain-dependent ones are transformed by the generator. 
%\elisa{please move figure 1 near to this paragraph}

\begin{figure}[b]
\centerline{\includegraphics[scale=0.37]{images/faradaynew_new.png}}
\caption{\icit{} Architecture from~\cite{li2023building}}\label{fig:icit}
\end{figure}

%\adrian{The equations takes a lot of space. We can put group 1,2; 3,4; 5,6.}

Formally, in the forward pass, for source domain sample $(\mathbf{x}_s, y_s)$ and target domain sample $(\mathbf{x}_t, y_t)$, we pass them to \textit{Private Source Generator}, $G_S$ and \textit{Private Target Generator}, $G_T$, respectively. We get private features $G_S(\mathbf{x}_s)$ and $G_T(\mathbf{x}_t)$, respectively. 
% Then, we pass them to \textit{Shared Generator}, $G$, to obtain the shared representations, \begin{align}\mathbf{x}_{gs} = G(G_S(\mathbf{x}_s))\end{align} \begin{align}\mathbf{x}_{gt}= G(G_T(\mathbf{x}_t))\end{align}
Then, we pass them to \textit{Shared Generator}, \( G \), to obtain the shared representations, 
%\eunseob{I merged the equations and corrected typos.}
\begin{align} \mathbf{x}_{gs} = G(G_S(\mathbf{x}_s)), \quad \mathbf{x}_{gt} = G(G_T(\mathbf{x}_t)) \end{align}
Then, we pass them to \textit{Discriminator}, \( D \) to obtain
\begin{align} \hat{\mathbf{d}}_{s} = D(\mathbf{x}_{gs}), \quad \hat{\mathbf{d}}_{t} = D(\mathbf{x}_{gt}) \end{align}
and also to \textit{Classifier}, $C$ to obtain \begin{align} \hat{\mathbf{y}}_{s} = C(\mathbf{x}_{gs}), \quad \hat{\mathbf{y}}_{t} = C(\mathbf{x}_{gt}) \end{align}

In backward pass, we compute three losses: (i) classification loss- which is a cross-entropy loss,  \begin{align}\mathcal{L}_c = -{\mathbf{y}_{s}} \cdot \log(\hat{\mathbf{y}_{s}}) - \lambda {\mathbf{y}_{t}} \cdot \log(\hat{\mathbf{y}_{t}})\end{align}(ii) discriminator loss- similar to cross-entropy as the discriminator itself is a classifier for domains,\begin{align}\mathcal{L}_d = -{\mathbf{d}_{s}} \cdot \log(\hat{\mathbf{d}_{s}}) - {\mathbf{d}_{t}} \cdot \log(\hat{\mathbf{d}_{t}})\end{align}  and (iii) Generator loss- it has the inverse form of discriminator loss so that when the discriminator predicts correctly (incorrectly), it gets a negative (positive) reinforcement, \begin{align}\mathcal{L}_g = -{(\mathbf{1}-\mathbf{d}_{s})} \cdot \log(\hat{\mathbf{d}_{s}}) - {(\mathbf{1}-\mathbf{d}_{t})} \cdot \log(\hat{\mathbf{d}_{t}})\end{align} 
The hyperparameter $\lambda$ ensures that the loss from target domain for classification is emphasized more than the source domain, as we will focus on the target domain classification. %\adrian{The above content with the graph should be sufficient. We can remove the rest of the text.}
%\eunseob{Deprecated}
% In the backpropagation step, %\textit{Classifier} and $\textit{Discriminator}$ 
%classifier and the discriminator are only updated by their respective loss gradients, namely \begin{align}\nabla C = \beta \frac{\partial \mathcal{L}_C}{\partial {C}}\end{align} \begin{align}\nabla D = \beta \frac{\partial \mathcal{L}_D}{\partial {D}}\end{align} respectively. But all the generators, along with the generator loss, also receive feedback from the classifier loss as 
%their generated features influence the classification. So, their gradients are formulated as \begin{align}\nabla G_{S} = \beta \frac{\partial \mathcal{L}_g}{\partial G_S} + \gamma \frac{\partial \mathcal{L}_c}{\partial G_S}\end{align} \begin{align}\nabla G_{T} = \beta \frac{\partial \mathcal{L}_g}{\partial G_T} + \gamma \frac{\partial \mathcal{L}_c}{\partial G_T}\end{align} \begin{align}\nabla G = \beta \frac{\partial \mathcal{L}_g}{\partial G} + \gamma \frac{\partial \mathcal{L}_c}{\partial G}\end{align}Here, $\beta, \gamma$ are the hyperparameters. 
%\elisa{I would not report these data as this is confusing for the reader.}
%This model has achieved 75\% accuracy on MixedWM38\footnote{https://github.com/Junliangwangdhu/WaferMap} source and WM-811K\footnote{https://www.kaggle.com/datasets/qingyi/wm811k-wafer-map} as target training data. 

\subsection{\icitmod{}- Domain-Ingrained Representation with Adversary as Critic
} \label{sec:icitmod} 
\icitmod{} is a variant of \icit{} where we modified the model training part based on some intuitions. Firstly, we hypothesize that when the generator $G$ receives private features, the information about the domain from which the features originate is not passed to $G$. 
However, the Classifier $C$ might need some domain-specific features. Therefore, if $G$ can have some latent information about the domain from which the generated features originate, it can generate some domain-dependent features to help the classifier. For this, the discriminator $D$ can help $G$. It will try to correctly classify the domains, and will feedback the loss accordingly to the generator; if $D$ classifies the domain correctly (incorrectly), $G$ will get positive (negative) reinforcement. This ensures that $G$ learns some domain-dependent features too. Hence, the generator loss is now the same as the discriminator loss: \begin{align}\mathcal{L}_g = \mathcal{L}_d = -{\mathbf{d}_{s}} \cdot \log(\hat{\mathbf{d}_{s}}) - {\mathbf{d}_{t}} \cdot \log(\hat{\mathbf{d}_{t}})\end{align} 

Secondly, in \icit{}, source and target classification losses are combined before being passed to the private generators $G_S$ and $G_T$. 
But they should only be responsible for their own domain losses. Hence, we split the classification losses into two components: source and target classification losses:
\begin{equation}
\mathcal{L}_{cs}= -{\mathbf{y}_{s}} \cdot \log(\hat{\mathbf{y}}_{s}), \quad \mathcal{L}_{ct}= -{\mathbf{y}}_{t} \cdot \log(\hat{\mathbf{y}}_{t})
\end{equation}
The classification loss is: \begin{align}\mathcal{L}_c = \mathcal{L}_{cs} + \lambda \mathcal{L}_{ct}\end{align}
Now, the gradient updates for \textit{private generators} are \begin{align}\nabla G_{S} = \beta \frac{\partial \mathcal{L}_g}{\partial G_S} + \gamma \frac{\partial \mathcal{L}_{cs}}{\partial G_S}, \nabla G_{T} = \beta \frac{\partial \mathcal{L}_g}{\partial G_T} + \gamma \frac{\partial \mathcal{L}_{ct}}{\partial G_T}\end{align}
%Now, the gradient updates for \textit{private generators} are \begin{align}\nabla G_{S} = \beta \frac{\partial \mathcal{L}_g}{\partial G_S} + \gamma \frac{\partial \mathcal{L}_{cs}}{\partial G_S}\end{align} \begin{align}\nabla G_{T} = \beta \frac{\partial \mathcal{L}_g}{\partial G_T} + \gamma \frac{\partial \mathcal{L}_{ct}}{\partial G_T}\end{align}

Lastly, instead of a single pass to update the discriminator, classifier, and generators together, we follow the training techniques by Goodfellow et al.~\cite{goodfellow2020generative}. 
For each training step, we take some forward 
passes and update only the discriminator $D$ in each pass. After that, we execute 
again a single forward pass, and update $G$, $G_S$, $G_T$, and $C$. This helps to prevent overfitting and enhance faster convergence. 

\subsection{Model Architecture} \label{sec:mod:arch}

All private generators $G_S, G_T$ have \textbf{Multi Layer Perceptron (MLP)} architecture with 1,025 input dimension, two hidden layers with 768 and 512 nodes, with Sigmoid activations. The shared generator $G$ is also an \textbf{MLP} with 512 input dimensions and a hidden layer with 200 nodes with ReLU activations. Both the discriminator $D$ and the classifier $C$ are also \textbf{MLP} with 200 input dimension and a dense layer of 100 nodes with ReLU activation. For output layer, Softmax is applied. All layers are optimized using the ADAM optimizer \cite{kingma2014adam} with a learning rate of $2 \times 10 ^ {-4}$ and a beta decay of 0.02.



==> first_draft/Results.tex <==
\begin{document}

\begin{tabular}{|c|c|c|c|c|c|c|c|}
 & Source Labeled Data Size & Target Labeled Data Size & Target Test Accuracy Mean VanillaBaselineSingleModel & Target Test Accuracy Mean VanillaBaselineMultiModel & Target Test Accuracy Mean VanillaBaselineFineTunedModel & Target Test Accuracy Mean ICIT-ADV-DA & Target Test Accuracy Mean modified-ICIT-ADV-DA \\
0 & 2000 & 50 & 0.459 & 0.446 & 0.513 & 0.773 & \font-weightbold 0.791 \\
1 & 2000 & 200 & 0.439 & 0.440 & 0.448 & 0.865 & \font-weightbold 0.867 \\
2 & 2000 & 500 & 0.447 & 0.458 & 0.501 & \font-weightbold 0.881 & 0.874 \\
3 & 2000 & 1000 & 0.452 & 0.524 & 0.545 & \font-weightbold 0.889 & 0.851 \\
4 & 2000 & 4000 & 0.451 & 0.501 & 0.565 & \font-weightbold 0.913 & 0.890 \\
5 & 2000 & 10000 & 0.453 & 0.563 & 0.563 & \font-weightbold 0.930 & 0.913 \\
6 & 2000 & 16000 & 0.455 & 0.563 & 0.563 & \font-weightbold 0.925 & 0.916 \\
7 & 5000 & 50 & 0.488 & 0.428 & 0.476 & \font-weightbold 0.805 & 0.784 \\
8 & 5000 & 200 & 0.420 & 0.452 & 0.470 & 0.856 & \font-weightbold 0.876 \\
9 & 5000 & 500 & 0.503 & 0.430 & 0.491 & 0.876 & \font-weightbold 0.884 \\
10 & 5000 & 1000 & 0.492 & 0.452 & 0.563 & 0.892 & \font-weightbold 0.897 \\
11 & 5000 & 4000 & 0.445 & 0.502 & 0.563 & 0.906 & \font-weightbold 0.911 \\
12 & 5000 & 10000 & 0.474 & 0.537 & 0.563 & \font-weightbold 0.928 & 0.916 \\
13 & 5000 & 16000 & 0.499 & 0.498 & 0.563 & \font-weightbold 0.930 & 0.913 \\
14 & 8000 & 50 & 0.445 & 0.407 & 0.461 & 0.788 & \font-weightbold 0.798 \\
15 & 8000 & 200 & 0.442 & 0.461 & 0.461 & 0.851 & \font-weightbold 0.874 \\
16 & 8000 & 500 & 0.452 & 0.480 & 0.497 & 0.871 & \font-weightbold 0.892 \\
17 & 8000 & 1000 & 0.418 & 0.441 & 0.563 & \font-weightbold 0.900 & 0.898 \\
18 & 8000 & 4000 & 0.442 & 0.478 & 0.565 & \font-weightbold 0.924 & 0.912 \\
19 & 8000 & 10000 & 0.447 & 0.497 & 0.563 & \font-weightbold 0.930 & 0.916 \\
20 & 8000 & 16000 & 0.434 & 0.537 & 0.563 & \font-weightbold 0.925 & 0.919 \\
21 & 10000 & 50 & 0.432 & 0.435 & 0.445 & 0.788 & \font-weightbold 0.799 \\
22 & 10000 & 200 & 0.475 & 0.477 & 0.444 & 0.840 & \font-weightbold 0.874 \\
23 & 10000 & 500 & 0.497 & 0.457 & 0.521 & 0.868 & \font-weightbold 0.887 \\
24 & 10000 & 1000 & 0.434 & 0.445 & 0.563 & \font-weightbold 0.901 & \font-weightbold 0.901 \\
25 & 10000 & 4000 & 0.482 & 0.505 & 0.563 & 0.888 & \font-weightbold 0.920 \\
26 & 10000 & 10000 & 0.436 & 0.478 & 0.563 & 0.905 & \font-weightbold 0.924 \\
27 & 10000 & 16000 & 0.450 & 0.516 & 0.563 & 0.904 & \font-weightbold 0.919 \\
28 & 16000 & 50 & 0.450 & 0.418 & 0.505 & 0.797 & \font-weightbold 0.798 \\
29 & 16000 & 200 & 0.448 & 0.490 & 0.486 & \font-weightbold 0.876 & 0.874 \\
30 & 16000 & 500 & 0.437 & 0.442 & 0.519 & 0.879 & \font-weightbold 0.893 \\
31 & 16000 & 1000 & 0.435 & 0.448 & 0.563 & 0.897 & \font-weightbold 0.899 \\
32 & 16000 & 4000 & 0.439 & 0.457 & 0.565 & 0.914 & \font-weightbold 0.916 \\
33 & 16000 & 10000 & 0.448 & 0.519 & 0.563 & 0.912 & \font-weightbold 0.922 \\
34 & 16000 & 16000 & 0.443 & 0.521 & 0.565 & 0.901 & \font-weightbold 0.913 \\
\end{tabular}
\end{document}


==> first_draft/first_draft_abstract.tex <==
\begin{abstract}
Cutting state monitoring in the milling process is crucial for improving manufacturing efficiency and tool life. Cutting sound detection using a machine learning (ML) approach, inspired by the expertise of experienced machinists, can be employed as a cost-effective and non-intrusive method in a complex manufacturing environment. However, labeling industry data for training an ML model is both costly and time-consuming. Moreover, industry data is often scarce. In this study, we propose a novel adversarial domain adaptation (DA) approach to leverage abundant lab data to learn from scarce industry data, both labeled, for labeling data 
%from the same industry domain
for training a cutting-sound detection model. We introduce the notion of private and shared generators - where rather than adapting the features from separate domains directly for a domain-invariant representation, we project them first into two separate latent spaces that jointly work as the feature space for learning domain-independent representations. We also analyze two different mechanisms for adversarial learning where the discriminator works as an adversary and a critic in separate settings. In these two settings, our model is able to learn expressive domain-invariant and domain-ingrained features, respectively. We also have collected cutting sound data, and prepared datasets from lab and industry domain, and evaluate our learning models on them. Experiments show that our models have optimal results compared to the ones by vanilla domain adaptation models.   



\end{abstract}



==> first_draft/first_draft_acknowledgement.tex <==
\section*{Acknowledgement}
This research was supported by NSF Grant No. 2134667 "FMRG: Manufacturing USA: Cyber: Privacy-Preserving Tiny Machine Learning Edge Analytics to Enable AI-Commons for Secure Manufacturing".

==> first_draft/first_draft_conclusion.tex <==
\section{Conclusion}
\mir{Draft conclusion for placeholder}
We discussed the problem of cutting state monitoring in the milling process and how it can be automated with machine learning techniques. We have applied adversarial domain adaptation approach to learn from abundant lab and scarce industry data, to infer the cutting sounds from industry processes. We have discussed how using the discriminator as an adversary and as a critic in separate settings can help our task; and devised a new methodology based on it. In the process, we also constructed cutting sound dataset, which can facilitate this study onwards; and studied the effect of different feature transformations on them. We also evaluated our models on these dataset and achieved optimal performance.  Myriad of extensions and potential
improvements are on the horizon, such as extending our model for multi-modal learning. Also, cross-sensor learning from sound data and studying our model for few or no labeled data from target domain while training are also some interesting directions we are likely to explore.

==> first_draft/first_draft_data_collection.tex <==
\input{tables/data_collection}

\section{Data Collection} \label{sec:datcol}
We collected operational sound data from CNC milling processes in both laboratory and industrial settings. This section briefly summarizes the sensors used, the data collection methodologies, and the notable differences between \textbf{IMI} and \textbf{KRPM} datasets. 
\elisa{In Table I, the entry "Working travel in x X y X z" needs to be complete with the actual numbers.}
\Cref{tab:datacollection} presents a comparison of the datasets. The laboratory data, referred to as \textbf{IMI}, was gathered at the Indiana Next Generation Manufacturing Competitiveness Center (IN-MaC) of the Indiana Manufacturing Institute (IMI) at Purdue University. Detailed information on the laboratory data collection can be found 
in ~\cite{kim2024online}. The industrial data, referred to as \textbf{KRPM}, was obtained from Kirby Risk Precision Machining (KRPM) in Indiana, a company specializing in the manufacturing of engine blocks for the heavy-duty industry. The raw sound data, recorded in WAV format, along with comprehensive descriptions, are accessible at \url{https://github.com/purduelamm/mt_cutting_dataset/}.

The two machines have different configurations, spindle capacities, and sizes. Additionally, the specific milling processes differed between the two settings. At the Purdue laboratory 
%\textbf{IMI}, 
the cutting process involved side milling with simple zig-zag tool paths, encompassing various cutting conditions such as different end mills, materials, and tool setups. In contrast, at Kirby Risk, the process
%\textbf{KRPM} 
included additional cutting processes such as facing and drilling. To label the cutting sound, an expert reviewed recorded video footage of the operation while simultaneously listening to the sound from each sensor, allowing for accurate labeling of the cutting time stamps. Given that the workpieces were made of cast iron and therefore had imprecise shapes, extracting the exact start and end times of the cutting process was challenging. Two types of sound sensors were employed: (1) Microphone, and (2) ISS. A microphone captures ambient noise whereas the ISS captures sound from a stethoscope on the target surface. Details of the ISS can be found in~\cite{yun2020development}. For each dataset three sound sensors were used to ensure a comprehensive data collection.




==> first_draft/first_draft_dataset_preparation.tex <==
\section{Dataset Preparation} \label{sec:datprep}
For both the \imi{} and \kirby{} datasets, we collected separate sound files of cutting processes. Each sound file ranges from 1 minute to 6.5 minute in length and has several time intervals where the machine cutting sounds are heard. \imi{} and \kirby{} have, respectively, 18 and 1 sound files for each sensor, with a total duration of 2789.97 \& 130.27 seconds respectively. Each sound file was sampled with 48 kHz rate, with the help of the Librosa~\cite{mcfee2015librosa} library. After that, these samples were transformed into Fourier domain using Fast Fourier Transformation (FFT)~\cite{nussbaumer1982fast}, with frequency windows set to $\mathit{n_{fft} = 2048}$, in Librosa \cite{mcfee2015librosa}. FFT returns $\mathit{1 + \frac{n_{fft}}{2}}$ frequency beans, hence each sample has $1 + \frac{2048}{2} = 1025$ frequency beans. Each frequency bean value was squared to get the intensity value, and then they converted to Decibels (dB). So, per data sample has 1025 intensities as features. The number of samples in Librosa \cite{mcfee2015librosa} conversion is defined as $\frac{4 \times \text{sampling rate} \times \text{time} }{n_{fft}}$, hence there are $\frac{4 \times 48000 \times 2789.97}{2048} \approx $ 261560 samples in \imi{} and $\frac{4 \times 48000 \times 130.27}{2048} \approx $ 12213 samples in \kirby{}, per sensor. Also, per sensor, the number of cut (non-cut) sample frames are- for \imi{}, 97312 (164248) and for \kirby{}, 5405 (6805).

==> first_draft/first_draft_discussion.tex <==
\section{Discussion}
From the results in \Cref{sec:exp}, we have seen that \icit{} and \icitmod{} achieve near-optimal results while learning from both lab data and a few industry data and inferring on industry data. This matches with our hypothesis that if we can separate domain-dependent and domain-independent features leveraging adversarial learning, we can learn a shared feature space which can be used to classify data from both source and target domain without domain labels. Also, transforming the features before running the models helps reduce the training load as no additional layers were needed to transform the feature spaces into a common range. Apart from learning and testing on randomly permuted and sampled data, we also ran our model on a sound file to label the cutting intervals and got optimal results. Nevertheless, the model still has some limitations. First, our GPU limitations let us only handle 16000 \& 12213 training samples from both domains. To learn a better representation, we need to find out a way to 
%integrate
\elisa{"integrate" does not sound the correct word to be used here. I have replaced with "load"; if you mean something different let me know and we can find a better term.}
load in memory all 261560 samples from the dataset. Second, our current model can only be applied only to data of the same type, that is, sound, or image or text.
%for sound data for nowthe domain data can be from image domain, text domain or a multi-modal domain like image with sound. 
We are yet to test our model on multi-modal data, that is, when the training and testing samples dataset contains data values of different types, to determine whether our methodology requires extensions. 
%Finally, the extent to which our work has been done- it will help greatly in industry research arena by introducing learning-based automation in place of manual annotation of industry data.


==> first_draft/first_draft_experiment.tex <==
\section{Experiments} \label{sec:exp}

\subsection{Experiment settings}
We implemented all our models using 
Tensorflow~\cite{tensorflow2015-whitepaper}, and Librosa~\cite{mcfee2015librosa}. The models were run on a NVIDIA GeForce RTX 3090 GPU with Cuda 12.2 support. For experiments, we split our dataset in 70\%-10\%-20\% ratio for train, validation and test split for each sensor. The details for hyperparameters are described separately in for each experiments.

\subsection{RQ1 Experiment}
The motivation behind our RQ1 experiment is to find out whether we need to perform any transformation on the source and target domain data before passing them to the model. Our hypothesis is: as the source and target domain feature distributions are different, if a priori transformation can improve the single domain classification (same source and domain) performance without the introduction of more deep layers to capture the domain invariant and dependent features, then we can use these transformed features as direct input to the transfer learning task, rather than using the original features as the direct input, which would then require introducing more deep layers. This would help us to learn smaller number of parameters to perform the transfer learning task optimally. For this, we introduce a simple binary classification model comprising of a neural network with a single hidden dense layer with 512 neurons. We use sigmoid and softmax as the activation functions in hidden and output layer respectively. The model architecture can be described as: $Input(1025) \rightarrow Hidden (Dense, 512 \text{ }nodes) \rightarrow sigmoid \rightarrow Output (Dense, 2 \text{ }) \rightarrow Softmax$. We ran the model for 20 epochs, with the batch size set as 128. We also used the same splits as before, and reported our results on validation set instead of test set, as the validation set results reflect more on the model’s generalizablity. Better accuracy in validation ensures that these transformations will also work better for transfer learning task. Also, for this experiment, we loaded all \imi{} data and ran the model. The model was simpler and hence it did not take much memory, so we could load the whole data in memory. The transformations in the experiments are: 
\\

\noindent
(i) Identity: \begin{align}idx(x) = x\end{align} (ii) Standardization: \begin{align}stanx(x) = \frac{x-min(x)}{max(x)-min(x)}\end{align}(iii) Log: \begin{align}logx(x) = 255 * (\frac{\log{(81+x)}}{\log{(81+\max{(x)})}})\end{align} (iv) Sigmoid: \begin{align}sigmoid(x) = 255 * (\frac{e^{x+41}}{1+ e^{x+41}})\end{align} (v) Gamma: \begin{align}gammax(x) = 255 * (\frac{81+x}{81+max{(x)}})^\gamma\end{align} where $\gamma$ is an arbitrary constant. 

From \Cref{tab:rq1imi} and \Cref{tab:rq1kirby}, we can see that for all sensors of both datasets, $gammax$ transformation outperforms all others in validation accuracy, thus being the representation with the greater generalization ability. $stanx$ has the best performance for training accuracy in \imi{} ($gammax$ is not very far). Overall, $gammax$ with $\gamma=4.2$ proves to be the best choice for transformation used in data-preprocessing. \textbf{We use this transformation in the next experiments}.\\ \adrian{To further save the space, we can skip the train accuracy in both tables and merge table 2 and 3 as one table.}
\input{tables/RQ1_results}

\subsection{RQ2 Experiment}
In this experiment, we compare our adversarial DA models with baseline models, for classifying unlabeled target data by learning on large labeled source domain data and small labeled target domain data. We run experiments on nine combinations: from all three sensors of the source domain (\imi{}) to all three sensors of domain (\kirby{}). We compare five models: three vanilla baselines (single, multi and fine-tuned) , and two adversarial DA models (\icit{}, \icitmod{}). For brevity, we refer to the \textbf{Vanilla} \textbf{B}aseline \textbf{S}ingle, \textbf{M}ulti and \textbf{F}ine Tuned \textbf{M}odels respectively as \vbs{}, \vbm{} and \vbf{}.

All the vanilla baselines have same architecture: $Input (1025) \rightarrow Dense(512) \rightarrow ReLu \rightarrow Dropout(p=0.2) \rightarrow Dense(200) \rightarrow ReLu  \rightarrow Dropout(p=0.2) \rightarrow Output(2) \rightarrow Softmax$. The difference is in how they are trained: \vbs{} is trained and validated with source domain data; \vbm{} is trained with validated with both source and target domain data; and finally, \vbf{} is at first trained and validated on source domain data, and later, the final dense layer and output layer are trained or fine tuned again with target domain data, while the first dense layer weights remain frozen. For the vanilla baselines, we have used CrossEntropyLoss with the Adam optimizer \cite{kingma2014adam}, with learning rate 0.001 and $\beta_1 = 0.9$.

For the \icit{}  and \icitmod{} models, we  train and validate on both source and target domain (train and validation split respectively) data. For both \icit{} and \icitmod{} models, we also use tge Adam optimizer for all components with same learning rate ($=0.0002$) and $\beta_1(=0.5)$. The value of loss weights $\beta, \gamma, \lambda$ are all set to 1 after trial and error over different ranges. The model architecture for these two models are the same as described in \Cref{sec:method}.  

All five models are tested on the target domain test data. As for hyperparameters, batch size and learning epoch is set to 128 and 20 respectively. Also, for \icit{} \& \icitmod{}, for each epoch, we iterate over the entire training data for both domains at least once. Thus for one entire training of the source domain, the target domain data is used multiple times. In each epoch, we calculate the number of steps to iterate over entire source domain data, and after a fixed number of steps (=40) iteratively, we perform validation and save the model with best target validation accuracy. 

We iterate over the pairing of source training data size = \{2000, 5000, 8000, 10000, 16000\} and target training data size = \{50, 200, 500, 1000, 4000, 10000, 16000\} (in total $7 \times 5 = 35$ combinations). We run each combination with all models, for three times with fixed seeds and the average  (and standard deviation) value of the accuracy were reported.


\input{tables/RQ2_imi_sensor_0_all}
\input{tables/RQ2_imi_sensor_1_all}
\input{tables/RQ2_imi_sensor_2_all}
\adrian{I don't think we have space for 2 tables, also the table is quite large. I suggest we just chose one table and trim it down to a few rows with most interesting results. And in the text we can say, we only report partial results with sensor 0 due to space limit, full results on sensor 0 as well as the experiment results with sensor 1 will be provided in the final version. }
\Cref{tab:rq2sens0,tab:rq2sens1,tab:rq2sens2} shows the performances of the different models, all three sensor data separately of \imi{} as source and data of sensor $0,1,2$ of \kirby{} respectively, as target. From the results we can see that \icit{} and \icitmod{} outperform all the vanilla baseline models by a considerable margin, with accuracy values ranging over $85\%$ at least, whereas the accuracy of the vanilla baselines is 70\% at most. These experimental results prove our models' effectiveness. 

\subsection{Demonstration on a proper-time ordered sound file}
For the previous experiments, we constructed the sound frames by sampling the sound files on a given rate, and later performing training, validation and testing batches from them after permutations. A question is whether from these permuted sound frames we can reconstruct the prediction for a full sound file. Also, as we ran the experiments for 16000 source and 4000 target sound frames, it remains to see whether we can choose two source sound files (namely Exp1-2 and Exp2-1 from \imi{}) containing around 16000 frames in total, and 4000 sampled frames from \kirby{}, and train on them to predict the cutting-non cut sound for the entire time frame. 
\elisa{There is a logical disconnection between the previous text and the one below. The reader would expect some sentences talking about the experiments you did to reply to this question.}
%The results are shown in
\Cref{fig:demo} shows the results. In the figure, the blue sound wave denotes the real cut (1) - non cut (0) frames, and the red line is the predicted one. We can see that the rate of true positives and negatives are quite high; but the rates of false ones could be reduced by training on more diverse dataset. 
\begin{figure}[htbp]
\centerline{\includegraphics[scale=0.6]{images/RQ5.png}}
\caption{Comparison of ground truth labels and \icitmod{}-inferred labels in a clipped \kirby{} sound file }\label{fig:demo}
\label{fig}
\end{figure}


==> first_draft/first_draft_industrial_background.tex <==
\section{Industrial Background} \label{sec:indback}


\adrian{The initial submission is up to 6 pages including references and figures. We might need to remove this section and merge it into the introduction.}

Optimizing equipment utilization and enhancing productivity are key factors in improving manufacturing competitiveness. Monitoring machine operations plays a pivotal role in enhancing manufacturing production by providing essential information that improves efficiency on 
factory floors~\cite{bueno2020smart}. Accordingly, manufacturing equipment nowadays features Information and Communication Technology (ICT) and Internet of Things (IoT) capabilities, facilitating data exchange of machine operation and the adoption of Artificial Intelligence (AI) solutions~\cite{maier2017big}. MTConnect which is a CNC machine tool data integration standard provides information of events, samples, and conditions from 
controller~\cite{liu2019cyber}. However, MTConnect does not provides exact cutting times. Additionally, many CNC machines estimate cutting time based on the accumulated cutting motion commands (e.g., G01, G02, G03, etc.) in G-Code, which can be inaccurate because it includes air-cutting. Monitoring the cutting state is also challenging when the machine is manually operated by a machinist. Accurate real-time cutting state monitoring can significantly improve factory floor operations.

On top of that, in situations where many legacy machines are still functioning well and widely used for production in real factory settings, it is crucial to digitize the operational information of these machines, which often lack hardware or software interfaces~\cite{guerreiro2018definition}. However, manufacturing companies, particularly Small and Medium-sized Enterprises (SMEs), are often reluctant to invest significantly in retrofitting these machines to gather operational data. Additionally, many SMEs prefer to maintain their existing manufacturing setup and avoid interrupting production for intrusive equipment monitoring, as this can lead to undesirable downtime and changes in production configurations. While machine sound monitoring could be a viable alternative with advances in ML, it faces challenges such as vulnerability to noise and the lack of solutions for various machines and situations. The high cost and labor-intensive process of labeling and gathering data are significant barriers to its adoption. Therefore, effective DA techniques and the development of more generalized models could greatly impact the adoption of machine sound monitoring in the industry.




==> first_draft/first_draft_introduction.tex <==
\section{Introduction}
Machine sound monitoring is a low-cost and non-intrusive method that converts acoustic signals into machine operational information. Manufacturing machines emit sounds containing ample process information as they operate. However, the intricate interactions between components of manufacturing equipment and the complex nature of vibration and sound propagation make modeling sound emission challenging in the unpredictably noisy environment of a real-world factory floor~\cite{wegener2021noise}. As an operator understands machine sounds through experience and learning, machine learning (ML) approaches adopting principles from Automatic Speech Recognition (ASR) have been utilized for machine sound monitoring~\cite{kim2021multiple}.  In the metal cutting industry, continuous monitoring of the cutting state is crucial for evaluating process efficiency ~\cite{liu2018real} and estimating cutting tool life \cite{benkedjouh2015health}.

It is not surprising that experienced machinists can detect cutting sounds solely by listening, even in varying noisy environments across different manufacturing equipment. In wet cutting conditions where coolant fluid floods the area making visual observation impossible, machinists can still discern the cutting state by sound. Additionally, an experienced machinist who primarily operates a specific Computer Numerical Control (CNC) milling machine can easily recognize cutting sounds. When operating another CNC milling machine from a different manufacturer and in a different location, the machinist can quickly identify the cutting sound after familiarizing themselves with the machine and its operations. This ability exemplifies the flexible auditory sensing capabilities of human experts in the manufacturing industry. 

 Machine learning (ML) techniques have been applied to the detection of cutting sounds [] \mir{any citation?}. However, due to the complex nature of manufacturing environments, several critical factors have been overlooked by previous detectors. The numerous combinations of operational conditions—including the type of machine, tool, cutting parameters, and environmental factors—significantly affect the operational sounds. Additionally, the type and placement of sound sensors impact the prediction performance of ML models in machine sound monitoring~\cite{kim2023sound, kim2024operation}. In a controlled laboratory setting, collecting and labeling diverse cutting data for a CNC machine tool equipped with a Cyber-Physical System (CPS) can be automated~\cite{kim2024online}. However, in a real industrial setting, data collection and labeling are costly and time-consuming. This raises an interesting question: {\em Can lab data be useful for training a model that predicts real-world data?} A ML model simply trained on lab data is typically unable to make accurate prediction on real industry data due to distinct sound emission characteristics between different machines and settings. Therefore, to effectively train the model, it is crucial to consider the different domains created by varying machine types, cutting conditions, and sensor types and placements.

% In a well-established lab setting, labeling of cutting data for CNC machine tool which has a Cyber-Physical System (CPS) could be automatically performed \cite{kim2024online}. In real industry setting, however, labeling is costly and time consuming \cite{wang2022cost}. Moreover, there are countless of combinations of operational conditions such as machine, tool, cutting parameters, and environment which affect operation sound. Sound emission characteristics are distinct from different machines as well as between in lab and industry settings. Even if sound sensor type and placement affect prediction performances of ML models in machine sound monitoring \cite{kim2023sound, kim2024operation}, sensor selection and installation could be limited. Thus, to effectively train the model, it is important to consider not only the imbalance of datasets but also the different domains created by machine types, cutting conditions, sensor types, and locations.

One approach to train an effective ML-based sound detector despite domain differences is through Domain Adaptation (DA)~\cite{ganin2016domain, tzeng2017adversarial, li2023building}. This method typically involves learning a common latent representation from two different domains, referred to as source and target domains. These domains are related but distinct; the source domain has a large training dataset (for example generated in a lab), whereas the target domain as few labeled data obtained from the actual deployment environment of the equipment (e.g., a manufacturing floor).
%with the source domain labeled while the target domain has all, few or no labels. 
A classifier is then trained using such latent common representation, also referred to as {\em domain-independent representation}. Because the representation is domain-invariant, the classifier can be ``transferred'' to make predictions in the target domain. For our research problem, the lab data is the labeled source domain and the industrial data is the target domain.
%, where \textbf{all} data are labeled.

In this work, we collected cutting datasets from CNC milling machines in both lab and industrial settings. These datasets were gathered from three sound sensors placed at different locations. The machines in the lab and industrial settings vary in configuration and size. The dataset collected in the lab setting is abundant, while the one collected in the industrial setting is scarce. Our work for the design a suitable DA approach to train a cutting detection model for deployment in a real factory floor,  answers the following Research  Questions (RQs):

\newlist{researchquestions}{enumerate}{1}
\setlist[researchquestions,1]{
    label=RQ\arabic*),
    left=10pt,
    leftmargin=*,
    labelsep=0.5em,
    listparindent=1em,
    align=left
}

\begin{researchquestions}
    \item Which type of transformation for the sound features improves learning performance?
    \item How good is DA for learning on adequate source and inadequate target labeled data, and performing inference on unlabeled target domain data?
    %\item What is the relation between the sizes of provided source and target labeled training data in terms of accuracy performance?
\end{researchquestions}


To answer the first question, we have experimentally evaluated single domain classification on both lab and industry data for separate sensors, after transforming their features in different ways. We show that, compared with other feature transformations, the Gamma ($\gamma = 4.2$) transformation has the best performance on training and validation performance. For the second research question, we compare two models: one has been developed 
by Li et al.~\cite{li2023building} but applied only the image data; the other is a modification of the first approach and our novel contribution. We refer the first model as \icit{} (\icitfull{})- as it fools (``flummoxes'') the adversarial discriminator by adapting through the mixing (``amalgamation'') of separate latent space representations for both domains. We refer to the second model as \icitmod{} (\icitmodfull{})- as in this methodology the generator will receive feedback from the discriminator more as a critic than as an adversary, to ingrain \adrian{Remove a bit of} a bit of domain identity information in the shared representation space.

\textbf{Paper organization.} In \Cref{sec:relwork,,sec:indback}, we provide background about ML based sound monitoring technique, domain adaptation and why is an important technique in industry-based use cases. Later, in \Cref{sec:datcol,,sec:datprep}, we discuss our process for lab and industry data collection and pre-preprocessing for our DA task, %and how we  preproces them for learning. 
Then, in \Cref{sec:method}, we formulate our research problem, and provide details about \icit{} and \icitmod{}. Finally, in \Cref{sec:exp}, we report the results of our  the evaluations with respect to our two research questions, by comparing different transformations and domain adaptation models. We also give a demonstration of our model on a short cutting-sound file.




==> first_draft/first_draft_methodology.tex <==
\section{Methodology} \label{sec:method}

Our approach is mostly based on the methodology by Li et al.~\cite{li2023building}, which uses DA along with data augmentation for training a target model from minimal and imbalanced training data from two domains (e.g., source and target), able to infer classes for samples from the target domains. We first give our problem statement in \Cref{sec:probstate}, followed by a description of the \icit{} model in \Cref{sec:icit}, and our new approach in \Cref{sec:icitmod}.

\subsection{Problem Statement} \label{sec:probstate}
\adrian{This section can be reduced. For example, we don't need to state the research problems in three ways. We can just keep the use case one and maybe the math one.}
\textbf{In words}, our research problem can be stated as follows:\\

\emph{``Given a large labeled dataset from a source domain, and a way smaller labeled dataset from a target domain, can we train a model which can classify samples
%an unlabeled dataset 
from the target domain, by learning domain dependent and domain independent features from source and target domains?''}\\

Formally, {Let $\mathcal{D}_s = \{(\mathbf{x}_s^{(i)}, y_s^{(i)})\}_{i=1}^{n_s}$, be a labeled dataset of size $n_s$, where sample data $\mathbf{x}_s^{(i)} \in \mathbf{S}$ -- the source domain. Also, let another labelled dataset be $\mathcal{D}_t= \{(\mathbf{x}_t^{(i)}, y_t^{(i)})\}_{i=1}^{n_t}$, of size $n_t$, where sample data $\mathbf{x}_t^{(i)} \in \mathbf{T}$ -- the target domain. Moreover, $y_s^{(i)}, y_t^{(i)} \in \{0,1\}$ are class labels for each sample irrespective of their domain. It is assumed that $n_s \gg n_t$.} Let $f_{dep}(.; \phi)$ \& $f_{indep}(.;\psi)$ be two models which learn domain dependent and independent features respectively ($\phi, \psi$ are learnable parameters). In other words, for a domain 
$\mathbf{\zeta}$ $\in \{\mathbf{S}, \mathbf{T}\}$, $ \forall_{\mathbf{x} \in \zeta } f_{indep}(\mathbf{x}| \mathbf{x} \in \mathbf{\zeta};\psi ) = f_{indep}(\mathbf{x};\psi )$ \& $ \exists_{\mathbf{x} \in \zeta } f_{dep}(\mathbf{x}| \mathbf{x} \in \mathbf{\zeta};\phi ) \neq f_{dep}(\mathbf{x};\phi )$. Let $f(.; \theta)$ be a binary-classification model with learnable parameters $\theta$. For brevity, we denote $f_{indep}(\mathbf{x};\psi )$ \& $f_{dep}(\mathbf{x}|\mathbf{x} \in \zeta;\phi )$ as $f_{\psi}(\mathbf{x})$ \& $f_{\phi}(\mathbf{x}, \mathbf{\zeta})$. \textbf{In terms of mathematical notations}, our problem can be stated as: \\\\\emph{``Can we learn a classification model $f(.; \theta)$, and feature learning models $f_{\psi}(.), f_{\phi}(.)$ from labeled dataset $\mathcal{D}_s$ of size $n_s$ from source domain $\mathbf{S}$ and labeled dataset $\mathcal{D}_t$ of size $n_t$ from target domain $\mathbf{T}$ (where $n_s \gg n_t$), such that for a target data sample $\mathbf{x_t} \in \mathbf{T}$, $f( \mathbf{x_t}, f_{\phi}(\mathbf{x_t},\mathbf{T}) ,f_{\psi}(\mathbf{x_t} ); \theta)$ can predict the associated class label $\mathbf{y_t} \in \{0,1\}$?''}.
\\

In terms of \textbf{our use case}, we can state the problem as follows:\\

\emph{``Given labeled sound samples from laboratory data and a few labeled sound samples from industry data, can we label unlabeled sound samples from industry data? Here, labelling means finding whether a sound sample is a cut sound or non-cut sound.''}

%In literature, classification models usually refer to single domain classification models, where we learn from samples from a particular domain, and predict the label from samples in the same domain. For example, if we are training on images of animals in sunlight, to predict whether an image is of a cat or of a dog, this kind of model can predict another image of a cat or a dog in sunlight; but not if the picture is taken in dark. If we intend to learn from the pictures of animals in sunlight but predict animals in the dark, we have to use domain adaptation classification models, which can learn to classify on a domain and infer classes in another domain. Another way to improve the classification performance is to learn from both the domains, for example, animals in both sunlight and darkness- so that we can learn domain-dependent (sunlight or dark) and domain-independent (cat or dog) features. Then, if we are given an image of a dog in darkness, the learning model can predict correctly. One way to learn by this way is \emph{Adversarial Domain Adaptation}, where we try to fool a discriminator so that it cannot distinguish from which domain the query image is, and simultaneously learn the classifier. This way, we learn both kinds of features- one that fools the discriminator (leading to domain-independent features), and one that helps to train the classifier (leading to domain-dependent features).  So, For our problem, as we have data available from both the source (lab) and target (industry) domain, we will follow the adversarial domain adaptation approach. We will mostly base our work on \cite{li2023building}, which has used this method of training along with data augmentation to learn from minimal and imbalanced training data from two domains, and infer classes from target domains. We will describe their model, and a modification of it in the later sections. 

\subsection{\icit{}- Flummoxing-Amalgam Representation Adaptation with Discriminator as Adversary} \label{sec:icit}On an abstract level, at the heart of this architecture (see Figure~\ref{fig:icit}), like any other adversarial training, are generator(s) and a discriminator. The goal of the adversarial training here is to generate features so that the discriminator cannot distinguish from which domain the features are from. There are two kinds of generators: \textit{private} and \textit{shared}. There are two \textit{private} generators for source and target domains separately, $G_S, G_T$ respectively- the corresponding generator takes input sample from a domain and is trained to generate private or domain-dependent features. The \textit{shared} generator $G$ takes those features as input, for both source and target domain, and generate domain-independent features. This generator directly tries to fool the discriminator $D$ and hence gets feedback in forms of loss propagation to learn how to generate domain-dependent features. Practically, the \textit{shared} generator makes sure the classifier $C$ does not even need domain information for inference- all it needs to get shared feature representations. In a sense- the classifier $C$ learns only from domain-independent features, as the domain dependent ones get transformed inside the generator. 
\elisa{please move figure 1 near to this paragraph}

\adrian{The equations takes a lot of space. We can put group 1,2; 3,4; 5,6.}

Formally, in the forward pass, for source domain sample $(\mathbf{x}_s, y_s)$ and target domain sample $(\mathbf{x}_t, y_t)$, we pass them to \textit{Private Source Generator}, $G_S$ and \textit{Private Target Generator}, $G_T$, respectively. From there, we get private features $G_S(\mathbf{x}_s)$ \& $G_T(\mathbf{x}_t)$ respectively. Then, we pass them to \textit{Shared Generator}, $G$, to obtain the shared representations, \begin{align}\mathbf{x}_{gs} = G(G_S(\mathbf{x}_s))\end{align} \begin{align}\mathbf{x}_{gt}= G(G_S(\mathbf{x}_t))\end{align}
Then, we pass them to \textit{Discriminator}, $D$ to obtain \begin{align}\hat{\mathbf{d}_{s}}= D(\mathbf{x}_{gs})\end{align} \begin{align}\hat{\mathbf{d}_{t}}= D(\mathbf{x}_{gt})\end{align} and also to \textit{Classifier}, $C$ to obtain \begin{align}\hat{\mathbf{y}_{s}} = C(\mathbf{x}_{gs})\end{align}\begin{align}\hat{\mathbf{y}_{t}} = C(\mathbf{x}_{gt})\end{align} 



In backward pass, we compute three losses: (i) classification Loss- which is a cross-entropy loss,  \begin{align}\mathcal{L}_c = -{\mathbf{y}_{s}} \cdot \log(\hat{\mathbf{y}_{s}}) - \lambda {\mathbf{y}_{s}} \cdot \log(\hat{\mathbf{y}_{s}})\end{align}(ii) discriminator loss- similar to cross-entropy as the discriminator is a classifier for domains\begin{align}\mathcal{L}_d = -{\mathbf{d}_{s}} \cdot \log(\hat{\mathbf{d}_{s}}) - {\mathbf{d}_{t}} \cdot \log(\hat{\mathbf{d}_{t}})\end{align}  and (iii) Generator loss- it has the inverse form of discriminator loss so that when the discriminator predicts correctly (incorrectly), it gets a negative (positive) reinforcement, \begin{align}\mathcal{L}_g = -{(\mathbf{1}-\mathbf{d}_{s})} \cdot \log(\hat{\mathbf{d}_{s}}) - {(\mathbf{1}-\mathbf{d}_{t})} \cdot \log(\hat{\mathbf{d}_{t}})\end{align} The hyperparameter $\lambda$ ensures that the loss from target domain for classification is emphasized more than the source domain, as we will focus on the target domain classification. \adrian{The above content with the graph should be sufficient. We can remove the rest of the text. }In the backpropagation step, %\textit{Classifier} and $\textit{Discriminator}$ 
classifier and the discriminator
are only updated by their respective loss gradients, namely \begin{align}\nabla C = \beta \frac{\partial \mathcal{L}_C}{\partial {C}}\end{align} \begin{align}\nabla D = \beta \frac{\partial \mathcal{L}_D}{\partial {D}}\end{align} respectively. But all the generators, along with the generator loss, also receive feedback from the classifier loss as 
their generated features influence the classification. So, their gradients are formulated as \begin{align}\nabla G_{S} = \beta \frac{\partial \mathcal{L}_g}{\partial G_S} + \gamma \frac{\partial \mathcal{L}_c}{\partial G_S}\end{align} \begin{align}\nabla G_{T} = \beta \frac{\partial \mathcal{L}_g}{\partial G_T} + \gamma \frac{\partial \mathcal{L}_c}{\partial G_T}\end{align} \begin{align}\nabla G = \beta \frac{\partial \mathcal{L}_g}{\partial G} + \gamma \frac{\partial \mathcal{L}_c}{\partial G}\end{align}Here, $\beta, \gamma$ are the hyperparameters. 
\elisa{I would not report these data as this is confusing for the reader.}
This model has achieved 75\% accuracy on MixedWM38\footnote{https://github.com/Junliangwangdhu/WaferMap} source and WM-811K\footnote{https://www.kaggle.com/datasets/qingyi/wm811k-wafer-map} as target training data. 

\begin{figure}[htbp]
\centerline{\includegraphics[scale=0.6]{images/model.png}}
\caption{\icit{} Architecture from~\cite{li2023building}}\label{fig:icit}
\end{figure}

\subsection{\icitmod{}- Domain-Ingrained Representation with Adversary as Critic} \label{sec:icitmod} 
We proposed a modification for \icit{} which is based on some intuitions regarding the training, whereas the model architectures remain the same. First, we hypothesize that when the generator $G$ receives private features, the information concerning from the domain the features originate is not passed to $G$. 
\elisa{I have re-written some of the text above as the original version was bad.}
%not being passed that  from which domain they are coming from. 
But sometimes, the Classifier $C$ might need some domain specific features. So, if $G$ can have some latent information about from which domain the generated features originate, it can generate some domain-dependent feature by itself to help the classifier. For this, the discriminator $D$ can help $G$- it will try to correctly classify the domains, and will feedback the loss accordingly to the generator; so if $D$ classifies the domain correctly (incorrectly), $G$ will get positive (negative) reinforcement. This ensures that $G$ learns some domain-dependent features too. For this reason, generator loss is now the same as the discriminator loss, that is: \begin{align}\mathcal{L}_g = \mathcal{L}_d = -{\mathbf{d}_{s}} \cdot \log(\hat{\mathbf{d}_{s}}) - {\mathbf{d}_{t}} \cdot \log(\hat{\mathbf{d}_{t}})\end{align} 

Second, the classification loss from both source and target domain are combined before being passed to the private generators $G_S, G_T$. But they should only be responsbile to their own domain losses. Hence, we split the classification losses into two components: source classification loss \begin{align}\mathcal{L}_{cs}= -{\mathbf{y}_{s}} \cdot \log(\hat{\mathbf{y}_{s}})\end{align} 

and target classification loss \begin{align}\mathcal{L}_{ct}= -{\mathbf{y}_{t}} \cdot \log(\hat{\mathbf{y}_{t}})\end{align} \begin{align}\mathcal{L}_c = \mathcal{L}_{cs} + \lambda \mathcal{L}_{ct}\end{align}Now, the gradient updates for \textit{private generators} are \begin{align}\nabla G_{S} = \beta \frac{\partial \mathcal{L}_g}{\partial G_S} + \gamma \frac{\partial \mathcal{L}_{cs}}{\partial G_S}\end{align} \begin{align}\nabla G_{T} = \beta \frac{\partial \mathcal{L}_g}{\partial G_T} + \gamma \frac{\partial \mathcal{L}_{ct}}{\partial G_T}\end{align}Third, instead of a single pass to update both discriminator, classifier and generators, we follow the training techniques by Goodfellow et al.~\cite{goodfellow2020generative}. For each training step, we do some forward pass and update the discriminator $D$ accordingly each pass, while keeping the other parts of the model fixed. After that, we execute again a single forward pass, and update $G, G_S, G_T, C$ accordingly. This helps to prevent overfitting and enhance faster convergence. 

\subsection{Model Architecture} 

All private generators $G_S, G_T$ have $Input(1025)\rightarrow Hidden(Dense, 768) \rightarrow Hidden(Dense,512)$ settings with sigmoid activations. The shared generator $G$ has $Input(512) \rightarrow Hidden(Dense,200)$ with ReLU activations. Both the discriminator $D$ and the classifier $C$ hav $Input(200) \rightarrow Hidden(Dense, 100) \rightarrow Output(2)$ layer settings with ReLU after Dense layer and Softmax activation for output layer. All layers are optimized with the ADAM optimizer \cite{kingma2014adam} with a learning rate of $2 \times 10 ^ {-4}$ and beta decay of $0.02$.



==> first_draft/first_draft_reference.tex <==
%\section*{References}
\bibliographystyle{IEEEtran}
\bibliography{main}



==> first_draft/first_draft_related_works.tex <==
\section{Related Works} \label{sec:relwork}
In the following sections, we discuss related work on machine sound monitoring and adversarial DA.
\subsection{Machine sound monitoring technique}
To tackle noise from sources other than the target machine, the Internal Sound Sensor (ISS) consisting of a stethoscope and a USB microphone was developed~\cite{yun2020development}. Similar to how a doctor inspects a patient's organ sounds using a stethoscope, the ISS focuses on sound from the target surface while minimizing external sound interference. The ISS demonstrated better prediction accuracy in detecting manufacturing equipment operations compared to a standard
microphone~\cite{kim2024operation}. While microphones capture ambient sound for operation and event prediction from multiple equipment or sources~\cite{kim2021sound}, in industrial scenarios, the types and locations of sound sensors can vary and be limited. Therefore, further research on sensor DA is critical.

In machine sound monitoring, frequency domain techniques or related methods, such as spectrograms, have been widely employed for feature extraction and have proven effective as ML model inputs. The frequency domain approach based on Fast Fourier Transform (FFT) captures the spectral content of the signal, highlighting dominant frequencies and harmonic structures~\cite{lauro2014monitoring}, which are essential for identifying specific machine states. These techniques allow for a detailed analysis of sound signals, facilitating the detection of patterns that are not easily discernible in the time domain~\cite{lei2008new}. Convolutional Neural Networks (CNNs) have been adopted in various classification tasks for manufacturing operation monitoring, such as the running state of machine tool 
components~\cite{kim2021multiple}, the operational state of multiple 
machines~\cite{kim2021sound}, runtime and productivity~\cite{kim2024online}, and cutting sound prediction~\cite{kim2023sound,kim2023real-time}. A 1D CNN using FFT features has shown the ability to detect subtle cutting sounds in micro-volume fine-milling processes and demonstrated a fast response for real-time monitoring applications~\cite{kim2023real-time}. 

However, none of the previous works have investigated the effect of FFT feature transformation on improving learning performance, and transfer learning and DA for multiple machines performing the same process in real industrial scenarios. In this paper, we address feature transformation for 1D CNNs and propose a novel adversarial DA approach for effective transfer learning and the training of a generalized model from abundant lab-generated data and scarce industrial data for cutting state detection.


\subsection{Adversarial domain adaptation}

These methods generally aim to learn a latent representation using two competing networks: a feature extractor and a  discriminator. One of the pioneering methods in this area is the Domain Adversarial Neural Network (DANN)~\cite{ganin2016domain}, which consists of three components: a feature extractor, a label predictor, and a domain classifier. In DANN, the generator is adversarially trained to maximize the domain classifier's loss by reversing its gradients. At the same time, the generator and label predictor work together to learn a representation that is domain-invariant. Similarly, the Adversarial Discriminative Domain Adaptation (ADDA)~\cite{tzeng2017adversarial} approach employs analogous network components but involves a multi-stage training process for these components. A recent method that aligns closely with our research is proposed by Li et al.~\cite{li2023building}. This approach combines DA with data augmentation to handle minimal and imbalanced training data from two domains, namely the source domain and the target domain, and to infer classes in target domains. However, these methods have primarily been applied and assessed in the context of image classification and object detection for source and target domains of images. Research has not explored domain knowledge adaptation for machine sound monitoring with the goal of training models for deployment across different machines, sensors, and environments.

==> first_draft/tables/RQ1_results.tex <==
\begin{table}[hbtp]
\caption{RQ1- Performance Comparison of Different Features Transformations on separate sensors of \imi{}}\label{tab:rq1imi}
\centering
\begin{tabular}{|c|cccccc|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Trans-\\ formation\end{tabular}} & \multicolumn{3}{c|}{Train Accuracy}                                                                                                                                                                                         & \multicolumn{3}{c|}{Validation Accuracy}                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{}                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 1\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 2\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 1\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Sensor 2\end{tabular} \\ \hline
$idx$                                                               & \multicolumn{1}{c|}{0.696}                                              & \multicolumn{1}{c|}{0.697}                                              & \multicolumn{1}{c|}{0.628}                                              & \multicolumn{1}{c|}{0.626}                                              & \multicolumn{1}{c|}{0.628}                                              & 0.623                                              \\ \hline
$stanx$                                                             & \multicolumn{1}{c|}{\textbf{0.987}}                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.984}}             & \multicolumn{1}{c|}{\textbf{0.993}}                                     & \multicolumn{1}{c|}{0.992}                                              & \multicolumn{1}{c|}{0.993}                                              & 0.992                                              \\ \hline
$logx$                                                          & \multicolumn{1}{c|}{0.676}                                              & \multicolumn{1}{c|}{0.677}                                              & \multicolumn{1}{c|}{0.941}                                              & \multicolumn{1}{c|}{0.942}                                              & \multicolumn{1}{c|}{0.972}                                              & 0.972                                              \\ \hline
$sigmoidx$                                                      & \multicolumn{1}{c|}{0.951}                                              & \multicolumn{1}{c|}{0.95}                                               & \multicolumn{1}{c|}{0.99}                                               & \multicolumn{1}{c|}{0.99}                                               & \multicolumn{1}{c|}{0.992}                                              & 0.991                                              \\ \hline
$gammax$                                                        & \multicolumn{1}{c|}{0.984}                                              & \multicolumn{1}{c|}{0.983}                                              & \multicolumn{1}{c|}{\textbf{0.993}}                                     & \multicolumn{1}{c|}{\textbf{0.993}}                                     & \multicolumn{1}{c|}{\textbf{0.994}}                                     & \textbf{0.993}                                     \\ \hline
\end{tabular}
\end{table}

\begin{table}[hbtp]
\centering
\caption{RQ1- Performance Comparison of Different Features Transformations on separate sensors of \kirby{}}\label{tab:rq1kirby}
\begin{tabular}{|c|cccccc|}
\hline


\textbf{\begin{tabular}[c]{@{}c@{}}Trans-\\ formation\end{tabular}} & \multicolumn{3}{c|}{Train Accuracy}                                                                                                                                                                                         & \multicolumn{3}{c|}{Validation Accuracy}                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{}                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 1\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 2\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 1\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Sensor 2\end{tabular} \\ \hline
$idx$                                                               & \multicolumn{1}{c|}{0.537}                                              & \multicolumn{1}{c|}{0.523}                                              & \multicolumn{1}{c|}{0.534}                                              & \multicolumn{1}{c|}{0.551}                                              & \multicolumn{1}{c|}{0.558}                                              & 0.544                                              \\ \hline
$stanx$                                                             & \multicolumn{1}{c|}{0.917}                                              & \multicolumn{1}{c|}{0.916}                                              & \multicolumn{1}{c|}{0.803}                                              & \multicolumn{1}{c|}{0.786}                                              & \multicolumn{1}{c|}{0.836}                                              & 0.544                                              \\ \hline
$logx$                                                          & \multicolumn{1}{c|}{0.54}                                               & \multicolumn{1}{c|}{0.527}                                              & \multicolumn{1}{c|}{0.538}                                              & \multicolumn{1}{c|}{0.541}                                              & \multicolumn{1}{c|}{0.733}                                              & 0.727                                              \\ \hline
$sigmoidx$                                                      & \multicolumn{1}{c|}{0.892}                                              & \multicolumn{1}{c|}{0.86}                                               & \multicolumn{1}{c|}{0.932}                                              & \multicolumn{1}{c|}{0.82}                                               & \multicolumn{1}{c|}{0.941}                                              & 0.821                                              \\ \hline
$gammax$                                                        & \multicolumn{1}{c|}{\textbf{1}}                                         & \multicolumn{1}{c|}{\textbf{0.959}}                                     & \multicolumn{1}{c|}{\textbf{0.95}}                                      & \multicolumn{1}{c|}{\textbf{0.914}}                                     & \multicolumn{1}{c|}{\textbf{0.952}}                                     & \textbf{0.883}                                     \\ \hline
\end{tabular}
\end{table}

==> first_draft/tables/RQ2_imi_sensor0.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[hbtp]
\begin{tabular}{|c|c|ccccc|}
\centering

\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\ Data \\ Size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\ Data\\ Size\end{tabular}} & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Target Test Accuracy for Kirby Sensor 0}}                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|l|}{\textbf{}}                                                    & \multicolumn{1}{l|}{\textbf{}}                                                  & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ Baseline\\ Single\\ Model\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ Baseline\\ Multi\\ Model\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ Baseline\\ FineTuned\\ Model\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}ICIT-\\ ADV-DA\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}modified\\ ICIT-\\ ADV-DA\end{tabular}} \\ \hline
2000                                                                               & 50                                                                              & \multicolumn{1}{c|}{0.459}                                                                                & \multicolumn{1}{c|}{0.446}                                                                               & \multicolumn{1}{c|}{0.513}                                                                                   & \multicolumn{1}{c|}{0.773}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.791}                                     \\ \hline
2000                                                                               & 200                                                                             & \multicolumn{1}{c|}{0.439}                                                                                & \multicolumn{1}{c|}{0.44}                                                                                & \multicolumn{1}{c|}{0.448}                                                                                   & \multicolumn{1}{c|}{0.865}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.867}                                     \\ \hline
2000                                                                               & 500                                                                             & \multicolumn{1}{c|}{0.447}                                                                                & \multicolumn{1}{c|}{0.458}                                                                               & \multicolumn{1}{c|}{0.501}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.881}}                          & 0.874                                                                      \\ \hline
2000                                                                               & 1000                                                                            & \multicolumn{1}{c|}{0.452}                                                                                & \multicolumn{1}{c|}{0.524}                                                                               & \multicolumn{1}{c|}{0.545}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.889}}                          & 0.851                                                                      \\ \hline
2000                                                                               & 4000                                                                            & \multicolumn{1}{c|}{0.451}                                                                                & \multicolumn{1}{c|}{0.501}                                                                               & \multicolumn{1}{c|}{0.565}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.913}}                          & 0.89                                                                       \\ \hline
2000                                                                               & 10000                                                                           & \multicolumn{1}{c|}{0.453}                                                                                & \multicolumn{1}{c|}{0.563}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.93}}                           & 0.913                                                                      \\ \hline
2000                                                                               & 16000                                                                           & \multicolumn{1}{c|}{0.455}                                                                                & \multicolumn{1}{c|}{0.563}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.925}}                          & 0.916                                                                      \\ \hline
5000                                                                               & 50                                                                              & \multicolumn{1}{c|}{0.488}                                                                                & \multicolumn{1}{c|}{0.428}                                                                               & \multicolumn{1}{c|}{0.476}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.805}}                          & 0.784                                                                      \\ \hline
5000                                                                               & 200                                                                             & \multicolumn{1}{c|}{0.42}                                                                                 & \multicolumn{1}{c|}{0.452}                                                                               & \multicolumn{1}{c|}{0.47}                                                                                    & \multicolumn{1}{c|}{0.856}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.876}                                     \\ \hline
5000                                                                               & 500                                                                             & \multicolumn{1}{c|}{0.503}                                                                                & \multicolumn{1}{c|}{0.43}                                                                                & \multicolumn{1}{c|}{0.491}                                                                                   & \multicolumn{1}{c|}{0.876}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.884}                                     \\ \hline
5000                                                                               & 1000                                                                            & \multicolumn{1}{c|}{0.492}                                                                                & \multicolumn{1}{c|}{0.452}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.892}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.897}                                     \\ \hline
5000                                                                               & 4000                                                                            & \multicolumn{1}{c|}{0.445}                                                                                & \multicolumn{1}{c|}{0.502}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.906}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.911}                                     \\ \hline
5000                                                                               & 10000                                                                           & \multicolumn{1}{c|}{0.474}                                                                                & \multicolumn{1}{c|}{0.537}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.928}}                          & 0.916                                                                      \\ \hline
5000                                                                               & 16000                                                                           & \multicolumn{1}{c|}{0.499}                                                                                & \multicolumn{1}{c|}{0.498}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.93}}                           & 0.913                                                                      \\ \hline
8000                                                                               & 50                                                                              & \multicolumn{1}{c|}{0.445}                                                                                & \multicolumn{1}{c|}{0.407}                                                                               & \multicolumn{1}{c|}{0.461}                                                                                   & \multicolumn{1}{c|}{0.788}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.798}                                     \\ \hline
8000                                                                               & 200                                                                             & \multicolumn{1}{c|}{0.442}                                                                                & \multicolumn{1}{c|}{0.461}                                                                               & \multicolumn{1}{c|}{0.461}                                                                                   & \multicolumn{1}{c|}{0.851}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.874}                                     \\ \hline
8000                                                                               & 500                                                                             & \multicolumn{1}{c|}{0.452}                                                                                & \multicolumn{1}{c|}{0.48}                                                                                & \multicolumn{1}{c|}{0.497}                                                                                   & \multicolumn{1}{c|}{0.871}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.892}                                     \\ \hline
8000                                                                               & 1000                                                                            & \multicolumn{1}{c|}{0.418}                                                                                & \multicolumn{1}{c|}{0.441}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.9}}                            & 0.898                                                                      \\ \hline
8000                                                                               & 4000                                                                            & \multicolumn{1}{c|}{0.442}                                                                                & \multicolumn{1}{c|}{0.478}                                                                               & \multicolumn{1}{c|}{0.565}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.924}}                          & 0.912                                                                      \\ \hline
8000                                                                               & 10000                                                                           & \multicolumn{1}{c|}{0.447}                                                                                & \multicolumn{1}{c|}{0.497}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.93}}                           & 0.916                                                                      \\ \hline
8000                                                                               & 16000                                                                           & \multicolumn{1}{c|}{0.434}                                                                                & \multicolumn{1}{c|}{0.537}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.925}}                          & 0.919                                                                      \\ \hline
10000                                                                              & 50                                                                              & \multicolumn{1}{c|}{0.432}                                                                                & \multicolumn{1}{c|}{0.435}                                                                               & \multicolumn{1}{c|}{0.445}                                                                                   & \multicolumn{1}{c|}{0.788}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.799}                                     \\ \hline
10000                                                                              & 200                                                                             & \multicolumn{1}{c|}{0.475}                                                                                & \multicolumn{1}{c|}{0.477}                                                                               & \multicolumn{1}{c|}{0.444}                                                                                   & \multicolumn{1}{c|}{0.84}                                                            & \cellcolor[HTML]{FFFFFF}\textbf{0.874}                                     \\ \hline
10000                                                                              & 500                                                                             & \multicolumn{1}{c|}{0.497}                                                                                & \multicolumn{1}{c|}{0.457}                                                                               & \multicolumn{1}{c|}{0.521}                                                                                   & \multicolumn{1}{c|}{0.868}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.887}                                     \\ \hline
10000                                                                              & 1000                                                                            & \multicolumn{1}{c|}{0.434}                                                                                & \multicolumn{1}{c|}{0.445}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.901}}                          & \cellcolor[HTML]{FFFFFF}\textbf{0.901}                                     \\ \hline
10000                                                                              & 4000                                                                            & \multicolumn{1}{c|}{0.482}                                                                                & \multicolumn{1}{c|}{0.505}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.888}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.92}                                      \\ \hline
10000                                                                              & 10000                                                                           & \multicolumn{1}{c|}{0.436}                                                                                & \multicolumn{1}{c|}{0.478}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.905}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.924}                                     \\ \hline
10000                                                                              & 16000                                                                           & \multicolumn{1}{c|}{0.45}                                                                                 & \multicolumn{1}{c|}{0.516}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.904}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.919}                                     \\ \hline
16000                                                                              & 50                                                                              & \multicolumn{1}{c|}{0.45}                                                                                 & \multicolumn{1}{c|}{0.418}                                                                               & \multicolumn{1}{c|}{0.505}                                                                                   & \multicolumn{1}{c|}{0.797}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.798}                                     \\ \hline
16000                                                                              & 200                                                                             & \multicolumn{1}{c|}{0.448}                                                                                & \multicolumn{1}{c|}{0.49}                                                                                & \multicolumn{1}{c|}{0.486}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.876}}                          & 0.874                                                                      \\ \hline
16000                                                                              & 500                                                                             & \multicolumn{1}{c|}{0.437}                                                                                & \multicolumn{1}{c|}{0.442}                                                                               & \multicolumn{1}{c|}{0.519}                                                                                   & \multicolumn{1}{c|}{0.879}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.893}                                     \\ \hline
16000                                                                              & 1000                                                                            & \multicolumn{1}{c|}{0.435}                                                                                & \multicolumn{1}{c|}{0.448}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.897}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.899}                                     \\ \hline
16000                                                                              & 4000                                                                            & \multicolumn{1}{c|}{0.439}                                                                                & \multicolumn{1}{c|}{0.457}                                                                               & \multicolumn{1}{c|}{0.565}                                                                                   & \multicolumn{1}{c|}{0.914}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.916}                                     \\ \hline
16000                                                                              & 10000                                                                           & \multicolumn{1}{c|}{0.448}                                                                                & \multicolumn{1}{c|}{0.519}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.912}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.922}                                     \\ \hline
16000                                                                              & 16000                                                                           & \multicolumn{1}{c|}{0.443}                                                                                & \multicolumn{1}{c|}{0.521}                                                                               & \multicolumn{1}{c|}{0.565}                                                                                   & \multicolumn{1}{c|}{0.901}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.913}                                     \\ \hline
\end{tabular}
\end{table}

==> first_draft/tables/RQ2_imi_sensor_0_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[htbp]
\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{0}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens0}


\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
                                                                                            &                                                                                          & \multicolumn{15}{c|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Target Test Accuracy for Kirby (in \%)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \cline{3-17} 
                                                                                            &                                                                                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 0}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 2}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{3-17} 
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\Data Size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\Data Size\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{} \end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular} \\ \hline
2000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{45.9}                                                                            & \multicolumn{1}{c|}{44.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{77.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.1}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{45.8}                                                                           & \multicolumn{1}{c|}{49.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.8}}                     & \multicolumn{1}{c|}{72.5}                                                                     & \multicolumn{1}{c|}{43.3}                                                                            & \multicolumn{1}{c|}{44}                                                                             & \multicolumn{1}{c|}{46.9}                                                                                   & \multicolumn{1}{c|}{73.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{74.2}                                    \\ \hline
2000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{44}                                                                             & \multicolumn{1}{c|}{44.8}                                                                                   & \multicolumn{1}{c|}{86.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.7}}                                    & \multicolumn{1}{c|}{43.8}                                                                            & \multicolumn{1}{c|}{46.9}                                                                           & \multicolumn{1}{c|}{48.8}                                                                                   & \multicolumn{1}{c|}{79.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.7}}                                    & \multicolumn{1}{c|}{43.3}                                                                            & \multicolumn{1}{c|}{43.7}                                                                           & \multicolumn{1}{c|}{50.3}                                                                                   & \multicolumn{1}{c|}{78.5}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{78.9}                                    \\ \hline
2000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{44.7}                                                                            & \multicolumn{1}{c|}{45.8}                                                                           & \multicolumn{1}{c|}{50.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.1}}                     & \multicolumn{1}{c|}{87.4}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{47.2}                                                                           & \multicolumn{1}{c|}{53.4}                                                                                   & \multicolumn{1}{c|}{77}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{49.2}                                                                           & \multicolumn{1}{c|}{48.6}                                                                                   & \multicolumn{1}{c|}{79.5}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{80.2}                                    \\ \hline
2000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{45.2}                                                                            & \multicolumn{1}{c|}{52.4}                                                                           & \multicolumn{1}{c|}{54.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{85.1}                                                                     & \multicolumn{1}{c|}{47.1}                                                                            & \multicolumn{1}{c|}{50.8}                                                                           & \multicolumn{1}{c|}{59.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.8}}                     & \multicolumn{1}{c|}{77.5}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{49.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{78.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{78.7}                                    \\ \hline
2000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{45.1}                                                                            & \multicolumn{1}{c|}{50.1}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                     & \multicolumn{1}{c|}{89}                                                                       & \multicolumn{1}{c|}{43.3}                                                                            & \multicolumn{1}{c|}{54.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{48.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.8}                                    \\ \hline
2000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{45.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{93}}                       & \multicolumn{1}{c|}{91.3}                                                                     & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.5}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
2000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{45.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.5}}                     & \multicolumn{1}{c|}{91.6}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.5}                                    \\ \hline
5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{48.8}                                                                            & \multicolumn{1}{c|}{42.8}                                                                           & \multicolumn{1}{c|}{47.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{78.4}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{47.2}                                                                           & \multicolumn{1}{c|}{43.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.6}}                     & \multicolumn{1}{c|}{72.2}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{45.7}                                                                           & \multicolumn{1}{c|}{43.7}                                                                                   & \multicolumn{1}{c|}{73.5}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.7}                                    \\ \hline
5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{42}                                                                              & \multicolumn{1}{c|}{45.2}                                                                           & \multicolumn{1}{c|}{47}                                                                                     & \multicolumn{1}{c|}{85.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.6}}                                    & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{43.9}                                                                           & \multicolumn{1}{c|}{46.3}                                                                                   & \multicolumn{1}{c|}{77}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.6}}                                    & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{43.8}                                                                           & \multicolumn{1}{c|}{46.4}                                                                                   & \multicolumn{1}{c|}{78.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79.1}                                    \\ \hline
5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{50.3}                                                                            & \multicolumn{1}{c|}{43}                                                                             & \multicolumn{1}{c|}{49.1}                                                                                   & \multicolumn{1}{c|}{87.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.4}}                                    & \multicolumn{1}{c|}{46.9}                                                                            & \multicolumn{1}{c|}{44.1}                                                                           & \multicolumn{1}{c|}{48.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.6}}                     & \multicolumn{1}{c|}{79.5}                                                                     & \multicolumn{1}{c|}{46.1}                                                                            & \multicolumn{1}{c|}{46.1}                                                                           & \multicolumn{1}{c|}{48.1}                                                                                   & \multicolumn{1}{c|}{81.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.6}                                    \\ \hline
5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{49.2}                                                                            & \multicolumn{1}{c|}{45.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                    & \multicolumn{1}{c|}{46.7}                                                                            & \multicolumn{1}{c|}{47.8}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{78.5}                                                      & \multicolumn{1}{c|}{79.5}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{43.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.2}                                    \\ \hline
5000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{44.5}                                                                            & \multicolumn{1}{c|}{50.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.1}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{51.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{81.4}                                                                     & \multicolumn{1}{c|}{46.1}                                                                            & \multicolumn{1}{c|}{50.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.1}}                     & 80.7                                                                     \\ \hline
5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{47.4}                                                                            & \multicolumn{1}{c|}{53.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.8}}                     & \multicolumn{1}{c|}{91.6}                                                                     & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{53.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.6}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
5000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{49.9}                                                                            & \multicolumn{1}{c|}{49.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{93}}                       & \multicolumn{1}{c|}{91.3}                                                                     & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{51.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.6}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{53.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
8000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{44.5}                                                                            & \multicolumn{1}{c|}{40.7}                                                                           & \multicolumn{1}{c|}{46.1}                                                                                   & \multicolumn{1}{c|}{78.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.8}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{43.9}                                                                           & \multicolumn{1}{c|}{46.6}                                                                                   & \multicolumn{1}{c|}{71.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.8}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{43.8}                                                                           & \multicolumn{1}{c|}{48.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.1}}                     & 72                                                                       \\ \hline
8000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{44.2}                                                                            & \multicolumn{1}{c|}{46.1}                                                                           & \multicolumn{1}{c|}{46.1}                                                                                   & \multicolumn{1}{c|}{85.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{49.9}                                                                           & \multicolumn{1}{c|}{46.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{77.9}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{47.2}                                                                           & \multicolumn{1}{c|}{45.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.2}}                     & 78.9                                                                     \\ \hline
8000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.2}                                                                            & \multicolumn{1}{c|}{48}                                                                             & \multicolumn{1}{c|}{49.7}                                                                                   & \multicolumn{1}{c|}{87.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{44}                                                                             & \multicolumn{1}{c|}{53.6}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{80.5}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{48}                                                                             & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.1}                                    \\ \hline
8000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{41.8}                                                                            & \multicolumn{1}{c|}{44.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90}}                       & \multicolumn{1}{c|}{89.8}                                                                     & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{45.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.2}}                                    & \multicolumn{1}{c|}{43.4}                                                                            & \multicolumn{1}{c|}{43.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.9}                                    \\ \hline
8000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{44.2}                                                                            & \multicolumn{1}{c|}{47.8}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.4}}                     & \multicolumn{1}{c|}{91.2}                                                                     & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{52.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.2}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{52.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
8000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{44.7}                                                                            & \multicolumn{1}{c|}{49.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{93}}                       & \multicolumn{1}{c|}{91.6}                                                                     & \multicolumn{1}{c|}{46.5}                                                                            & \multicolumn{1}{c|}{52.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{53.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{43.4}                                                                            & \multicolumn{1}{c|}{53.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.5}}                     & \multicolumn{1}{c|}{91.9}                                                                     & \multicolumn{1}{c|}{46}                                                                              & \multicolumn{1}{c|}{48.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{43.2}                                                                            & \multicolumn{1}{c|}{43.5}                                                                           & \multicolumn{1}{c|}{44.5}                                                                                   & \multicolumn{1}{c|}{78.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{46}                                                                             & \multicolumn{1}{c|}{44}                                                                                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74}}                       & \multicolumn{1}{c|}{71.7}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{46.3}                                                                           & \multicolumn{1}{c|}{50.8}                                                                                   & \multicolumn{1}{c|}{72.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{47.5}                                                                            & \multicolumn{1}{c|}{47.7}                                                                           & \multicolumn{1}{c|}{44.4}                                                                                   & \multicolumn{1}{c|}{84}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{44.2}                                                                           & \multicolumn{1}{c|}{48.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.2}}                     & \multicolumn{1}{c|}{76.7}                                                                     & \multicolumn{1}{c|}{46.4}                                                                            & \multicolumn{1}{c|}{43.4}                                                                           & \multicolumn{1}{c|}{43.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                       & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{49.7}                                                                            & \multicolumn{1}{c|}{45.7}                                                                           & \multicolumn{1}{c|}{52.1}                                                                                   & \multicolumn{1}{c|}{86.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{48.5}                                                                           & \multicolumn{1}{c|}{49.4}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{81}                                                                       & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{54.1}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.2}                                    \\ \hline
10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{43.4}                                                                            & \multicolumn{1}{c|}{44.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                    & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{46.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81}                                                        & \multicolumn{1}{c|}{81.1}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{43.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.5}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.3}                                    \\ \hline
10000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{50.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92}}                                      & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{46.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                     & \multicolumn{1}{c|}{81.9}                                                                     & \multicolumn{1}{c|}{46.1}                                                                            & \multicolumn{1}{c|}{46.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.6}                                    \\ \hline
10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{43.6}                                                                            & \multicolumn{1}{c|}{47.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.4}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{54.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{52.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
10000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{45}                                                                              & \multicolumn{1}{c|}{51.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{54}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{83.1}                                                                     & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{54.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
16000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{45}                                                                              & \multicolumn{1}{c|}{41.8}                                                                           & \multicolumn{1}{c|}{50.5}                                                                                   & \multicolumn{1}{c|}{79.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.8}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{44.1}                                                                           & \multicolumn{1}{c|}{44.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.5}}                     & \multicolumn{1}{c|}{72.3}                                                                     & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{44.8}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{73.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.9}                                    \\ \hline
16000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{44.8}                                                                            & \multicolumn{1}{c|}{49}                                                                             & \multicolumn{1}{c|}{48.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.6}}                     & \multicolumn{1}{c|}{87.4}                                                                     & \multicolumn{1}{c|}{44.7}                                                                            & \multicolumn{1}{c|}{48.2}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{77.7}                                                      & \multicolumn{1}{c|}{\textbf{77.9}}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{43.7}                                                                           & \multicolumn{1}{c|}{48.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.3}}                     & 78.7                                                                     \\ \hline
16000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{44.2}                                                                           & \multicolumn{1}{c|}{51.9}                                                                                   & \multicolumn{1}{c|}{87.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.3}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{46.3}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.3}}                     & \multicolumn{1}{c|}{79.7}                                                                     & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{46.7}                                                                           & \multicolumn{1}{c|}{51.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.8}}                     & 81.1                                                                     \\ \hline
16000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{43.5}                                                                            & \multicolumn{1}{c|}{44.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{44.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{48.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.6}                                    \\ \hline
16000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{45.7}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{91.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                    & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{54.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.9}}                                    & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{49.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.9}}                     & 82.2                                                                     \\ \hline
16000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{44.8}                                                                            & \multicolumn{1}{c|}{51.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{91.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.2}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{51.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.2}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{53.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
16000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{44.3}                                                                            & \multicolumn{1}{c|}{52.1}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{90.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                    & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{50.7}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.7}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
\end{tabular}
\end{table*}

==> first_draft/tables/RQ2_imi_sensor_1_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[hbtp]

\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{1}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens1}

\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
                                                                                            &                                                                                          & \multicolumn{15}{c|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Target Test Accuracy for Kirby(in \%)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \cline{3-17} 
                                                                                            &                                                                                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 0}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \cline{3-17} 
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\Data Size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\Data Size\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular} \\ \hline
2000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{61.9}                                                                           & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.4}}                     & \multicolumn{1}{c|}{86.3}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{49.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.5}}                     & \multicolumn{1}{c|}{79.4}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                                                      & 76.7                                                                     \\ \hline
2000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{69}                                                                             & \multicolumn{1}{c|}{61.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.4}}                     & \multicolumn{1}{c|}{82.6}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{53.9}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{79.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{80.2}                                    \\ \hline
2000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{74.2}                                                                            & \multicolumn{1}{c|}{68.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.8}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{76.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{56.9}                                                                                   & \multicolumn{1}{c|}{77.8}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
2000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{71.8}                                                                            & \multicolumn{1}{c|}{67.7}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.6}}                     & \multicolumn{1}{c|}{88.5}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.6}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.9}                                                                           & \multicolumn{1}{c|}{57.3}                                                                                   & \multicolumn{1}{c|}{81.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.8}                                    \\ \hline
2000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{75.2}                                                                            & \multicolumn{1}{c|}{61.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.6}}                                                                     & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81}                                                                                         & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
2000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{73.6}                                                                            & \multicolumn{1}{c|}{67.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.5}}                                                                     & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{67.6}                                                                            & \multicolumn{1}{c|}{70.6}                                                                           & \multicolumn{1}{c|}{50.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.9}}                     & \multicolumn{1}{c|}{79.2}                                                                                                      & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72}}                       & \multicolumn{1}{c|}{71.9}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{73.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{65.6}                                                                           & \multicolumn{1}{c|}{53.6}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.7}                                                                           & \multicolumn{1}{c|}{53.2}                                                                                   & \multicolumn{1}{c|}{76.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                                                                       & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{77.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{78.8}                                    \\ \hline
5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{67.7}                                                                            & \multicolumn{1}{c|}{66}                                                                             & \multicolumn{1}{c|}{55.8}                                                                                   & \multicolumn{1}{c|}{88}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.5}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                                      & 79.8                                                                     \\ \hline
5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{63.5}                                                                            & \multicolumn{1}{c|}{67.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.6}}                     & \multicolumn{1}{c|}{89.4}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80}}                       & \multicolumn{1}{c|}{78.3}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{79.7}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{81.9}                                    \\ \hline
5000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{62.7}                                                                            & \multicolumn{1}{c|}{71.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.2}}                     & \multicolumn{1}{c|}{90.1}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.1}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.5}                                    \\ \hline
5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{64.4}                                                                            & \multicolumn{1}{c|}{69.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84}                                      \\ \hline
5000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{63.5}                                                                            & \multicolumn{1}{c|}{74.9}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.4}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
8000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{71.8}                                                                            & \multicolumn{1}{c|}{70.9}                                                                           & \multicolumn{1}{c|}{50.5}                                                                                   & \multicolumn{1}{c|}{77.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                                                                       & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{70.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.2}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{55.8}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{71.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{73.7}                                    \\ \hline
8000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{66.3}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{44.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.5}}                     & \multicolumn{1}{c|}{87.2}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{51.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{78.1}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{51.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.2}}                                                      & 78.9                                                                     \\ \hline
8000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{60.8}                                                                            & \multicolumn{1}{c|}{64.4}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{88.8}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{57}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.4}}                     & \multicolumn{1}{c|}{80.3}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{81.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{81.4}                                    \\ \hline
8000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{64.9}                                                                            & \multicolumn{1}{c|}{68}                                                                             & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{88.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{81.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83.1}                                    \\ \hline
8000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{61}                                                                              & \multicolumn{1}{c|}{80.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.5}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{76.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                                                     & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.5}                                    \\ \hline
8000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{59.8}                                                                            & \multicolumn{1}{c|}{81}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
8000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{67.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.8}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{64.3}                                                                            & \multicolumn{1}{c|}{65.6}                                                                           & \multicolumn{1}{c|}{50.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{78.9}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{50.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{71.6}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{72.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{74}                                      \\ \hline
10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{71.2}                                                                            & \multicolumn{1}{c|}{67}                                                                             & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{87}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.2}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{48.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                     & \multicolumn{1}{c|}{77.8}                                                                                                      & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.8}}                                                      & 78.7                                                                     \\ \hline
10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{67.7}                                                                            & \multicolumn{1}{c|}{62.9}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{88.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.4}}                                                                     & \multicolumn{1}{c|}{55.8}                                                                            & \multicolumn{1}{c|}{57.5}                                                                           & \multicolumn{1}{c|}{53.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                       & \multicolumn{1}{c|}{80}                                                                                                        & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{80.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.4}                                    \\ \hline
10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{64.8}                                                                            & \multicolumn{1}{c|}{69.6}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.4}}                                                                     & \multicolumn{1}{c|}{55.9}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                                                                       & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.7}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83}                                      \\ \hline
10000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{70.3}                                                                            & \multicolumn{1}{c|}{79.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{57.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{81.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.7}                                    \\ \hline
10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{60.2}                                                                            & \multicolumn{1}{c|}{75.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{91.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                                                     & \multicolumn{1}{c|}{54.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.9}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
10000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{63.6}                                                                            & \multicolumn{1}{c|}{75}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92}}                                                                       & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.1}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{62.7}                                                                            & \multicolumn{1}{c|}{68.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.8}}                     & \multicolumn{1}{c|}{78.7}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{54.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.6}}                     & \multicolumn{1}{c|}{72.5}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.8}}                                                      & 73.4                                                                     \\ \hline
16000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{64}                                                                              & \multicolumn{1}{c|}{59.4}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{86.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87}}                                                                       & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                     & \multicolumn{1}{c|}{78}                                                                                                        & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{55.4}                                                                           & \multicolumn{1}{c|}{49.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                                                      & 78.6                                                                     \\ \hline
16000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{67.2}                                                                            & \multicolumn{1}{c|}{62.8}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{87.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{77.4}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{54}                                                                             & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{81.8}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.3}                                    \\ \hline
16000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{59.6}                                                                            & \multicolumn{1}{c|}{69.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{82}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{82.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83.4}                                    \\ \hline
16000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{67.6}                                                                            & \multicolumn{1}{c|}{79.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.2}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.2}}                                                                     & \multicolumn{1}{c|}{55.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{84}                                                                                         & \cellcolor[HTML]{FFFFFF}\textbf{85.1}                                    \\ \hline
16000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{65.7}                                                                            & \multicolumn{1}{c|}{82}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.4}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.8}}                                                                     & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
16000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{59.7}                                                                            & \multicolumn{1}{c|}{79.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.4}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.6}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
\end{tabular}

\end{table*}

==> first_draft/tables/RQ2_imi_sensor_2_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[htbp]

\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{2}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens2}

\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
                                                                                            &                                                                                          & \multicolumn{15}{c|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Target Test Accuracy for Kirby(in \%)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \cline{3-17} 
                                                                                            &                                                                                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 0}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 2}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{3-17} 
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\Data Size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\Data Size\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular} \\ \hline
2000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{45.4}                                                                            & \multicolumn{1}{c|}{57.3}                                                                           & \multicolumn{1}{c|}{56.8}                                                                                   & \multicolumn{1}{c|}{85.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.3}}                                    & \multicolumn{1}{c|}{58.6}                                                                            & \multicolumn{1}{c|}{57.7}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{78.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78}}                       & 77.7                                                                     \\ \hline
2000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.4}                                                                            & \multicolumn{1}{c|}{57.3}                                                                           & \multicolumn{1}{c|}{55.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.6}}                     & \multicolumn{1}{c|}{88.5}                                                                     & \multicolumn{1}{c|}{58.1}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{55.2}                                                                                   & \multicolumn{1}{c|}{78.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.3}}                                    & \multicolumn{1}{c|}{51.6}                                                                            & \multicolumn{1}{c|}{58.6}                                                                           & \multicolumn{1}{c|}{58.7}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79.3}                                    \\ \hline
2000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{59.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                     & \multicolumn{1}{c|}{88.5}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{58.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{77.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{52.8}                                                                            & \multicolumn{1}{c|}{55.8}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{78.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{78.6}                                    \\ \hline
2000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{47}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                     & \multicolumn{1}{c|}{89.1}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.6}}                                    & \multicolumn{1}{c|}{52.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.7}                                    \\ \hline
2000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{44.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{57.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{52.7}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56}                                                                                     & \multicolumn{1}{c|}{80.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
2000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{45.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.7}}                                    & \multicolumn{1}{c|}{58.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.9}}                                    & \multicolumn{1}{c|}{53.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{49.3}                                                                           & \multicolumn{1}{c|}{56.1}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{59.2}                                                                           & \multicolumn{1}{c|}{48.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{72.1}                                                                     & \multicolumn{1}{c|}{51.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{71.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.3}                                    \\ \hline
5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{50.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{52.1}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.6}}                                    & \multicolumn{1}{c|}{53.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{77.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.4}}                                    & \multicolumn{1}{c|}{55.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{79.3}                                    \\ \hline
5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.3}                                                                            & \multicolumn{1}{c|}{62.8}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{87.7}                                                                     & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{48.9}                                                                                   & \multicolumn{1}{c|}{79.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                    & \multicolumn{1}{c|}{54.9}                                                                            & \multicolumn{1}{c|}{58.8}                                                                           & \multicolumn{1}{c|}{48.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.2}                                    \\ \hline
5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{51}                                                                              & \multicolumn{1}{c|}{71.1}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                     & \multicolumn{1}{c|}{87.6}                                                                     & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{76.4}                                                                     & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.4}                                    \\ \hline
5000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{54.6}                                                                            & \multicolumn{1}{c|}{64.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.2}}                     & \multicolumn{1}{c|}{89.5}                                                                     & \multicolumn{1}{c|}{58.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82}}                                      & \multicolumn{1}{c|}{54.5}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.9}                                    \\ \hline
5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{46.5}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.7}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.1}}                                    & \multicolumn{1}{c|}{53.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
5000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{50.3}                                                                            & \multicolumn{1}{c|}{61.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{85.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{53.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{48.7}                                                                            & \multicolumn{1}{c|}{52.7}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80}}                       & \multicolumn{1}{c|}{77.3}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{72.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74.4}}                                    & \multicolumn{1}{c|}{51.2}                                                                            & \multicolumn{1}{c|}{54.2}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{72.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
8000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{86.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{49.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{78.2}                                                                     & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                       & 78.8                                                                     \\ \hline
8000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{56.9}                                                                            & \multicolumn{1}{c|}{52.6}                                                                           & \multicolumn{1}{c|}{55.8}                                                                                   & \multicolumn{1}{c|}{88.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                     & \multicolumn{1}{c|}{79.8}                                                                     & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{57.6}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.3}                                    \\ \hline
8000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{48.6}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                    & \multicolumn{1}{c|}{57.2}                                                                            & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{54.1}                                                                            & \multicolumn{1}{c|}{58.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.4}                                    \\ \hline
8000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{57.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                    & \multicolumn{1}{c|}{54.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
8000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{48.1}                                                                            & \multicolumn{1}{c|}{59.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                    & \multicolumn{1}{c|}{51.9}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{49.9}                                                                            & \multicolumn{1}{c|}{63.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{88}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                    & \multicolumn{1}{c|}{56.9}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                    & \multicolumn{1}{c|}{53.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{51}                                                                              & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{74.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.2}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{57.6}                                                                           & \multicolumn{1}{c|}{51.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{71.8}                                                                     & \multicolumn{1}{c|}{52}                                                                              & \multicolumn{1}{c|}{51.9}                                                                           & \multicolumn{1}{c|}{46.7}                                                                                   & \multicolumn{1}{c|}{71.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.3}                                    \\ \hline
10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{49}                                                                              & \multicolumn{1}{c|}{54.8}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{77.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                                    & \multicolumn{1}{c|}{52}                                                                              & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{86.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                                    & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{53.6}                                                                           & \multicolumn{1}{c|}{50.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.2}}                     & \multicolumn{1}{c|}{80.8}                                                                     & \multicolumn{1}{c|}{53}                                                                              & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.2}}                     & 81.2                                                                     \\ \hline
10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{51.7}                                                                            & \multicolumn{1}{c|}{57}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{60}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                     & \multicolumn{1}{c|}{80.5}                                                                     & \multicolumn{1}{c|}{54.4}                                                                            & \multicolumn{1}{c|}{58}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{82.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.1}                                    \\ \hline
10000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{53.7}                                                                            & \multicolumn{1}{c|}{74.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.9}}                                    & \multicolumn{1}{c|}{57.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                     & \multicolumn{1}{c|}{82.3}                                                                     & \multicolumn{1}{c|}{54.8}                                                                            & \multicolumn{1}{c|}{60.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.7}                                    \\ \hline
10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{61.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.3}}                                    & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83}}                                      & \multicolumn{1}{c|}{54.2}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.6}                                    \\ \hline
10000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{57.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.3}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{51.2}                                                                            & \multicolumn{1}{c|}{55.1}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{75.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                                    & \multicolumn{1}{c|}{54.7}                                                                            & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.8}}                     & \multicolumn{1}{c|}{71.6}                                                                     & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{54.3}                                                                           & \multicolumn{1}{c|}{46.4}                                                                                   & \multicolumn{1}{c|}{72.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.9}                                    \\ \hline
16000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{52.2}                                                                            & \multicolumn{1}{c|}{49.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{87}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{58.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.3}}                     & \multicolumn{1}{c|}{78.2}                                                                     & \multicolumn{1}{c|}{54.6}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{50.6}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{79.1}                                    \\ \hline
16000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{47.9}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{88.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                    & \multicolumn{1}{c|}{57.6}                                                                            & \multicolumn{1}{c|}{60.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                       & \multicolumn{1}{c|}{79.5}                                                                     & \multicolumn{1}{c|}{49.4}                                                                            & \multicolumn{1}{c|}{52.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.8}                                    \\ \hline
16000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{53}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                    & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{61.3}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{53.6}                                                                            & \multicolumn{1}{c|}{58.5}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{82}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{83.6}                                    \\ \hline
16000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{51.6}                                                                            & \multicolumn{1}{c|}{65.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{58.3}                                                                            & \multicolumn{1}{c|}{59.1}                                                                           & \multicolumn{1}{c|}{56.1}                                                                                   & \multicolumn{1}{c|}{83}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84}}                                      & \multicolumn{1}{c|}{52.4}                                                                            & \multicolumn{1}{c|}{60.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.7}                                    \\ \hline
16000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{74.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                    & \multicolumn{1}{c|}{57.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.7}}                                    & \multicolumn{1}{c|}{54.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{47.3}                                                                            & \multicolumn{1}{c|}{58.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.5}}                                    & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
\end{tabular}

\end{table*}

==> first_draft/tables/data_collection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Sound data collection comparison}\label{tab:datacollection}
\begin{tabular}{|cc|c|c|}
\hline
\multicolumn{2}{|c|}{Category} &
  \begin{tabular}[c]{@{}c@{}}Lab\\ (\textbf{IMI})\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Industry\\ (\textbf{KRPM})\end{tabular} \\ \hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}Machine\\ (Model, Manufacturer)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}3-axis Vertical Mill\\ (VM20i, Hurco)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}4-axis Horizontal Mill\\ (HCN-6000, Mazak)\end{tabular} \\ \hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}Working travel \\ in x$\times$y$\times$z in inch\end{tabular}} &
  40$\times$20$\times$20 &
  31.5$\times$31.5$\times$31.5 \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Max.\\ spindle \\ specification\end{tabular}}} &
  Torque &
  82.3 ft-lbs &
  442 ft-lbs \\ \cline{2-4} 
\multicolumn{1}{|c|}{} &
  \begin{tabular}[c]{@{}c@{}}Rotational \\ speed\end{tabular} &
  12,000 rpm &
  10,000 rpm \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} \\Sensor\\ (Location)\end{tabular}}} &
  0 &
  \begin{tabular}[c]{@{}c@{}}Microphone\\ (Working area)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Microphone\\ (Working area)\end{tabular} \\ \cline{2-4} 
\multicolumn{1}{|c|}{} &
  1 &
  \begin{tabular}[c]{@{}c@{}}ISS\\ (Near spindle)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}ISS\\ (Spindle)\end{tabular} \\ \cline{2-4} 
\multicolumn{1}{|c|}{} &
  2 &
  \begin{tabular}[c]{@{}c@{}}ISS\\ (Base)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}ISS\\ (Base)\end{tabular} \\ \hline
\multicolumn{2}{|c|}{Process} &
  Side milling &
  \begin{tabular}[c]{@{}c@{}}Side milling, facing, \\ drilling\end{tabular} \\ \hline
\multicolumn{2}{|c|}{Material} &
  \begin{tabular}[c]{@{}c@{}}AL6061, AISI4140, \\ AISI1018\end{tabular} &
  Cast iron \\ \hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}Total data length in second\\ (Cutting time)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}2789.97\\ (1032.97)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}130.27\\ (57.51)\end{tabular} \\ \hline
\end{tabular}
\end{table}

==> tables/RQ1_result_merged.tex <==
\begin{table}[tb]
\caption{RQ1- Performance Comparison of Different Features Transformations on each sensor}\label{tab:rq1_merged}
\centering
\begin{tabular}{|c|ccc|ccc|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Trans-}\\ \textbf{formation}\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\imi{}\\ Train (Validation) Accuracy\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\kirby{}\\ Train (Validation) Accuracy\end{tabular}} \\ \cline{2-7} 
 &
  \multicolumn{1}{c|}{Sensor0} &
  \multicolumn{1}{c|}{Sensor1} &
  Sensor2 &
  \multicolumn{1}{c|}{Sensor0} &
  \multicolumn{1}{c|}{Sensor1} &
  Sensor2 \\ \hline
$idx$ &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.696\\ (0.626)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.697\\ (0.628)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}0.628\\ (0.623)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.537\\ (0.551)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.523\\ (0.558)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}0.534\\ (0.544)\end{tabular} \\ \hline
$stanx$ &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{0.987}\\ (0.992)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{0.984}\\ (0.993)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\textbf{0.993}\\ (0.992)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.917\\ (0.786)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.916\\ (0.836)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}0.803\\ (0.544)\end{tabular} \\ \hline
$logx$ &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.676\\ (0.942)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.677\\ (0.972)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}0.941\\ (0.972)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.540\\ (0.541)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.527\\ (0.733)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}0.538\\ (0.727)\end{tabular} \\ \hline
$sigmoidx$ &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.951\\ (0.990)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.950\\ (0.992)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}0.990\\ (0.991)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.891\\ (0.820)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.860\\ (0.941)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}0.932\\ (0.821)\end{tabular} \\ \hline
$gammax$ &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.984\\ (\textbf{0.993})\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}0.983\\ (\textbf{0.994})\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\textbf{0.993}\\ (\textbf{0.993})\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{1.000}\\ (\textbf{0.914})\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{0.959}\\ (\textbf{0.952})\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\textbf{0.950}\\ (\textbf{0.883})\end{tabular} \\ \hline
\end{tabular}
\end{table}

==> tables/RQ1_results.tex <==
\begin{table}[hbtp]
\caption{RQ1- Performance Comparison of Different Features Transformations on separate sensors of \imi{}}\label{tab:rq1imi}
\centering
\begin{tabular}{|c|cccccc|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Trans-\\ formation\end{tabular}} & \multicolumn{3}{c|}{Train Accuracy}                                                                                                                                                                                         & \multicolumn{3}{c|}{Validation Accuracy}                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{}                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 1\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 2\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 1\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Sensor 2\end{tabular} \\ \hline
$idx$                                                               & \multicolumn{1}{c|}{0.696}                                              & \multicolumn{1}{c|}{0.697}                                              & \multicolumn{1}{c|}{0.628}                                              & \multicolumn{1}{c|}{0.626}                                              & \multicolumn{1}{c|}{0.628}                                              & 0.623                                              \\ \hline
$stanx$                                                             & \multicolumn{1}{c|}{\textbf{0.987}}                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.984}}             & \multicolumn{1}{c|}{\textbf{0.993}}                                     & \multicolumn{1}{c|}{0.992}                                              & \multicolumn{1}{c|}{0.993}                                              & 0.992                                              \\ \hline
$logx$                                                          & \multicolumn{1}{c|}{0.676}                                              & \multicolumn{1}{c|}{0.677}                                              & \multicolumn{1}{c|}{0.941}                                              & \multicolumn{1}{c|}{0.942}                                              & \multicolumn{1}{c|}{0.972}                                              & 0.972                                              \\ \hline
$sigmoidx$                                                      & \multicolumn{1}{c|}{0.951}                                              & \multicolumn{1}{c|}{0.95}                                               & \multicolumn{1}{c|}{0.99}                                               & \multicolumn{1}{c|}{0.99}                                               & \multicolumn{1}{c|}{0.992}                                              & 0.991                                              \\ \hline
$gammax$                                                        & \multicolumn{1}{c|}{0.984}                                              & \multicolumn{1}{c|}{0.983}                                              & \multicolumn{1}{c|}{\textbf{0.993}}                                     & \multicolumn{1}{c|}{\textbf{0.993}}                                     & \multicolumn{1}{c|}{\textbf{0.994}}                                     & \textbf{0.993}                                     \\ \hline
\end{tabular}
\end{table}

\begin{table}[hbtp]
\centering
\caption{RQ1- Performance Comparison of Different Features Transformations on separate sensors of \kirby{}}\label{tab:rq1kirby}
\begin{tabular}{|c|cccccc|}
\hline


\textbf{\begin{tabular}[c]{@{}c@{}}Trans-\\ formation\end{tabular}} & \multicolumn{3}{c|}{Train Accuracy}                                                                                                                                                                                         & \multicolumn{3}{c|}{Validation Accuracy}                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{}                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 1\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 2\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 0\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Sensor 1\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Sensor 2\end{tabular} \\ \hline
$idx$                                                               & \multicolumn{1}{c|}{0.537}                                              & \multicolumn{1}{c|}{0.523}                                              & \multicolumn{1}{c|}{0.534}                                              & \multicolumn{1}{c|}{0.551}                                              & \multicolumn{1}{c|}{0.558}                                              & 0.544                                              \\ \hline
$stanx$                                                             & \multicolumn{1}{c|}{0.917}                                              & \multicolumn{1}{c|}{0.916}                                              & \multicolumn{1}{c|}{0.803}                                              & \multicolumn{1}{c|}{0.786}                                              & \multicolumn{1}{c|}{0.836}                                              & 0.544                                              \\ \hline
$logx$                                                          & \multicolumn{1}{c|}{0.54}                                               & \multicolumn{1}{c|}{0.527}                                              & \multicolumn{1}{c|}{0.538}                                              & \multicolumn{1}{c|}{0.541}                                              & \multicolumn{1}{c|}{0.733}                                              & 0.727                                              \\ \hline
$sigmoidx$                                                      & \multicolumn{1}{c|}{0.892}                                              & \multicolumn{1}{c|}{0.86}                                               & \multicolumn{1}{c|}{0.932}                                              & \multicolumn{1}{c|}{0.82}                                               & \multicolumn{1}{c|}{0.941}                                              & 0.821                                              \\ \hline
$gammax$                                                        & \multicolumn{1}{c|}{\textbf{1}}                                         & \multicolumn{1}{c|}{\textbf{0.959}}                                     & \multicolumn{1}{c|}{\textbf{0.95}}                                      & \multicolumn{1}{c|}{\textbf{0.914}}                                     & \multicolumn{1}{c|}{\textbf{0.952}}                                     & \textbf{0.883}                                     \\ \hline
\end{tabular}
\end{table}

==> tables/RQ2_imi_sensor0.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[hbtp]
\begin{tabular}{|c|c|ccccc|}
\centering

\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\ Data \\ Size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\ Data\\ Size\end{tabular}} & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Target Test Accuracy for Kirby Sensor 0}}                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|l|}{\textbf{}}                                                    & \multicolumn{1}{l|}{\textbf{}}                                                  & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ Baseline\\ Single\\ Model\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ Baseline\\ Multi\\ Model\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Vanilla\\ Baseline\\ FineTuned\\ Model\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}ICIT-\\ ADV-DA\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}modified\\ ICIT-\\ ADV-DA\end{tabular}} \\ \hline
2000                                                                               & 50                                                                              & \multicolumn{1}{c|}{0.459}                                                                                & \multicolumn{1}{c|}{0.446}                                                                               & \multicolumn{1}{c|}{0.513}                                                                                   & \multicolumn{1}{c|}{0.773}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.791}                                     \\ \hline
2000                                                                               & 200                                                                             & \multicolumn{1}{c|}{0.439}                                                                                & \multicolumn{1}{c|}{0.44}                                                                                & \multicolumn{1}{c|}{0.448}                                                                                   & \multicolumn{1}{c|}{0.865}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.867}                                     \\ \hline
2000                                                                               & 500                                                                             & \multicolumn{1}{c|}{0.447}                                                                                & \multicolumn{1}{c|}{0.458}                                                                               & \multicolumn{1}{c|}{0.501}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.881}}                          & 0.874                                                                      \\ \hline
2000                                                                               & 1000                                                                            & \multicolumn{1}{c|}{0.452}                                                                                & \multicolumn{1}{c|}{0.524}                                                                               & \multicolumn{1}{c|}{0.545}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.889}}                          & 0.851                                                                      \\ \hline
2000                                                                               & 4000                                                                            & \multicolumn{1}{c|}{0.451}                                                                                & \multicolumn{1}{c|}{0.501}                                                                               & \multicolumn{1}{c|}{0.565}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.913}}                          & 0.89                                                                       \\ \hline
2000                                                                               & 10000                                                                           & \multicolumn{1}{c|}{0.453}                                                                                & \multicolumn{1}{c|}{0.563}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.93}}                           & 0.913                                                                      \\ \hline
2000                                                                               & 16000                                                                           & \multicolumn{1}{c|}{0.455}                                                                                & \multicolumn{1}{c|}{0.563}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.925}}                          & 0.916                                                                      \\ \hline
5000                                                                               & 50                                                                              & \multicolumn{1}{c|}{0.488}                                                                                & \multicolumn{1}{c|}{0.428}                                                                               & \multicolumn{1}{c|}{0.476}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.805}}                          & 0.784                                                                      \\ \hline
5000                                                                               & 200                                                                             & \multicolumn{1}{c|}{0.42}                                                                                 & \multicolumn{1}{c|}{0.452}                                                                               & \multicolumn{1}{c|}{0.47}                                                                                    & \multicolumn{1}{c|}{0.856}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.876}                                     \\ \hline
5000                                                                               & 500                                                                             & \multicolumn{1}{c|}{0.503}                                                                                & \multicolumn{1}{c|}{0.43}                                                                                & \multicolumn{1}{c|}{0.491}                                                                                   & \multicolumn{1}{c|}{0.876}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.884}                                     \\ \hline
5000                                                                               & 1000                                                                            & \multicolumn{1}{c|}{0.492}                                                                                & \multicolumn{1}{c|}{0.452}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.892}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.897}                                     \\ \hline
5000                                                                               & 4000                                                                            & \multicolumn{1}{c|}{0.445}                                                                                & \multicolumn{1}{c|}{0.502}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.906}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.911}                                     \\ \hline
5000                                                                               & 10000                                                                           & \multicolumn{1}{c|}{0.474}                                                                                & \multicolumn{1}{c|}{0.537}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.928}}                          & 0.916                                                                      \\ \hline
5000                                                                               & 16000                                                                           & \multicolumn{1}{c|}{0.499}                                                                                & \multicolumn{1}{c|}{0.498}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.93}}                           & 0.913                                                                      \\ \hline
8000                                                                               & 50                                                                              & \multicolumn{1}{c|}{0.445}                                                                                & \multicolumn{1}{c|}{0.407}                                                                               & \multicolumn{1}{c|}{0.461}                                                                                   & \multicolumn{1}{c|}{0.788}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.798}                                     \\ \hline
8000                                                                               & 200                                                                             & \multicolumn{1}{c|}{0.442}                                                                                & \multicolumn{1}{c|}{0.461}                                                                               & \multicolumn{1}{c|}{0.461}                                                                                   & \multicolumn{1}{c|}{0.851}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.874}                                     \\ \hline
8000                                                                               & 500                                                                             & \multicolumn{1}{c|}{0.452}                                                                                & \multicolumn{1}{c|}{0.48}                                                                                & \multicolumn{1}{c|}{0.497}                                                                                   & \multicolumn{1}{c|}{0.871}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.892}                                     \\ \hline
8000                                                                               & 1000                                                                            & \multicolumn{1}{c|}{0.418}                                                                                & \multicolumn{1}{c|}{0.441}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.9}}                            & 0.898                                                                      \\ \hline
8000                                                                               & 4000                                                                            & \multicolumn{1}{c|}{0.442}                                                                                & \multicolumn{1}{c|}{0.478}                                                                               & \multicolumn{1}{c|}{0.565}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.924}}                          & 0.912                                                                      \\ \hline
8000                                                                               & 10000                                                                           & \multicolumn{1}{c|}{0.447}                                                                                & \multicolumn{1}{c|}{0.497}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.93}}                           & 0.916                                                                      \\ \hline
8000                                                                               & 16000                                                                           & \multicolumn{1}{c|}{0.434}                                                                                & \multicolumn{1}{c|}{0.537}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.925}}                          & 0.919                                                                      \\ \hline
10000                                                                              & 50                                                                              & \multicolumn{1}{c|}{0.432}                                                                                & \multicolumn{1}{c|}{0.435}                                                                               & \multicolumn{1}{c|}{0.445}                                                                                   & \multicolumn{1}{c|}{0.788}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.799}                                     \\ \hline
10000                                                                              & 200                                                                             & \multicolumn{1}{c|}{0.475}                                                                                & \multicolumn{1}{c|}{0.477}                                                                               & \multicolumn{1}{c|}{0.444}                                                                                   & \multicolumn{1}{c|}{0.84}                                                            & \cellcolor[HTML]{FFFFFF}\textbf{0.874}                                     \\ \hline
10000                                                                              & 500                                                                             & \multicolumn{1}{c|}{0.497}                                                                                & \multicolumn{1}{c|}{0.457}                                                                               & \multicolumn{1}{c|}{0.521}                                                                                   & \multicolumn{1}{c|}{0.868}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.887}                                     \\ \hline
10000                                                                              & 1000                                                                            & \multicolumn{1}{c|}{0.434}                                                                                & \multicolumn{1}{c|}{0.445}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.901}}                          & \cellcolor[HTML]{FFFFFF}\textbf{0.901}                                     \\ \hline
10000                                                                              & 4000                                                                            & \multicolumn{1}{c|}{0.482}                                                                                & \multicolumn{1}{c|}{0.505}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.888}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.92}                                      \\ \hline
10000                                                                              & 10000                                                                           & \multicolumn{1}{c|}{0.436}                                                                                & \multicolumn{1}{c|}{0.478}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.905}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.924}                                     \\ \hline
10000                                                                              & 16000                                                                           & \multicolumn{1}{c|}{0.45}                                                                                 & \multicolumn{1}{c|}{0.516}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.904}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.919}                                     \\ \hline
16000                                                                              & 50                                                                              & \multicolumn{1}{c|}{0.45}                                                                                 & \multicolumn{1}{c|}{0.418}                                                                               & \multicolumn{1}{c|}{0.505}                                                                                   & \multicolumn{1}{c|}{0.797}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.798}                                     \\ \hline
16000                                                                              & 200                                                                             & \multicolumn{1}{c|}{0.448}                                                                                & \multicolumn{1}{c|}{0.49}                                                                                & \multicolumn{1}{c|}{0.486}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.876}}                          & 0.874                                                                      \\ \hline
16000                                                                              & 500                                                                             & \multicolumn{1}{c|}{0.437}                                                                                & \multicolumn{1}{c|}{0.442}                                                                               & \multicolumn{1}{c|}{0.519}                                                                                   & \multicolumn{1}{c|}{0.879}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.893}                                     \\ \hline
16000                                                                              & 1000                                                                            & \multicolumn{1}{c|}{0.435}                                                                                & \multicolumn{1}{c|}{0.448}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.897}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.899}                                     \\ \hline
16000                                                                              & 4000                                                                            & \multicolumn{1}{c|}{0.439}                                                                                & \multicolumn{1}{c|}{0.457}                                                                               & \multicolumn{1}{c|}{0.565}                                                                                   & \multicolumn{1}{c|}{0.914}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.916}                                     \\ \hline
16000                                                                              & 10000                                                                           & \multicolumn{1}{c|}{0.448}                                                                                & \multicolumn{1}{c|}{0.519}                                                                               & \multicolumn{1}{c|}{0.563}                                                                                   & \multicolumn{1}{c|}{0.912}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.922}                                     \\ \hline
16000                                                                              & 16000                                                                           & \multicolumn{1}{c|}{0.443}                                                                                & \multicolumn{1}{c|}{0.521}                                                                               & \multicolumn{1}{c|}{0.565}                                                                                   & \multicolumn{1}{c|}{0.901}                                                           & \cellcolor[HTML]{FFFFFF}\textbf{0.913}                                     \\ \hline
\end{tabular}
\end{table}

==> tables/RQ2_imi_sensor_0_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[htbp]
\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{0}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens0}


\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
                                                                                            &                                                                                          & \multicolumn{15}{c|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Target Test Accuracy for Kirby (in \%)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \cline{3-17} 
                                                                                            &                                                                                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 0}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 2}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{3-17} 
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\Data Size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\Data Size\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{} \end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular} \\ \hline
2000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{45.9}                                                                            & \multicolumn{1}{c|}{44.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{77.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.1}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{45.8}                                                                           & \multicolumn{1}{c|}{49.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.8}}                     & \multicolumn{1}{c|}{72.5}                                                                     & \multicolumn{1}{c|}{43.3}                                                                            & \multicolumn{1}{c|}{44}                                                                             & \multicolumn{1}{c|}{46.9}                                                                                   & \multicolumn{1}{c|}{73.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{74.2}                                    \\ \hline
2000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{44}                                                                             & \multicolumn{1}{c|}{44.8}                                                                                   & \multicolumn{1}{c|}{86.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.7}}                                    & \multicolumn{1}{c|}{43.8}                                                                            & \multicolumn{1}{c|}{46.9}                                                                           & \multicolumn{1}{c|}{48.8}                                                                                   & \multicolumn{1}{c|}{79.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.7}}                                    & \multicolumn{1}{c|}{43.3}                                                                            & \multicolumn{1}{c|}{43.7}                                                                           & \multicolumn{1}{c|}{50.3}                                                                                   & \multicolumn{1}{c|}{78.5}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{78.9}                                    \\ \hline
2000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{44.7}                                                                            & \multicolumn{1}{c|}{45.8}                                                                           & \multicolumn{1}{c|}{50.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.1}}                     & \multicolumn{1}{c|}{87.4}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{47.2}                                                                           & \multicolumn{1}{c|}{53.4}                                                                                   & \multicolumn{1}{c|}{77}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{49.2}                                                                           & \multicolumn{1}{c|}{48.6}                                                                                   & \multicolumn{1}{c|}{79.5}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{80.2}                                    \\ \hline
2000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{45.2}                                                                            & \multicolumn{1}{c|}{52.4}                                                                           & \multicolumn{1}{c|}{54.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{85.1}                                                                     & \multicolumn{1}{c|}{47.1}                                                                            & \multicolumn{1}{c|}{50.8}                                                                           & \multicolumn{1}{c|}{59.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.8}}                     & \multicolumn{1}{c|}{77.5}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{49.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{78.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{78.7}                                    \\ \hline
2000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{45.1}                                                                            & \multicolumn{1}{c|}{50.1}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                     & \multicolumn{1}{c|}{89}                                                                       & \multicolumn{1}{c|}{43.3}                                                                            & \multicolumn{1}{c|}{54.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{48.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.8}                                    \\ \hline
2000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{45.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{93}}                       & \multicolumn{1}{c|}{91.3}                                                                     & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.5}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
2000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{45.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.5}}                     & \multicolumn{1}{c|}{91.6}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.5}                                    \\ \hline
5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{48.8}                                                                            & \multicolumn{1}{c|}{42.8}                                                                           & \multicolumn{1}{c|}{47.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{78.4}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{47.2}                                                                           & \multicolumn{1}{c|}{43.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.6}}                     & \multicolumn{1}{c|}{72.2}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{45.7}                                                                           & \multicolumn{1}{c|}{43.7}                                                                                   & \multicolumn{1}{c|}{73.5}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.7}                                    \\ \hline
5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{42}                                                                              & \multicolumn{1}{c|}{45.2}                                                                           & \multicolumn{1}{c|}{47}                                                                                     & \multicolumn{1}{c|}{85.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.6}}                                    & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{43.9}                                                                           & \multicolumn{1}{c|}{46.3}                                                                                   & \multicolumn{1}{c|}{77}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.6}}                                    & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{43.8}                                                                           & \multicolumn{1}{c|}{46.4}                                                                                   & \multicolumn{1}{c|}{78.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79.1}                                    \\ \hline
5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{50.3}                                                                            & \multicolumn{1}{c|}{43}                                                                             & \multicolumn{1}{c|}{49.1}                                                                                   & \multicolumn{1}{c|}{87.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.4}}                                    & \multicolumn{1}{c|}{46.9}                                                                            & \multicolumn{1}{c|}{44.1}                                                                           & \multicolumn{1}{c|}{48.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.6}}                     & \multicolumn{1}{c|}{79.5}                                                                     & \multicolumn{1}{c|}{46.1}                                                                            & \multicolumn{1}{c|}{46.1}                                                                           & \multicolumn{1}{c|}{48.1}                                                                                   & \multicolumn{1}{c|}{81.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.6}                                    \\ \hline
5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{49.2}                                                                            & \multicolumn{1}{c|}{45.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                    & \multicolumn{1}{c|}{46.7}                                                                            & \multicolumn{1}{c|}{47.8}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{78.5}                                                      & \multicolumn{1}{c|}{79.5}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{43.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.2}                                    \\ \hline
5000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{44.5}                                                                            & \multicolumn{1}{c|}{50.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.1}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{51.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{81.4}                                                                     & \multicolumn{1}{c|}{46.1}                                                                            & \multicolumn{1}{c|}{50.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.1}}                     & 80.7                                                                     \\ \hline
5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{47.4}                                                                            & \multicolumn{1}{c|}{53.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.8}}                     & \multicolumn{1}{c|}{91.6}                                                                     & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{53.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.6}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
5000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{49.9}                                                                            & \multicolumn{1}{c|}{49.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{93}}                       & \multicolumn{1}{c|}{91.3}                                                                     & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{51.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.6}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{53.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
8000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{44.5}                                                                            & \multicolumn{1}{c|}{40.7}                                                                           & \multicolumn{1}{c|}{46.1}                                                                                   & \multicolumn{1}{c|}{78.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.8}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{43.9}                                                                           & \multicolumn{1}{c|}{46.6}                                                                                   & \multicolumn{1}{c|}{71.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.8}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{43.8}                                                                           & \multicolumn{1}{c|}{48.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.1}}                     & 72                                                                       \\ \hline
8000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{44.2}                                                                            & \multicolumn{1}{c|}{46.1}                                                                           & \multicolumn{1}{c|}{46.1}                                                                                   & \multicolumn{1}{c|}{85.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{49.9}                                                                           & \multicolumn{1}{c|}{46.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{77.9}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{47.2}                                                                           & \multicolumn{1}{c|}{45.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.2}}                     & 78.9                                                                     \\ \hline
8000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.2}                                                                            & \multicolumn{1}{c|}{48}                                                                             & \multicolumn{1}{c|}{49.7}                                                                                   & \multicolumn{1}{c|}{87.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{44}                                                                             & \multicolumn{1}{c|}{53.6}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{80.5}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{48}                                                                             & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.1}                                    \\ \hline
8000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{41.8}                                                                            & \multicolumn{1}{c|}{44.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90}}                       & \multicolumn{1}{c|}{89.8}                                                                     & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{45.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.2}}                                    & \multicolumn{1}{c|}{43.4}                                                                            & \multicolumn{1}{c|}{43.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.9}                                    \\ \hline
8000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{44.2}                                                                            & \multicolumn{1}{c|}{47.8}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.4}}                     & \multicolumn{1}{c|}{91.2}                                                                     & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{52.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.2}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{52.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
8000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{44.7}                                                                            & \multicolumn{1}{c|}{49.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{93}}                       & \multicolumn{1}{c|}{91.6}                                                                     & \multicolumn{1}{c|}{46.5}                                                                            & \multicolumn{1}{c|}{52.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{53.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{43.4}                                                                            & \multicolumn{1}{c|}{53.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.5}}                     & \multicolumn{1}{c|}{91.9}                                                                     & \multicolumn{1}{c|}{46}                                                                              & \multicolumn{1}{c|}{48.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{43.2}                                                                            & \multicolumn{1}{c|}{43.5}                                                                           & \multicolumn{1}{c|}{44.5}                                                                                   & \multicolumn{1}{c|}{78.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{46}                                                                             & \multicolumn{1}{c|}{44}                                                                                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74}}                       & \multicolumn{1}{c|}{71.7}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{46.3}                                                                           & \multicolumn{1}{c|}{50.8}                                                                                   & \multicolumn{1}{c|}{72.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{47.5}                                                                            & \multicolumn{1}{c|}{47.7}                                                                           & \multicolumn{1}{c|}{44.4}                                                                                   & \multicolumn{1}{c|}{84}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{44.2}                                                                           & \multicolumn{1}{c|}{48.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.2}}                     & \multicolumn{1}{c|}{76.7}                                                                     & \multicolumn{1}{c|}{46.4}                                                                            & \multicolumn{1}{c|}{43.4}                                                                           & \multicolumn{1}{c|}{43.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                       & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{49.7}                                                                            & \multicolumn{1}{c|}{45.7}                                                                           & \multicolumn{1}{c|}{52.1}                                                                                   & \multicolumn{1}{c|}{86.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{48.5}                                                                           & \multicolumn{1}{c|}{49.4}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{81}                                                                       & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{54.1}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.2}                                    \\ \hline
10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{43.4}                                                                            & \multicolumn{1}{c|}{44.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                    & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{46.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81}                                                        & \multicolumn{1}{c|}{81.1}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{43.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.5}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.3}                                    \\ \hline
10000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{50.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92}}                                      & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{46.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                     & \multicolumn{1}{c|}{81.9}                                                                     & \multicolumn{1}{c|}{46.1}                                                                            & \multicolumn{1}{c|}{46.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.6}                                    \\ \hline
10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{43.6}                                                                            & \multicolumn{1}{c|}{47.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.4}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{54.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{52.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
10000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{45}                                                                              & \multicolumn{1}{c|}{51.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{54}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{83.1}                                                                     & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{54.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
16000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{45}                                                                              & \multicolumn{1}{c|}{41.8}                                                                           & \multicolumn{1}{c|}{50.5}                                                                                   & \multicolumn{1}{c|}{79.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.8}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{44.1}                                                                           & \multicolumn{1}{c|}{44.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.5}}                     & \multicolumn{1}{c|}{72.3}                                                                     & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{44.8}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{73.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.9}                                    \\ \hline
16000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{44.8}                                                                            & \multicolumn{1}{c|}{49}                                                                             & \multicolumn{1}{c|}{48.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.6}}                     & \multicolumn{1}{c|}{87.4}                                                                     & \multicolumn{1}{c|}{44.7}                                                                            & \multicolumn{1}{c|}{48.2}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{77.7}                                                      & \multicolumn{1}{c|}{\textbf{77.9}}                                                                     & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{43.7}                                                                           & \multicolumn{1}{c|}{48.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.3}}                     & 78.7                                                                     \\ \hline
16000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{44.2}                                                                           & \multicolumn{1}{c|}{51.9}                                                                                   & \multicolumn{1}{c|}{87.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.3}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{46.3}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.3}}                     & \multicolumn{1}{c|}{79.7}                                                                     & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{46.7}                                                                           & \multicolumn{1}{c|}{51.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.8}}                     & 81.1                                                                     \\ \hline
16000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{43.5}                                                                            & \multicolumn{1}{c|}{44.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.9}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{44.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{48.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.6}                                    \\ \hline
16000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{45.7}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{91.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                    & \multicolumn{1}{c|}{43.9}                                                                            & \multicolumn{1}{c|}{54.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.9}}                                    & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{49.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.9}}                     & 82.2                                                                     \\ \hline
16000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{44.8}                                                                            & \multicolumn{1}{c|}{51.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{91.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.2}}                                    & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{51.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.2}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{53.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
16000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{44.3}                                                                            & \multicolumn{1}{c|}{52.1}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{90.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                    & \multicolumn{1}{c|}{44}                                                                              & \multicolumn{1}{c|}{50.7}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.7}}                                    & \multicolumn{1}{c|}{43.7}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
\end{tabular}
\end{table*}

==> tables/RQ2_imi_sensor_0_reduced.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{0}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens0_reduced}
\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
\multirow{3}{*}{ \begin{tabular}[c]{@{}c@{}}\\Source\\
%Labeled\\
Data Size\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\\Target\\
  %Labeled\\
  Data Size\end{tabular}} &
  \multicolumn{15}{c|}{Target Test Accuracy for \kirby{} in \%} \\ \cline{3-17} 
 &
   &
  \multicolumn{5}{c|}{Sensor 0} &
  \multicolumn{5}{c|}{Sensor 1} &
  \multicolumn{5}{c|}{Sensor 2} \\ \cline{3-17} 
 &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BSM}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BMM}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BFM}\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{FARADAy}} &
  \multicolumn{1}{c|}{\textbf{DIRAC}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BSM}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BMM}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BFM}\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{FARADAy}} &
  \multicolumn{1}{c|}{\textbf{DIRAC}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BSM}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BMM}\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Vanilla}\\ \textbf{BFM}\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{FARADAy}} &
  \textbf{DIRAC} \\ \hline
2,000 &
  50 &
  \multicolumn{1}{c|}{45.9} &
  \multicolumn{1}{c|}{44.6} &
  \multicolumn{1}{c|}{51.3} &
  \multicolumn{1}{c|}{77.3} &
  \multicolumn{1}{c|}{\textbf{79.1}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{45.8} &
  \multicolumn{1}{c|}{49.7} &
  \multicolumn{1}{c|}{\textbf{72.8}} &
  \multicolumn{1}{c|}{72.5} &
  \multicolumn{1}{c|}{43.3} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{46.9} &
  \multicolumn{1}{c|}{73.4} &
  \textbf{74.2} \\ \hline
2,000 &
  500 &
  \multicolumn{1}{c|}{44.7} &
  \multicolumn{1}{c|}{45.8} &
  \multicolumn{1}{c|}{50.1} &
  \multicolumn{1}{c|}{\textbf{88.1}} &
  \multicolumn{1}{c|}{87.4} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{47.2} &
  \multicolumn{1}{c|}{53.4} &
  \multicolumn{1}{c|}{77.0} &
  \multicolumn{1}{c|}{\textbf{80.5}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{49.2} &
  \multicolumn{1}{c|}{48.6} &
  \multicolumn{1}{c|}{79.5} &
  \textbf{80.2} \\ \hline
2,000 &
  4,000 &
  \multicolumn{1}{c|}{45.1} &
  \multicolumn{1}{c|}{50.1} &
  \multicolumn{1}{c|}{56.5} &
  \multicolumn{1}{c|}{\textbf{91.3}} &
  \multicolumn{1}{c|}{89.0} &
  \multicolumn{1}{c|}{43.3} &
  \multicolumn{1}{c|}{54.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.8} &
  \multicolumn{1}{c|}{\textbf{81.9}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{48.4} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.7} &
  \textbf{82.8} \\ \hline
2,000 &
  12,213 &
  \multicolumn{1}{c|}{45.5} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{\textbf{92.5}} &
  \multicolumn{1}{c|}{91.6} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.7} &
  \multicolumn{1}{c|}{\textbf{82.9}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{81.1} &
  \textbf{84.5} \\ \hline
8,000 &
  50 &
  \multicolumn{1}{c|}{44.5} &
  \multicolumn{1}{c|}{40.7} &
  \multicolumn{1}{c|}{46.1} &
  \multicolumn{1}{c|}{78.8} &
  \multicolumn{1}{c|}{\textbf{79.8}} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{43.9} &
  \multicolumn{1}{c|}{46.6} &
  \multicolumn{1}{c|}{71.4} &
  \multicolumn{1}{c|}{\textbf{73.8}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{43.8} &
  \multicolumn{1}{c|}{48.5} &
  \multicolumn{1}{c|}{\textbf{73.1}} &
  72.0 \\ \hline
8,000 &
  500 &
  \multicolumn{1}{c|}{45.2} &
  \multicolumn{1}{c|}{48.0} &
  \multicolumn{1}{c|}{49.7} &
  \multicolumn{1}{c|}{87.1} &
  \multicolumn{1}{c|}{\textbf{89.2}} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{53.6} &
  \multicolumn{1}{c|}{80.1} &
  \multicolumn{1}{c|}{\textbf{80.5}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{48.0} &
  \multicolumn{1}{c|}{51.3} &
  \multicolumn{1}{c|}{81.8} &
  \textbf{82.1} \\ \hline
8,000 &
  4,000 &
  \multicolumn{1}{c|}{44.2} &
  \multicolumn{1}{c|}{47.8} &
  \multicolumn{1}{c|}{56.5} &
  \multicolumn{1}{c|}{\textbf{92.4}} &
  \multicolumn{1}{c|}{91.2} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{52.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{81.6} &
  \multicolumn{1}{c|}{\textbf{83.2}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{52.2} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{83.1} &
  \textbf{84.2} \\ \hline
8,000 &
  12,213 &
  \multicolumn{1}{c|}{43.4} &
  \multicolumn{1}{c|}{53.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{\textbf{92.5}} &
  \multicolumn{1}{c|}{91.9} &
  \multicolumn{1}{c|}{46.0} &
  \multicolumn{1}{c|}{48.8} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.2} &
  \multicolumn{1}{c|}{\textbf{82.9}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.2} &
  \textbf{84.9} \\ \hline
16,000 &
  50 &
  \multicolumn{1}{c|}{45.0} &
  \multicolumn{1}{c|}{41.8} &
  \multicolumn{1}{c|}{50.5} &
  \multicolumn{1}{c|}{79.7} &
  \multicolumn{1}{c|}{\textbf{79.8}} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{44.4} &
  \multicolumn{1}{c|}{\textbf{73.5}} &
  \multicolumn{1}{c|}{72.3} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{44.8} &
  \multicolumn{1}{c|}{51.3} &
  \multicolumn{1}{c|}{73.6} &
  \textbf{73.9} \\ \hline
16,000 &
  500 &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{44.2} &
  \multicolumn{1}{c|}{51.9} &
  \multicolumn{1}{c|}{87.9} &
  \multicolumn{1}{c|}{\textbf{89.3}} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{46.3} &
  \multicolumn{1}{c|}{51.4} &
  \multicolumn{1}{c|}{\textbf{80.3}} &
  \multicolumn{1}{c|}{79.7} &
  \multicolumn{1}{c|}{48.2} &
  \multicolumn{1}{c|}{46.7} &
  \multicolumn{1}{c|}{51.8} &
  \multicolumn{1}{c|}{\textbf{81.8}} &
  81.1 \\ \hline
16,000 &
  4,000 &
  \multicolumn{1}{c|}{43.9} &
  \multicolumn{1}{c|}{45.7} &
  \multicolumn{1}{c|}{56.5} &
  \multicolumn{1}{c|}{91.4} &
  \multicolumn{1}{c|}{\textbf{91.6}} &
  \multicolumn{1}{c|}{43.9} &
  \multicolumn{1}{c|}{54.5} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{82.7} &
  \multicolumn{1}{c|}{\textbf{83.9}} &
  \multicolumn{1}{c|}{46.3} &
  \multicolumn{1}{c|}{49.2} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{\textbf{83.9}} &
  82.2 \\ \hline
16,000 &
  12,213 &
  \multicolumn{1}{c|}{44.3} &
  \multicolumn{1}{c|}{52.1} &
  \multicolumn{1}{c|}{56.5} &
  \multicolumn{1}{c|}{90.1} &
  \multicolumn{1}{c|}{\textbf{91.3}} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{50.7} &
  \multicolumn{1}{c|}{56.4} &
  \multicolumn{1}{c|}{82.1} &
  \multicolumn{1}{c|}{\textbf{83.7}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{60.6} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{83.3} &
  \textbf{85.0} \\ \hline
\end{tabular}
\end{table*}



==> tables/RQ2_imi_sensor_0_reduced_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{RQ2- Target Test Accuracy (in \%) Comparison among transfer learning models with \imi{} Sensor $\textbf{0}$ as Source, \& \kirby{} sensors as Target, with varying data size}
\label{tab:rq2sens0_reduced}
\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}\\ Target Sensor\\ Index $\rightarrow$\end{tabular}} &
\multicolumn{5}{c|}{Sensor 0} &
  \multicolumn{5}{c|}{Sensor 1} &
  \multicolumn{5}{c|}{Sensor 2} 
  
  %\multicolumn{15}{c|}{k} 
  \\ \cline{1-17} 
  
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}\\ Model \\ $\rightarrow$\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}}
  &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}}
  
  
  \\ 
  \cline{1-2} 
 {\begin{tabular}[c]{@{}c@{}}\\ Source\\Labeled\\Data\\Size $\downarrow$\\\  \end{tabular}}
 &  {\begin{tabular}[c]{@{}c@{}}\\ Target\\Labeled\\Data\\Size$\downarrow$\\\  \end{tabular}}
   & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &
   \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &
   \multicolumn{1}{c|}{}
   
   %\multicolumn{15}{c|}{k} 
   \\ \hline
2,000 &
  50 &
  \multicolumn{1}{c|}{45.9} &
  \multicolumn{1}{c|}{44.6} &
  \multicolumn{1}{c|}{51.3} &
  \multicolumn{1}{c|}{77.3} &
  \multicolumn{1}{c|}{\textbf{79.1}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{45.8} &
  \multicolumn{1}{c|}{49.7} &
  \multicolumn{1}{c|}{\textbf{72.8}} &
  \multicolumn{1}{c|}{72.5} &
  \multicolumn{1}{c|}{43.3} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{46.9} &
  \multicolumn{1}{c|}{73.4} &
  \textbf{74.2} \\ \hline
2,000 &
  500 &
  \multicolumn{1}{c|}{44.7} &
  \multicolumn{1}{c|}{45.8} &
  \multicolumn{1}{c|}{50.1} &
  \multicolumn{1}{c|}{\textbf{88.1}} &
  \multicolumn{1}{c|}{87.4} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{47.2} &
  \multicolumn{1}{c|}{53.4} &
  \multicolumn{1}{c|}{77.0} &
  \multicolumn{1}{c|}{\textbf{80.5}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{49.2} &
  \multicolumn{1}{c|}{48.6} &
  \multicolumn{1}{c|}{79.5} &
  \textbf{80.2} \\ \hline
2,000 &
  4,000 &
  \multicolumn{1}{c|}{45.1} &
  \multicolumn{1}{c|}{50.1} &
  \multicolumn{1}{c|}{56.5} &
  \multicolumn{1}{c|}{\textbf{91.3}} &
  \multicolumn{1}{c|}{89.0} &
  \multicolumn{1}{c|}{43.3} &
  \multicolumn{1}{c|}{54.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.8} &
  \multicolumn{1}{c|}{\textbf{81.9}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{48.4} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.7} &
  \textbf{82.8} \\ \hline
2,000 &
  12,213 &
  \multicolumn{1}{c|}{45.5} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{\textbf{92.5}} &
  \multicolumn{1}{c|}{91.6} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.7} &
  \multicolumn{1}{c|}{\textbf{82.9}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{81.1} &
  \textbf{84.5} \\ \hline
8,000 &
  50 &
  \multicolumn{1}{c|}{44.5} &
  \multicolumn{1}{c|}{40.7} &
  \multicolumn{1}{c|}{46.1} &
  \multicolumn{1}{c|}{78.8} &
  \multicolumn{1}{c|}{\textbf{79.8}} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{43.9} &
  \multicolumn{1}{c|}{46.6} &
  \multicolumn{1}{c|}{71.4} &
  \multicolumn{1}{c|}{\textbf{73.8}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{43.8} &
  \multicolumn{1}{c|}{48.5} &
  \multicolumn{1}{c|}{\textbf{73.1}} &
  72.0 \\ \hline
8,000 &
  500 &
  \multicolumn{1}{c|}{45.2} &
  \multicolumn{1}{c|}{48.0} &
  \multicolumn{1}{c|}{49.7} &
  \multicolumn{1}{c|}{87.1} &
  \multicolumn{1}{c|}{\textbf{89.2}} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{53.6} &
  \multicolumn{1}{c|}{80.1} &
  \multicolumn{1}{c|}{\textbf{80.5}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{48.0} &
  \multicolumn{1}{c|}{51.3} &
  \multicolumn{1}{c|}{81.8} &
  \textbf{82.1} \\ \hline
8,000 &
  4,000 &
  \multicolumn{1}{c|}{44.2} &
  \multicolumn{1}{c|}{47.8} &
  \multicolumn{1}{c|}{56.5} &
  \multicolumn{1}{c|}{\textbf{92.4}} &
  \multicolumn{1}{c|}{91.2} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{52.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{81.6} &
  \multicolumn{1}{c|}{\textbf{83.2}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{52.2} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{83.1} &
  \textbf{84.2} \\ \hline
8,000 &
  12,213 &
  \multicolumn{1}{c|}{43.4} &
  \multicolumn{1}{c|}{53.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{\textbf{92.5}} &
  \multicolumn{1}{c|}{91.9} &
  \multicolumn{1}{c|}{46.0} &
  \multicolumn{1}{c|}{48.8} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.2} &
  \multicolumn{1}{c|}{\textbf{82.9}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{80.2} &
  \textbf{84.9} \\ \hline
16,000 &
  50 &
  \multicolumn{1}{c|}{45.0} &
  \multicolumn{1}{c|}{41.8} &
  \multicolumn{1}{c|}{50.5} &
  \multicolumn{1}{c|}{79.7} &
  \multicolumn{1}{c|}{\textbf{79.8}} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{44.4} &
  \multicolumn{1}{c|}{\textbf{73.5}} &
  \multicolumn{1}{c|}{72.3} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{44.8} &
  \multicolumn{1}{c|}{51.3} &
  \multicolumn{1}{c|}{73.6} &
  \textbf{73.9} \\ \hline
16,000 &
  500 &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{44.2} &
  \multicolumn{1}{c|}{51.9} &
  \multicolumn{1}{c|}{87.9} &
  \multicolumn{1}{c|}{\textbf{89.3}} &
  \multicolumn{1}{c|}{44.1} &
  \multicolumn{1}{c|}{46.3} &
  \multicolumn{1}{c|}{51.4} &
  \multicolumn{1}{c|}{\textbf{80.3}} &
  \multicolumn{1}{c|}{79.7} &
  \multicolumn{1}{c|}{48.2} &
  \multicolumn{1}{c|}{46.7} &
  \multicolumn{1}{c|}{51.8} &
  \multicolumn{1}{c|}{\textbf{81.8}} &
  81.1 \\ \hline
16,000 &
  4,000 &
  \multicolumn{1}{c|}{43.9} &
  \multicolumn{1}{c|}{45.7} &
  \multicolumn{1}{c|}{56.5} &
  \multicolumn{1}{c|}{91.4} &
  \multicolumn{1}{c|}{\textbf{91.6}} &
  \multicolumn{1}{c|}{43.9} &
  \multicolumn{1}{c|}{54.5} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{82.7} &
  \multicolumn{1}{c|}{\textbf{83.9}} &
  \multicolumn{1}{c|}{46.3} &
  \multicolumn{1}{c|}{49.2} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{\textbf{83.9}} &
  82.2 \\ \hline
16,000 &
  12,213 &
  \multicolumn{1}{c|}{44.3} &
  \multicolumn{1}{c|}{52.1} &
  \multicolumn{1}{c|}{56.5} &
  \multicolumn{1}{c|}{90.1} &
  \multicolumn{1}{c|}{\textbf{91.3}} &
  \multicolumn{1}{c|}{44.0} &
  \multicolumn{1}{c|}{50.7} &
  \multicolumn{1}{c|}{56.4} &
  \multicolumn{1}{c|}{82.1} &
  \multicolumn{1}{c|}{\textbf{83.7}} &
  \multicolumn{1}{c|}{43.7} &
  \multicolumn{1}{c|}{60.6} &
  \multicolumn{1}{c|}{56.3} &
  \multicolumn{1}{c|}{83.3} &
  \textbf{85.0} \\ \hline
\end{tabular}
\end{table*}

==> tables/RQ2_imi_sensor_1_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[hbtp]

\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{1}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens1}

\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
                                                                                            &                                                                                          & \multicolumn{15}{c|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Target Test Accuracy for Kirby(in \%)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \cline{3-17} 
                                                                                            &                                                                                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 0}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \cline{3-17} 
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\Data Size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\Data Size\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular} \\ \hline
 2000& 50& \multicolumn{1}{c|}{71.7} & \multicolumn{1}{c|}{64.9}& \multicolumn{1}{c|}{62.9} & \multicolumn{1}{c|}{78} & \multicolumn{1}{c|}{79.4}& \multicolumn{1}{c|}{56.1}& \multicolumn{1}{c|}{56.2} & \multicolumn{1}{c|}{53.8}& \multicolumn{1}{c|}{72.8} & \multicolumn{1}{c|}{75} & \multicolumn{1}{c|}{56.7}& \multicolumn{1}{c|}{54.3} & \multicolumn{1}{c|}{53.5} & \multicolumn{1}{c|}{75.3} & \multicolumn{1}{c|}{73.7}\\ \hline
2000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{61.9}                                                                           & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.4}}                     & \multicolumn{1}{c|}{86.3}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{49.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.5}}                     & \multicolumn{1}{c|}{79.4}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                                                      & 76.7                                                                     \\ \hline
2000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{69}                                                                             & \multicolumn{1}{c|}{61.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.4}}                     & \multicolumn{1}{c|}{82.6}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{53.9}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{79.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{80.2}                                    \\ \hline
2000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{74.2}                                                                            & \multicolumn{1}{c|}{68.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.8}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{76.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{56.9}                                                                                   & \multicolumn{1}{c|}{77.8}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
2000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{71.8}                                                                            & \multicolumn{1}{c|}{67.7}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.6}}                     & \multicolumn{1}{c|}{88.5}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.6}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.9}                                                                           & \multicolumn{1}{c|}{57.3}                                                                                   & \multicolumn{1}{c|}{81.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.8}                                    \\ \hline
2000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{75.2}                                                                            & \multicolumn{1}{c|}{61.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.6}}                                                                     & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81}                                                                                         & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
2000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{73.6}                                                                            & \multicolumn{1}{c|}{67.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.5}}                                                                     & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{67.6}                                                                            & \multicolumn{1}{c|}{70.6}                                                                           & \multicolumn{1}{c|}{50.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.9}}                     & \multicolumn{1}{c|}{79.2}                                                                                                      & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72}}                       & \multicolumn{1}{c|}{71.9}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{73.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{65.6}                                                                           & \multicolumn{1}{c|}{53.6}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.7}                                                                           & \multicolumn{1}{c|}{53.2}                                                                                   & \multicolumn{1}{c|}{76.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                                                                       & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{77.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{78.8}                                    \\ \hline
5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{67.7}                                                                            & \multicolumn{1}{c|}{66}                                                                             & \multicolumn{1}{c|}{55.8}                                                                                   & \multicolumn{1}{c|}{88}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.5}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                                      & 79.8                                                                     \\ \hline
5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{63.5}                                                                            & \multicolumn{1}{c|}{67.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.6}}                     & \multicolumn{1}{c|}{89.4}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80}}                       & \multicolumn{1}{c|}{78.3}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{79.7}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{81.9}                                    \\ \hline
5000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{62.7}                                                                            & \multicolumn{1}{c|}{71.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.2}}                     & \multicolumn{1}{c|}{90.1}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.1}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.5}                                    \\ \hline
5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{64.4}                                                                            & \multicolumn{1}{c|}{69.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84}                                      \\ \hline
5000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{63.5}                                                                            & \multicolumn{1}{c|}{74.9}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.4}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
8000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{71.8}                                                                            & \multicolumn{1}{c|}{70.9}                                                                           & \multicolumn{1}{c|}{50.5}                                                                                   & \multicolumn{1}{c|}{77.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                                                                       & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{70.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.2}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{55.8}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{71.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{73.7}                                    \\ \hline
8000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{66.3}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{44.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.5}}                     & \multicolumn{1}{c|}{87.2}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{51.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{78.1}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{51.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.2}}                                                      & 78.9                                                                     \\ \hline
8000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{60.8}                                                                            & \multicolumn{1}{c|}{64.4}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{88.8}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{57}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.4}}                     & \multicolumn{1}{c|}{80.3}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{81.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{81.4}                                    \\ \hline
8000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{64.9}                                                                            & \multicolumn{1}{c|}{68}                                                                             & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{88.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{81.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83.1}                                    \\ \hline
8000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{61}                                                                              & \multicolumn{1}{c|}{80.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.5}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{76.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                                                     & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.5}                                    \\ \hline
8000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{59.8}                                                                            & \multicolumn{1}{c|}{81}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
8000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{67.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.8}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{64.3}                                                                            & \multicolumn{1}{c|}{65.6}                                                                           & \multicolumn{1}{c|}{50.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{78.9}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{50.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{71.6}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{72.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{74}                                      \\ \hline
10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{71.2}                                                                            & \multicolumn{1}{c|}{67}                                                                             & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{87}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.2}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{48.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                     & \multicolumn{1}{c|}{77.8}                                                                                                      & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.8}}                                                      & 78.7                                                                     \\ \hline
10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{67.7}                                                                            & \multicolumn{1}{c|}{62.9}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{88.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.4}}                                                                     & \multicolumn{1}{c|}{55.8}                                                                            & \multicolumn{1}{c|}{57.5}                                                                           & \multicolumn{1}{c|}{53.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                       & \multicolumn{1}{c|}{80}                                                                                                        & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{80.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.4}                                    \\ \hline
10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{64.8}                                                                            & \multicolumn{1}{c|}{69.6}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.4}}                                                                     & \multicolumn{1}{c|}{55.9}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                                                                       & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.7}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83}                                      \\ \hline
10000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{70.3}                                                                            & \multicolumn{1}{c|}{79.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{57.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{81.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.7}                                    \\ \hline
10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{60.2}                                                                            & \multicolumn{1}{c|}{75.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{91.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                                                     & \multicolumn{1}{c|}{54.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.9}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
10000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{63.6}                                                                            & \multicolumn{1}{c|}{75}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92}}                                                                       & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.1}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{62.7}                                                                            & \multicolumn{1}{c|}{68.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.8}}                     & \multicolumn{1}{c|}{78.7}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{54.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.6}}                     & \multicolumn{1}{c|}{72.5}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.8}}                                                      & 73.4                                                                     \\ \hline
16000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{64}                                                                              & \multicolumn{1}{c|}{59.4}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{86.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87}}                                                                       & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                     & \multicolumn{1}{c|}{78}                                                                                                        & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{55.4}                                                                           & \multicolumn{1}{c|}{49.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                                                      & 78.6                                                                     \\ \hline
16000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{67.2}                                                                            & \multicolumn{1}{c|}{62.8}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{87.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{77.4}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{54}                                                                             & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{81.8}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.3}                                    \\ \hline
16000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{59.6}                                                                            & \multicolumn{1}{c|}{69.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{82}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{82.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83.4}                                    \\ \hline
16000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{67.6}                                                                            & \multicolumn{1}{c|}{79.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.2}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.2}}                                                                     & \multicolumn{1}{c|}{55.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{84}                                                                                         & \cellcolor[HTML]{FFFFFF}\textbf{85.1}                                    \\ \hline
16000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{65.7}                                                                            & \multicolumn{1}{c|}{82}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.4}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.8}}                                                                     & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
16000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{59.7}                                                                            & \multicolumn{1}{c|}{79.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.4}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.6}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
\end{tabular}

\end{table*}

==> tables/RQ2_imi_sensor_1_reduced.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[hbtp]

\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{1}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens1_reduced}

\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
                                                                                            &                                                                                          & \multicolumn{15}{c|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Target Test Accuracy for Kirby(in \%)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \cline{3-17} 
                                                                                            &                                                                                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 0}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \cline{3-17} 
 \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\Data Size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\Data Size\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular} \\ \hline
 2,000& 50& \multicolumn{1}{c|}{71.7} & \multicolumn{1}{c|}{64.9}& \multicolumn{1}{c|}{62.9} & \multicolumn{1}{c|}{78} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.4}}& \multicolumn{1}{c|}{56.1}& \multicolumn{1}{c|}{56.2} & \multicolumn{1}{c|}{53.8}& \multicolumn{1}{c|}{72.8} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{75}} & \multicolumn{1}{c|}{56.7}& \multicolumn{1}{c|}{54.3} & \multicolumn{1}{c|}{53.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{75.3}} & \multicolumn{1}{c|}{73.7}\\ \hline
%2,000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{61.9}                                                                           & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.4}}                     & \multicolumn{1}{c|}{86.3}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{49.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.5}}                     & \multicolumn{1}{c|}{79.4}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                                                      & 76.7                                                                     \\ \hline
2,000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{69}                                                                             & \multicolumn{1}{c|}{61.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.4}}                     & \multicolumn{1}{c|}{82.6}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{53.9}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{79.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{80.2}                                    \\ \hline
%2,000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{74.2}                                                                            & \multicolumn{1}{c|}{68.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.8}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{76.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{56.9}                                                                                   & \multicolumn{1}{c|}{77.8}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
2,000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{71.8}                                                                            & \multicolumn{1}{c|}{67.7}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.6}}                     & \multicolumn{1}{c|}{88.5}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.6}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.9}                                                                           & \multicolumn{1}{c|}{57.3}                                                                                   & \multicolumn{1}{c|}{81.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.8}                                    \\ \hline
%2,000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{75.2}                                                                            & \multicolumn{1}{c|}{61.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.6}}                                                                     & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81}                                                                                         & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
2,000                                                                                        & 12,213                                                                                   & \multicolumn{1}{c|}{73.6}                                                                            & \multicolumn{1}{c|}{67.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.5}}                                                                     & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
%5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{67.6}                                                                            & \multicolumn{1}{c|}{70.6}                                                                           & \multicolumn{1}{c|}{50.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.9}}                     & \multicolumn{1}{c|}{79.2}                                                                                                      & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72}}                       & \multicolumn{1}{c|}{71.9}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{73.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
%5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{65.6}                                                                           & \multicolumn{1}{c|}{53.6}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.7}                                                                           & \multicolumn{1}{c|}{53.2}                                                                                   & \multicolumn{1}{c|}{76.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                                                                       & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{77.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{78.8}                                    \\ \hline
%5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{67.7}                                                                            & \multicolumn{1}{c|}{66}                                                                             & \multicolumn{1}{c|}{55.8}                                                                                   & \multicolumn{1}{c|}{88}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.5}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                                      & 79.8                                                                     \\ \hline
%5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{63.5}                                                                            & \multicolumn{1}{c|}{67.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.6}}                     & \multicolumn{1}{c|}{89.4}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80}}                       & \multicolumn{1}{c|}{78.3}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{79.7}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{81.9}                                    \\ \hline
%5000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{62.7}                                                                            & \multicolumn{1}{c|}{71.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.2}}                     & \multicolumn{1}{c|}{90.1}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.1}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.5}                                    \\ \hline
%5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{64.4}                                                                            & \multicolumn{1}{c|}{69.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84}                                      \\ \hline
%5000                                                                                        & 16,000                                                                                    & \multicolumn{1}{c|}{63.5}                                                                            & \multicolumn{1}{c|}{74.9}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.4}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
8,000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{71.8}                                                                            & \multicolumn{1}{c|}{70.9}                                                                           & \multicolumn{1}{c|}{50.5}                                                                                   & \multicolumn{1}{c|}{77.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                                                                       & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{70.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.2}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{55.8}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{71.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{73.7}                                    \\ \hline
%8,000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{66.3}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{44.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.5}}                     & \multicolumn{1}{c|}{87.2}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{51.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{78.1}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{51.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.2}}                                                      & 78.9                                                                     \\ \hline
8,000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{60.8}                                                                            & \multicolumn{1}{c|}{64.4}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{88.8}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{57}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.4}}                     & \multicolumn{1}{c|}{80.3}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{81.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{81.4}                                    \\ \hline
%8,000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{64.9}                                                                            & \multicolumn{1}{c|}{68}                                                                             & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{88.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{81.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83.1}                                    \\ \hline
8,000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{61}                                                                              & \multicolumn{1}{c|}{80.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.5}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{76.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                                                     & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.5}                                    \\ \hline
%8,000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{59.8}                                                                            & \multicolumn{1}{c|}{81}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
8,000                                                                                        & 12,213                                                                                    & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{67.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.8}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
%10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{64.3}                                                                            & \multicolumn{1}{c|}{65.6}                                                                           & \multicolumn{1}{c|}{50.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{78.9}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{50.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{71.6}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{72.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{74}                                      \\ \hline
%10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{71.2}                                                                            & \multicolumn{1}{c|}{67}                                                                             & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{87}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.2}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{48.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                     & \multicolumn{1}{c|}{77.8}                                                                                                      & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.8}}                                                      & 78.7                                                                     \\ \hline
%10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{67.7}                                                                            & \multicolumn{1}{c|}{62.9}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{88.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.4}}                                                                     & \multicolumn{1}{c|}{55.8}                                                                            & \multicolumn{1}{c|}{57.5}                                                                           & \multicolumn{1}{c|}{53.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                       & \multicolumn{1}{c|}{80}                                                                                                        & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{80.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.4}                                    \\ \hline
%10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{64.8}                                                                            & \multicolumn{1}{c|}{69.6}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.4}}                                                                     & \multicolumn{1}{c|}{55.9}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                                                                       & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.7}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83}                                      \\ \hline
%10000                                                                                       & 4,000                                                                                     & \multicolumn{1}{c|}{70.3}                                                                            & \multicolumn{1}{c|}{79.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{57.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{81.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.7}                                    \\ \hline
%10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{60.2}                                                                            & \multicolumn{1}{c|}{75.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{91.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                                                     & \multicolumn{1}{c|}{54.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.9}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
%10000                                                                                       & 16,000                                                                                    & \multicolumn{1}{c|}{63.6}                                                                            & \multicolumn{1}{c|}{75}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92}}                                                                       & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.1}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16,000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{62.7}                                                                            & \multicolumn{1}{c|}{68.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.8}}                     & \multicolumn{1}{c|}{78.7}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{54.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.6}}                     & \multicolumn{1}{c|}{72.5}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.8}}                                                      & 73.4                                                                     \\ \hline
%16,000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{64}                                                                              & \multicolumn{1}{c|}{59.4}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{86.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87}}                                                                       & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                     & \multicolumn{1}{c|}{78}                                                                                                        & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{55.4}                                                                           & \multicolumn{1}{c|}{49.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                                                      & 78.6                                                                     \\ \hline
16,000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{67.2}                                                                            & \multicolumn{1}{c|}{62.8}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{87.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{77.4}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{54}                                                                             & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{81.8}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.3}                                    \\ \hline
%16,000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{59.6}                                                                            & \multicolumn{1}{c|}{69.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{82}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{82.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83.4}                                    \\ \hline
16,000                                                                                       & 4,000                                                                                     & \multicolumn{1}{c|}{67.6}                                                                            & \multicolumn{1}{c|}{79.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.2}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.2}}                                                                     & \multicolumn{1}{c|}{55.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{84}                                                                                         & \cellcolor[HTML]{FFFFFF}\textbf{85.1}                                    \\ \hline
%16,000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{65.7}                                                                            & \multicolumn{1}{c|}{82}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.4}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.8}}                                                                     & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
16,000                                                                                       & 12,213                                                                                    & \multicolumn{1}{c|}{59.7}                                                                            & \multicolumn{1}{c|}{79.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.4}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.6}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
\end{tabular}

\end{table*}

==> tables/RQ2_imi_sensor_1_reduced_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[hbtp]

\centering
\caption{RQ2- Target Test Accuracy (in \%) Comparison among transfer learning models with \imi{} Sensor $\textbf{1}$ as Source, \& \kirby{} sensors as Target, with varying data size}
\label{tab:rq2sens1_reduced}

\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}\\ Target Sensor\\ Index $\rightarrow$\end{tabular}} &
\multicolumn{5}{c|}{Sensor 0} &
  \multicolumn{5}{c|}{Sensor 1} &
  \multicolumn{5}{c|}{Sensor 2} 
  
  %\multicolumn{15}{c|}{k} 
  \\ \cline{1-17} 
  
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}\\ Model \\ $\rightarrow$\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}}
  &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}}
  
  
  \\ 
  \cline{1-2} 
 {\begin{tabular}[c]{@{}c@{}}\\ Source\\Labeled\\Data\\Size $\downarrow$\\\  \end{tabular}}
 &  {\begin{tabular}[c]{@{}c@{}}\\ Target\\Labeled\\Data\\Size$\downarrow$\\\  \end{tabular}}
   & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &
   \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &
   \multicolumn{1}{c|}{}
   
   %\multicolumn{15}{c|}{k} 
   \\ \hline
 2,000& 50& \multicolumn{1}{c|}{71.7} & \multicolumn{1}{c|}{64.9}& \multicolumn{1}{c|}{62.9} & \multicolumn{1}{c|}{78} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.4}}& \multicolumn{1}{c|}{56.1}& \multicolumn{1}{c|}{56.2} & \multicolumn{1}{c|}{53.8}& \multicolumn{1}{c|}{72.8} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{75}} & \multicolumn{1}{c|}{56.7}& \multicolumn{1}{c|}{54.3} & \multicolumn{1}{c|}{53.5} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{75.3}} & \multicolumn{1}{c|}{73.7}\\ \hline
%2,000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{61.9}                                                                           & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.4}}                     & \multicolumn{1}{c|}{86.3}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{49.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.5}}                     & \multicolumn{1}{c|}{79.4}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                                                      & 76.7                                                                     \\ \hline
2,000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{69}                                                                             & \multicolumn{1}{c|}{61.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.4}}                     & \multicolumn{1}{c|}{82.6}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{53.9}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{79.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{80.2}                                    \\ \hline
%2,000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{74.2}                                                                            & \multicolumn{1}{c|}{68.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.8}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{76.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{56.9}                                                                                   & \multicolumn{1}{c|}{77.8}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
2,000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{71.8}                                                                            & \multicolumn{1}{c|}{67.7}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.6}}                     & \multicolumn{1}{c|}{88.5}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.6}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.9}                                                                           & \multicolumn{1}{c|}{57.3}                                                                                   & \multicolumn{1}{c|}{81.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.8}                                    \\ \hline
%2,000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{75.2}                                                                            & \multicolumn{1}{c|}{61.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.6}}                                                                     & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81}                                                                                         & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
2,000                                                                                        & 12,213                                                                                   & \multicolumn{1}{c|}{73.6}                                                                            & \multicolumn{1}{c|}{67.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.5}}                                                                     & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
%5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{67.6}                                                                            & \multicolumn{1}{c|}{70.6}                                                                           & \multicolumn{1}{c|}{50.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.9}}                     & \multicolumn{1}{c|}{79.2}                                                                                                      & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72}}                       & \multicolumn{1}{c|}{71.9}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{73.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
%5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{65.6}                                                                           & \multicolumn{1}{c|}{53.6}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.7}                                                                           & \multicolumn{1}{c|}{53.2}                                                                                   & \multicolumn{1}{c|}{76.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                                                                       & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{77.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{78.8}                                    \\ \hline
%5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{67.7}                                                                            & \multicolumn{1}{c|}{66}                                                                             & \multicolumn{1}{c|}{55.8}                                                                                   & \multicolumn{1}{c|}{88}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.5}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                                      & 79.8                                                                     \\ \hline
%5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{63.5}                                                                            & \multicolumn{1}{c|}{67.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.6}}                     & \multicolumn{1}{c|}{89.4}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80}}                       & \multicolumn{1}{c|}{78.3}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{79.7}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{81.9}                                    \\ \hline
%5000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{62.7}                                                                            & \multicolumn{1}{c|}{71.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.2}}                     & \multicolumn{1}{c|}{90.1}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.1}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.5}                                    \\ \hline
%5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{64.4}                                                                            & \multicolumn{1}{c|}{69.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84}                                      \\ \hline
%5000                                                                                        & 16,000                                                                                    & \multicolumn{1}{c|}{63.5}                                                                            & \multicolumn{1}{c|}{74.9}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.4}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
8,000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{71.8}                                                                            & \multicolumn{1}{c|}{70.9}                                                                           & \multicolumn{1}{c|}{50.5}                                                                                   & \multicolumn{1}{c|}{77.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                                                                       & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{70.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.2}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{55.8}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{71.5}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{73.7}                                    \\ \hline
%8,000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{66.3}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{44.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.5}}                     & \multicolumn{1}{c|}{87.2}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{51.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{78.1}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{51.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.2}}                                                      & 78.9                                                                     \\ \hline
8,000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{60.8}                                                                            & \multicolumn{1}{c|}{64.4}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{88.8}                                                                                                      & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{57}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.4}}                     & \multicolumn{1}{c|}{80.3}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{81.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{81.4}                                    \\ \hline
%8,000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{64.9}                                                                            & \multicolumn{1}{c|}{68}                                                                             & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{88.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{81.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83.1}                                    \\ \hline
8,000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{61}                                                                              & \multicolumn{1}{c|}{80.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.5}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{76.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                                                     & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.5}                                    \\ \hline
%8,000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{59.8}                                                                            & \multicolumn{1}{c|}{81}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
8,000                                                                                        & 12,213                                                                                    & \multicolumn{1}{c|}{67}                                                                              & \multicolumn{1}{c|}{67.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{80.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.8}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
%10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{64.3}                                                                            & \multicolumn{1}{c|}{65.6}                                                                           & \multicolumn{1}{c|}{50.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{78.9}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{50.6}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{71.6}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{72.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{74}                                      \\ \hline
%10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{71.2}                                                                            & \multicolumn{1}{c|}{67}                                                                             & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{87}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.2}}                                                                     & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{48.4}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                     & \multicolumn{1}{c|}{77.8}                                                                                                      & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.8}}                                                      & 78.7                                                                     \\ \hline
%10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{67.7}                                                                            & \multicolumn{1}{c|}{62.9}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{88.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.4}}                                                                     & \multicolumn{1}{c|}{55.8}                                                                            & \multicolumn{1}{c|}{57.5}                                                                           & \multicolumn{1}{c|}{53.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                       & \multicolumn{1}{c|}{80}                                                                                                        & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{80.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.4}                                    \\ \hline
%10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{64.8}                                                                            & \multicolumn{1}{c|}{69.6}                                                                           & \multicolumn{1}{c|}{56.6}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.4}}                                                                     & \multicolumn{1}{c|}{55.9}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                                                                       & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.7}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83}                                      \\ \hline
%10000                                                                                       & 4,000                                                                                     & \multicolumn{1}{c|}{70.3}                                                                            & \multicolumn{1}{c|}{79.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{57.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{81.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.7}                                    \\ \hline
%10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{60.2}                                                                            & \multicolumn{1}{c|}{75.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{91.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                                                     & \multicolumn{1}{c|}{54.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{82.9}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
%10000                                                                                       & 16,000                                                                                    & \multicolumn{1}{c|}{63.6}                                                                            & \multicolumn{1}{c|}{75}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92}}                                                                       & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.1}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16,000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{62.7}                                                                            & \multicolumn{1}{c|}{68.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.8}}                     & \multicolumn{1}{c|}{78.7}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{54.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.6}}                     & \multicolumn{1}{c|}{72.5}                                                                                                      & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{73.8}}                                                      & 73.4                                                                     \\ \hline
%16,000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{64}                                                                              & \multicolumn{1}{c|}{59.4}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{86.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87}}                                                                       & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                     & \multicolumn{1}{c|}{78}                                                                                                        & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{55.4}                                                                           & \multicolumn{1}{c|}{49.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.7}}                                                      & 78.6                                                                     \\ \hline
16,000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{67.2}                                                                            & \multicolumn{1}{c|}{62.8}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{87.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{55.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{77.4}                                                                                                      & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{54}                                                                             & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{81.8}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{82.3}                                    \\ \hline
%16,000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{59.6}                                                                            & \multicolumn{1}{c|}{69.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{82}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{82.3}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{83.4}                                    \\ \hline
16,000                                                                                       & 4,000                                                                                     & \multicolumn{1}{c|}{67.6}                                                                            & \multicolumn{1}{c|}{79.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.2}}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.2}}                                                                     & \multicolumn{1}{c|}{55.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{84}                                                                                         & \cellcolor[HTML]{FFFFFF}\textbf{85.1}                                    \\ \hline
%16,000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{65.7}                                                                            & \multicolumn{1}{c|}{82}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.4}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.8}}                                                                     & \multicolumn{1}{c|}{56}                                                                              & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
16,000                                                                                       & 12,213                                                                                    & \multicolumn{1}{c|}{59.7}                                                                            & \multicolumn{1}{c|}{79.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.4}}                                                                     & \multicolumn{1}{c|}{56.1}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.6}}                                                                     & \multicolumn{1}{c|}{56.6}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.2}                                                                                       & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
\end{tabular}

\end{table*}

==> tables/RQ2_imi_sensor_2_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[htbp]

\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{2}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens2}

\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
                                                                                            &                                                                                          & \multicolumn{15}{c|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Target Test Accuracy for Kirby(in \%)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \cline{3-17} 
                                                                                            &                                                                                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 0}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 2}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{3-17} 
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\Data Size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\Data Size\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular} \\
 2000& 50& 0.495& 0.537& 0.503& 0.798& 0.797& 0.584& 0.576& 0.525& 0.716& 0.729& 0.527& 0.523& 0.531& 0.74&0.741\\ \hline

2000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{45.4}                                                                            & \multicolumn{1}{c|}{57.3}                                                                           & \multicolumn{1}{c|}{56.8}                                                                                   & \multicolumn{1}{c|}{85.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.3}}                                    & \multicolumn{1}{c|}{58.6}                                                                            & \multicolumn{1}{c|}{57.7}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{78.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78}}                       & 77.7                                                                     \\ \hline
2000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.4}                                                                            & \multicolumn{1}{c|}{57.3}                                                                           & \multicolumn{1}{c|}{55.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.6}}                     & \multicolumn{1}{c|}{88.5}                                                                     & \multicolumn{1}{c|}{58.1}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{55.2}                                                                                   & \multicolumn{1}{c|}{78.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.3}}                                    & \multicolumn{1}{c|}{51.6}                                                                            & \multicolumn{1}{c|}{58.6}                                                                           & \multicolumn{1}{c|}{58.7}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79.3}                                    \\ \hline
2000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{59.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                     & \multicolumn{1}{c|}{88.5}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{58.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{77.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{52.8}                                                                            & \multicolumn{1}{c|}{55.8}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{78.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{78.6}                                    \\ \hline
2000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{47}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                     & \multicolumn{1}{c|}{89.1}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.6}}                                    & \multicolumn{1}{c|}{52.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.7}                                    \\ \hline
2000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{44.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{57.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{52.7}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56}                                                                                     & \multicolumn{1}{c|}{80.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
2000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{45.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.7}}                                    & \multicolumn{1}{c|}{58.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.9}}                                    & \multicolumn{1}{c|}{53.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{49.3}                                                                           & \multicolumn{1}{c|}{56.1}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{59.2}                                                                           & \multicolumn{1}{c|}{48.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{72.1}                                                                     & \multicolumn{1}{c|}{51.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{71.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.3}                                    \\ \hline
5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{50.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{52.1}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.6}}                                    & \multicolumn{1}{c|}{53.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{77.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.4}}                                    & \multicolumn{1}{c|}{55.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{79.3}                                    \\ \hline
5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.3}                                                                            & \multicolumn{1}{c|}{62.8}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{87.7}                                                                     & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{48.9}                                                                                   & \multicolumn{1}{c|}{79.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                    & \multicolumn{1}{c|}{54.9}                                                                            & \multicolumn{1}{c|}{58.8}                                                                           & \multicolumn{1}{c|}{48.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.2}                                    \\ \hline
5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{51}                                                                              & \multicolumn{1}{c|}{71.1}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                     & \multicolumn{1}{c|}{87.6}                                                                     & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{76.4}                                                                     & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.4}                                    \\ \hline
5000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{54.6}                                                                            & \multicolumn{1}{c|}{64.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.2}}                     & \multicolumn{1}{c|}{89.5}                                                                     & \multicolumn{1}{c|}{58.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82}}                                      & \multicolumn{1}{c|}{54.5}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.9}                                    \\ \hline
5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{46.5}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.7}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.1}}                                    & \multicolumn{1}{c|}{53.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
5000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{50.3}                                                                            & \multicolumn{1}{c|}{61.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{85.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{53.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{48.7}                                                                            & \multicolumn{1}{c|}{52.7}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80}}                       & \multicolumn{1}{c|}{77.3}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{72.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74.4}}                                    & \multicolumn{1}{c|}{51.2}                                                                            & \multicolumn{1}{c|}{54.2}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{72.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
8000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{86.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{49.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{78.2}                                                                     & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                       & 78.8                                                                     \\ \hline
8000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{56.9}                                                                            & \multicolumn{1}{c|}{52.6}                                                                           & \multicolumn{1}{c|}{55.8}                                                                                   & \multicolumn{1}{c|}{88.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                     & \multicolumn{1}{c|}{79.8}                                                                     & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{57.6}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.3}                                    \\ \hline
8000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{48.6}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                    & \multicolumn{1}{c|}{57.2}                                                                            & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{54.1}                                                                            & \multicolumn{1}{c|}{58.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.4}                                    \\ \hline
8000                                                                                        & 4000                                                                                     & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{57.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                    & \multicolumn{1}{c|}{54.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
8000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{48.1}                                                                            & \multicolumn{1}{c|}{59.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                    & \multicolumn{1}{c|}{51.9}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8000                                                                                        & 16000                                                                                    & \multicolumn{1}{c|}{49.9}                                                                            & \multicolumn{1}{c|}{63.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{88}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                    & \multicolumn{1}{c|}{56.9}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                    & \multicolumn{1}{c|}{53.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{51}                                                                              & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{74.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.2}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{57.6}                                                                           & \multicolumn{1}{c|}{51.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{71.8}                                                                     & \multicolumn{1}{c|}{52}                                                                              & \multicolumn{1}{c|}{51.9}                                                                           & \multicolumn{1}{c|}{46.7}                                                                                   & \multicolumn{1}{c|}{71.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.3}                                    \\ \hline
10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{49}                                                                              & \multicolumn{1}{c|}{54.8}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{77.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                                    & \multicolumn{1}{c|}{52}                                                                              & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{86.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                                    & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{53.6}                                                                           & \multicolumn{1}{c|}{50.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.2}}                     & \multicolumn{1}{c|}{80.8}                                                                     & \multicolumn{1}{c|}{53}                                                                              & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.2}}                     & 81.2                                                                     \\ \hline
10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{51.7}                                                                            & \multicolumn{1}{c|}{57}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{60}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                     & \multicolumn{1}{c|}{80.5}                                                                     & \multicolumn{1}{c|}{54.4}                                                                            & \multicolumn{1}{c|}{58}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{82.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.1}                                    \\ \hline
10000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{53.7}                                                                            & \multicolumn{1}{c|}{74.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.9}}                                    & \multicolumn{1}{c|}{57.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                     & \multicolumn{1}{c|}{82.3}                                                                     & \multicolumn{1}{c|}{54.8}                                                                            & \multicolumn{1}{c|}{60.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.7}                                    \\ \hline
10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{61.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.3}}                                    & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83}}                                      & \multicolumn{1}{c|}{54.2}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.6}                                    \\ \hline
10000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{57.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.3}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{51.2}                                                                            & \multicolumn{1}{c|}{55.1}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{75.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                                    & \multicolumn{1}{c|}{54.7}                                                                            & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.8}}                     & \multicolumn{1}{c|}{71.6}                                                                     & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{54.3}                                                                           & \multicolumn{1}{c|}{46.4}                                                                                   & \multicolumn{1}{c|}{72.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.9}                                    \\ \hline
16000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{52.2}                                                                            & \multicolumn{1}{c|}{49.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{87}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{58.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.3}}                     & \multicolumn{1}{c|}{78.2}                                                                     & \multicolumn{1}{c|}{54.6}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{50.6}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{79.1}                                    \\ \hline
16000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{47.9}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{88.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                    & \multicolumn{1}{c|}{57.6}                                                                            & \multicolumn{1}{c|}{60.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                       & \multicolumn{1}{c|}{79.5}                                                                     & \multicolumn{1}{c|}{49.4}                                                                            & \multicolumn{1}{c|}{52.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.8}                                    \\ \hline
16000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{53}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                    & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{61.3}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{53.6}                                                                            & \multicolumn{1}{c|}{58.5}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{82}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{83.6}                                    \\ \hline
16000                                                                                       & 4000                                                                                     & \multicolumn{1}{c|}{51.6}                                                                            & \multicolumn{1}{c|}{65.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{58.3}                                                                            & \multicolumn{1}{c|}{59.1}                                                                           & \multicolumn{1}{c|}{56.1}                                                                                   & \multicolumn{1}{c|}{83}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84}}                                      & \multicolumn{1}{c|}{52.4}                                                                            & \multicolumn{1}{c|}{60.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.7}                                    \\ \hline
16000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{74.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                    & \multicolumn{1}{c|}{57.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.7}}                                    & \multicolumn{1}{c|}{54.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16000                                                                                       & 16000                                                                                    & \multicolumn{1}{c|}{47.3}                                                                            & \multicolumn{1}{c|}{58.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.5}}                                    & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
\end{tabular}

\end{table*}

==> tables/RQ2_imi_sensor_2_reduced.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[htbp]

\centering
\caption{RQ2- Comparison among transfer learning models with \imi{} Sensor $\textbf{2}$ as Source, \& \kirby{} as Target, with varying data size}
\label{tab:rq2sens2_reduced}

\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
                                                                                            &                                                                                          & \multicolumn{15}{c|}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Target Test Accuracy for Kirby(in \%)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \cline{3-17} 
                                                                                            &                                                                                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 0}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 1}                                                                                                                                                                                                                                                                                                                                                                                                                                                     & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Sensor 2}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{3-17} 
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Source \\ Labeled \\Data Size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Target\\ Labeled\\Data Size\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbstable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbmtable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\vbftable{}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\icittable{}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\icitmodtable{}\end{tabular} \\ \hline
 {2,000} & 50& \multicolumn{1}{c|}{49.5} & \multicolumn{1}{c|}{53.7} & \multicolumn{1}{c|}{50.3} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.8}} & \multicolumn{1}{c|}{79.7} & \multicolumn{1}{c|}{58.4} & \multicolumn{1}{c|}{57.6} & \multicolumn{1}{c|}{52.5} & \multicolumn{1}{c|}{71.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.9}} & \multicolumn{1}{c|}{52.7} & \multicolumn{1}{c|}{52.3} & \multicolumn{1}{c|}{53.1} & \multicolumn{1}{c|}{74.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74.1}}\\ 

%2,000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{45.4}                                                                            & \multicolumn{1}{c|}{57.3}                                                                           & \multicolumn{1}{c|}{56.8}                                                                                   & \multicolumn{1}{c|}{85.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.3}}                                    & \multicolumn{1}{c|}{58.6}                                                                            & \multicolumn{1}{c|}{57.7}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{78.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78}}                       & 77.7                                                                     \\ \hline
2,000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.4}                                                                            & \multicolumn{1}{c|}{57.3}                                                                           & \multicolumn{1}{c|}{55.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.6}}                     & \multicolumn{1}{c|}{88.5}                                                                     & \multicolumn{1}{c|}{58.1}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{55.2}                                                                                   & \multicolumn{1}{c|}{78.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.3}}                                    & \multicolumn{1}{c|}{51.6}                                                                            & \multicolumn{1}{c|}{58.6}                                                                           & \multicolumn{1}{c|}{58.7}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79.3}                                    \\ \hline
%2,000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{59.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                     & \multicolumn{1}{c|}{88.5}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{58.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{77.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{52.8}                                                                            & \multicolumn{1}{c|}{55.8}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{78.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{78.6}                                    \\ \hline
2,000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{47}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                     & \multicolumn{1}{c|}{89.1}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.6}}                                    & \multicolumn{1}{c|}{52.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.7}                                    \\ \hline
%2,000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{44.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{57.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{52.7}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56}                                                                                     & \multicolumn{1}{c|}{80.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
2,000                                                                                        & 12,213                                                                                    & \multicolumn{1}{c|}{45.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.7}}                                    & \multicolumn{1}{c|}{58.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.9}}                                    & \multicolumn{1}{c|}{53.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
%5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{49.3}                                                                           & \multicolumn{1}{c|}{56.1}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{59.2}                                                                           & \multicolumn{1}{c|}{48.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{72.1}                                                                     & \multicolumn{1}{c|}{51.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{71.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.3}                                    \\ \hline
%5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{50.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{52.1}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.6}}                                    & \multicolumn{1}{c|}{53.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{77.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.4}}                                    & \multicolumn{1}{c|}{55.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{79.3}                                    \\ \hline
%5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.3}                                                                            & \multicolumn{1}{c|}{62.8}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{87.7}                                                                     & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{48.9}                                                                                   & \multicolumn{1}{c|}{79.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                    & \multicolumn{1}{c|}{54.9}                                                                            & \multicolumn{1}{c|}{58.8}                                                                           & \multicolumn{1}{c|}{48.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.2}                                    \\ \hline
%5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{51}                                                                              & \multicolumn{1}{c|}{71.1}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                     & \multicolumn{1}{c|}{87.6}                                                                     & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{76.4}                                                                     & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.4}                                    \\ \hline
%5000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{54.6}                                                                            & \multicolumn{1}{c|}{64.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.2}}                     & \multicolumn{1}{c|}{89.5}                                                                     & \multicolumn{1}{c|}{58.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82}}                                      & \multicolumn{1}{c|}{54.5}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.9}                                    \\ \hline
%5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{46.5}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.7}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.1}}                                    & \multicolumn{1}{c|}{53.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
%5000                                                                                        & 12,213                                                                                    & \multicolumn{1}{c|}{50.3}                                                                            & \multicolumn{1}{c|}{61.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{85.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{53.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8,000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{48.7}                                                                            & \multicolumn{1}{c|}{52.7}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80}}                       & \multicolumn{1}{c|}{77.3}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{72.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74.4}}                                    & \multicolumn{1}{c|}{51.2}                                                                            & \multicolumn{1}{c|}{54.2}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{72.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
%8,000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{86.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{49.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{78.2}                                                                     & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                       & 78.8                                                                     \\ \hline
8,000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{56.9}                                                                            & \multicolumn{1}{c|}{52.6}                                                                           & \multicolumn{1}{c|}{55.8}                                                                                   & \multicolumn{1}{c|}{88.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                     & \multicolumn{1}{c|}{79.8}                                                                     & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{57.6}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.3}                                    \\ \hline
%8,000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{48.6}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                    & \multicolumn{1}{c|}{57.2}                                                                            & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{54.1}                                                                            & \multicolumn{1}{c|}{58.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.4}                                    \\ \hline
8,000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{57.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                    & \multicolumn{1}{c|}{54.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
%8,000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{48.1}                                                                            & \multicolumn{1}{c|}{59.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                    & \multicolumn{1}{c|}{51.9}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8,000                                                                                        & 12,213                                                                                    & \multicolumn{1}{c|}{49.9}                                                                            & \multicolumn{1}{c|}{63.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{88}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                    & \multicolumn{1}{c|}{56.9}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                    & \multicolumn{1}{c|}{53.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
%10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{51}                                                                              & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{74.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.2}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{57.6}                                                                           & \multicolumn{1}{c|}{51.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{71.8}                                                                     & \multicolumn{1}{c|}{52}                                                                              & \multicolumn{1}{c|}{51.9}                                                                           & \multicolumn{1}{c|}{46.7}                                                                                   & \multicolumn{1}{c|}{71.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.3}                                    \\ \hline
%10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{49}                                                                              & \multicolumn{1}{c|}{54.8}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{77.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                                    & \multicolumn{1}{c|}{52}                                                                              & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
%10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{86.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                                    & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{53.6}                                                                           & \multicolumn{1}{c|}{50.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.2}}                     & \multicolumn{1}{c|}{80.8}                                                                     & \multicolumn{1}{c|}{53}                                                                              & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.2}}                     & 81.2                                                                     \\ \hline
%10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{51.7}                                                                            & \multicolumn{1}{c|}{57}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{60}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                     & \multicolumn{1}{c|}{80.5}                                                                     & \multicolumn{1}{c|}{54.4}                                                                            & \multicolumn{1}{c|}{58}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{82.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.1}                                    \\ \hline
%10000                                                                                       & 4,000                                                                                     & \multicolumn{1}{c|}{53.7}                                                                            & \multicolumn{1}{c|}{74.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.9}}                                    & \multicolumn{1}{c|}{57.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                     & \multicolumn{1}{c|}{82.3}                                                                     & \multicolumn{1}{c|}{54.8}                                                                            & \multicolumn{1}{c|}{60.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.7}                                    \\ \hline
%10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{61.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.3}}                                    & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83}}                                      & \multicolumn{1}{c|}{54.2}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.6}                                    \\ \hline
%10000                                                                                       & 12,213                                                                                    & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{57.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.3}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16,000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{51.2}                                                                            & \multicolumn{1}{c|}{55.1}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{75.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                                    & \multicolumn{1}{c|}{54.7}                                                                            & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.8}}                     & \multicolumn{1}{c|}{71.6}                                                                     & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{54.3}                                                                           & \multicolumn{1}{c|}{46.4}                                                                                   & \multicolumn{1}{c|}{72.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.9}                                    \\ \hline
%16,000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{52.2}                                                                            & \multicolumn{1}{c|}{49.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{87}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{58.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.3}}                     & \multicolumn{1}{c|}{78.2}                                                                     & \multicolumn{1}{c|}{54.6}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{50.6}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{79.1}                                    \\ \hline
16,000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{47.9}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{88.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                    & \multicolumn{1}{c|}{57.6}                                                                            & \multicolumn{1}{c|}{60.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                       & \multicolumn{1}{c|}{79.5}                                                                     & \multicolumn{1}{c|}{49.4}                                                                            & \multicolumn{1}{c|}{52.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.8}                                    \\ \hline
%16,000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{53}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                    & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{61.3}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{53.6}                                                                            & \multicolumn{1}{c|}{58.5}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{82}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{83.6}                                    \\ \hline
16,000                                                                                       & 4,000                                                                                     & \multicolumn{1}{c|}{51.6}                                                                            & \multicolumn{1}{c|}{65.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{58.3}                                                                            & \multicolumn{1}{c|}{59.1}                                                                           & \multicolumn{1}{c|}{56.1}                                                                                   & \multicolumn{1}{c|}{83}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84}}                                      & \multicolumn{1}{c|}{52.4}                                                                            & \multicolumn{1}{c|}{60.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.7}                                    \\ \hline
%16,000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{74.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                    & \multicolumn{1}{c|}{57.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.7}}                                    & \multicolumn{1}{c|}{54.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16,000                                                                                       & 12,213                                                                                    & \multicolumn{1}{c|}{47.3}                                                                            & \multicolumn{1}{c|}{58.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.5}}                                    & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
\end{tabular}

\end{table*}

==> tables/RQ2_imi_sensor_2_reduced_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[hbtp]

\centering
\caption{RQ2- Target Test Accuracy (in \%) Comparison among transfer learning models with \imi{} Sensor $\textbf{2}$ as Source, \& \kirby{} sensors as Target, with varying data size}
\label{tab:rq2sens1_reduced}

\begin{tabular}{|c|c|ccccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}\\ Target Sensor\\ Index $\rightarrow$\end{tabular}} &
\multicolumn{5}{c|}{Sensor 0} &
  \multicolumn{5}{c|}{Sensor 1} &
  \multicolumn{5}{c|}{Sensor 2} 
  
  %\multicolumn{15}{c|}{k} 
  \\ \cline{1-17} 
  
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}\\ Model \\ $\rightarrow$\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}}
  &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BSM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BMM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{Vanilla}\\ \textbf{BFM}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{FARADAy}\end{tabular}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \textbf{DIRAC}\end{tabular}}}
  
  
  \\ 
  \cline{1-2} 
 {\begin{tabular}[c]{@{}c@{}}\\ Source\\Labeled\\Data\\Size $\downarrow$\\\  \end{tabular}}
 &  {\begin{tabular}[c]{@{}c@{}}\\ Target\\Labeled\\Data\\Size$\downarrow$\\\  \end{tabular}}
   & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &
   \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &
   \multicolumn{1}{c|}{}
   
   %\multicolumn{15}{c|}{k} 
   \\ \hline
 {2,000} & 50& \multicolumn{1}{c|}{49.5} & \multicolumn{1}{c|}{53.7} & \multicolumn{1}{c|}{50.3} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.8}} & \multicolumn{1}{c|}{79.7} & \multicolumn{1}{c|}{58.4} & \multicolumn{1}{c|}{57.6} & \multicolumn{1}{c|}{52.5} & \multicolumn{1}{c|}{71.6} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.9}} & \multicolumn{1}{c|}{52.7} & \multicolumn{1}{c|}{52.3} & \multicolumn{1}{c|}{53.1} & \multicolumn{1}{c|}{74.0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74.1}}\\ \hline

%2,000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{45.4}                                                                            & \multicolumn{1}{c|}{57.3}                                                                           & \multicolumn{1}{c|}{56.8}                                                                                   & \multicolumn{1}{c|}{85.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{86.3}}                                    & \multicolumn{1}{c|}{58.6}                                                                            & \multicolumn{1}{c|}{57.7}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{78.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78}}                       & 77.7                                                                     \\ \hline
2,000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.4}                                                                            & \multicolumn{1}{c|}{57.3}                                                                           & \multicolumn{1}{c|}{55.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.6}}                     & \multicolumn{1}{c|}{88.5}                                                                     & \multicolumn{1}{c|}{58.1}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{55.2}                                                                                   & \multicolumn{1}{c|}{78.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.3}}                                    & \multicolumn{1}{c|}{51.6}                                                                            & \multicolumn{1}{c|}{58.6}                                                                           & \multicolumn{1}{c|}{58.7}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79.3}                                    \\ \hline
%2,000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{44.1}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{59.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                     & \multicolumn{1}{c|}{88.5}                                                                     & \multicolumn{1}{c|}{56.4}                                                                            & \multicolumn{1}{c|}{58.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{77.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{52.8}                                                                            & \multicolumn{1}{c|}{55.8}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{78.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{78.6}                                    \\ \hline
2,000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{47}                                                                              & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                     & \multicolumn{1}{c|}{89.1}                                                                     & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.6}}                                    & \multicolumn{1}{c|}{52.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.7}                                    \\ \hline
%2,000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{44.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{57.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{52.7}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56}                                                                                     & \multicolumn{1}{c|}{80.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
2,000                                                                                        & 12,213                                                                                    & \multicolumn{1}{c|}{45.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.7}}                                    & \multicolumn{1}{c|}{58.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.9}}                                    & \multicolumn{1}{c|}{53.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
%5000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{46.3}                                                                            & \multicolumn{1}{c|}{49.3}                                                                           & \multicolumn{1}{c|}{56.1}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{59.2}                                                                           & \multicolumn{1}{c|}{48.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{72.1}                                                                     & \multicolumn{1}{c|}{51.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{71.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.3}                                    \\ \hline
%5000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{50.4}                                                                            & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{52.1}                                                                                   & \multicolumn{1}{c|}{87.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.6}}                                    & \multicolumn{1}{c|}{53.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{77.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.4}}                                    & \multicolumn{1}{c|}{55.3}                                                                            & \multicolumn{1}{c|}{56.1}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{79.3}                                    \\ \hline
%5000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{45.3}                                                                            & \multicolumn{1}{c|}{62.8}                                                                           & \multicolumn{1}{c|}{54.1}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.9}}                     & \multicolumn{1}{c|}{87.7}                                                                     & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{48.9}                                                                                   & \multicolumn{1}{c|}{79.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                                    & \multicolumn{1}{c|}{54.9}                                                                            & \multicolumn{1}{c|}{58.8}                                                                           & \multicolumn{1}{c|}{48.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.2}                                    \\ \hline
%5000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{51}                                                                              & \multicolumn{1}{c|}{71.1}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.2}}                     & \multicolumn{1}{c|}{87.6}                                                                     & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.5}}                     & \multicolumn{1}{c|}{76.4}                                                                     & \multicolumn{1}{c|}{55.4}                                                                            & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.4}                                    \\ \hline
%5000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{54.6}                                                                            & \multicolumn{1}{c|}{64.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.2}}                     & \multicolumn{1}{c|}{89.5}                                                                     & \multicolumn{1}{c|}{58.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{79.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82}}                                      & \multicolumn{1}{c|}{54.5}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.9}                                    \\ \hline
%5000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{46.5}                                                                            & \multicolumn{1}{c|}{56.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{88.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.7}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.1}}                                    & \multicolumn{1}{c|}{53.5}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.1}                                    \\ \hline
%5000                                                                                        & 12,213                                                                                    & \multicolumn{1}{c|}{50.3}                                                                            & \multicolumn{1}{c|}{61.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{85.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.6}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{53.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8,000                                                                                        & 50                                                                                       & \multicolumn{1}{c|}{48.7}                                                                            & \multicolumn{1}{c|}{52.7}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80}}                       & \multicolumn{1}{c|}{77.3}                                                                     & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56.6}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{72.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{74.4}}                                    & \multicolumn{1}{c|}{51.2}                                                                            & \multicolumn{1}{c|}{54.2}                                                                           & \multicolumn{1}{c|}{51.5}                                                                                   & \multicolumn{1}{c|}{72.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.6}                                    \\ \hline
%8,000                                                                                        & 200                                                                                      & \multicolumn{1}{c|}{48.2}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{86.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{49.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                     & \multicolumn{1}{c|}{78.2}                                                                     & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79}}                       & 78.8                                                                     \\ \hline
8,000                                                                                        & 500                                                                                      & \multicolumn{1}{c|}{56.9}                                                                            & \multicolumn{1}{c|}{52.6}                                                                           & \multicolumn{1}{c|}{55.8}                                                                                   & \multicolumn{1}{c|}{88.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{53.9}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{79.9}}                     & \multicolumn{1}{c|}{79.8}                                                                     & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{57.6}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{82.3}                                    \\ \hline
%8,000                                                                                        & 1000                                                                                     & \multicolumn{1}{c|}{48.6}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{89.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{89.7}}                                    & \multicolumn{1}{c|}{57.2}                                                                            & \multicolumn{1}{c|}{59.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{54.1}                                                                            & \multicolumn{1}{c|}{58.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.4}                                    \\ \hline
8,000                                                                                        & 4,000                                                                                     & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{57.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.3}}                                    & \multicolumn{1}{c|}{54.3}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{83.1}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.2}                                    \\ \hline
%8,000                                                                                        & 10000                                                                                    & \multicolumn{1}{c|}{48.1}                                                                            & \multicolumn{1}{c|}{59.9}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.9}}                                    & \multicolumn{1}{c|}{56.2}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                    & \multicolumn{1}{c|}{51.9}                                                                            & \multicolumn{1}{c|}{56.2}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.4}                                    \\ \hline
8,000                                                                                        & 12,213                                                                                    & \multicolumn{1}{c|}{49.9}                                                                            & \multicolumn{1}{c|}{63.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{88}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91.3}}                                    & \multicolumn{1}{c|}{56.9}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{80.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.5}}                                    & \multicolumn{1}{c|}{53.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.3}                                    \\ \hline
%10000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{51}                                                                              & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{54}                                                                                     & \multicolumn{1}{c|}{74.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.2}}                                    & \multicolumn{1}{c|}{56.3}                                                                            & \multicolumn{1}{c|}{57.6}                                                                           & \multicolumn{1}{c|}{51.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.5}}                     & \multicolumn{1}{c|}{71.8}                                                                     & \multicolumn{1}{c|}{52}                                                                              & \multicolumn{1}{c|}{51.9}                                                                           & \multicolumn{1}{c|}{46.7}                                                                                   & \multicolumn{1}{c|}{71.4}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.3}                                    \\ \hline
%10000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{49}                                                                              & \multicolumn{1}{c|}{54.8}                                                                           & \multicolumn{1}{c|}{53.8}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{60.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{77.6}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{77.9}}                                    & \multicolumn{1}{c|}{52}                                                                              & \multicolumn{1}{c|}{56.5}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{78.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{79}                                      \\ \hline
%10000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{53.7}                                                                                   & \multicolumn{1}{c|}{86.9}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.8}}                                    & \multicolumn{1}{c|}{57}                                                                              & \multicolumn{1}{c|}{53.6}                                                                           & \multicolumn{1}{c|}{50.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81.2}}                     & \multicolumn{1}{c|}{80.8}                                                                     & \multicolumn{1}{c|}{53}                                                                              & \multicolumn{1}{c|}{55.6}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.2}}                     & 81.2                                                                     \\ \hline
%10000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{51.7}                                                                            & \multicolumn{1}{c|}{57}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.8}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                    & \multicolumn{1}{c|}{57.8}                                                                            & \multicolumn{1}{c|}{60}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{80.7}}                     & \multicolumn{1}{c|}{80.5}                                                                     & \multicolumn{1}{c|}{54.4}                                                                            & \multicolumn{1}{c|}{58}                                                                             & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{82.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.1}                                    \\ \hline
%10000                                                                                       & 4,000                                                                                     & \multicolumn{1}{c|}{53.7}                                                                            & \multicolumn{1}{c|}{74.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.9}}                                    & \multicolumn{1}{c|}{57.6}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                     & \multicolumn{1}{c|}{82.3}                                                                     & \multicolumn{1}{c|}{54.8}                                                                            & \multicolumn{1}{c|}{60.5}                                                                           & \multicolumn{1}{c|}{56.2}                                                                                   & \multicolumn{1}{c|}{80.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{83.7}                                    \\ \hline
%10000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{50.6}                                                                            & \multicolumn{1}{c|}{61.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.3}}                                    & \multicolumn{1}{c|}{56.7}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83}}                                      & \multicolumn{1}{c|}{54.2}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.6}                                    \\ \hline
%10000                                                                                       & 12,213                                                                                    & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{57.7}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{92.3}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.8}}                                    & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{56}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16,000                                                                                       & 50                                                                                       & \multicolumn{1}{c|}{51.2}                                                                            & \multicolumn{1}{c|}{55.1}                                                                           & \multicolumn{1}{c|}{51.4}                                                                                   & \multicolumn{1}{c|}{75.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.9}}                                    & \multicolumn{1}{c|}{54.7}                                                                            & \multicolumn{1}{c|}{57.2}                                                                           & \multicolumn{1}{c|}{51.7}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{72.8}}                     & \multicolumn{1}{c|}{71.6}                                                                     & \multicolumn{1}{c|}{52.1}                                                                            & \multicolumn{1}{c|}{54.3}                                                                           & \multicolumn{1}{c|}{46.4}                                                                                   & \multicolumn{1}{c|}{72.3}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{73.9}                                    \\ \hline
%16,000                                                                                       & 200                                                                                      & \multicolumn{1}{c|}{52.2}                                                                            & \multicolumn{1}{c|}{49.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{87}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{87.4}}                                    & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{58.6}                                                                           & \multicolumn{1}{c|}{51.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{78.3}}                     & \multicolumn{1}{c|}{78.2}                                                                     & \multicolumn{1}{c|}{54.6}                                                                            & \multicolumn{1}{c|}{57.9}                                                                           & \multicolumn{1}{c|}{50.6}                                                                                   & \multicolumn{1}{c|}{79}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{79.1}                                    \\ \hline
16,000                                                                                       & 500                                                                                      & \multicolumn{1}{c|}{47.9}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{88.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{88.7}}                                    & \multicolumn{1}{c|}{57.6}                                                                            & \multicolumn{1}{c|}{60.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{81}}                       & \multicolumn{1}{c|}{79.5}                                                                     & \multicolumn{1}{c|}{49.4}                                                                            & \multicolumn{1}{c|}{52.5}                                                                           & \multicolumn{1}{c|}{56.5}                                                                                   & \multicolumn{1}{c|}{81.7}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{81.8}                                    \\ \hline
%16,000                                                                                       & 1000                                                                                     & \multicolumn{1}{c|}{52.9}                                                                            & \multicolumn{1}{c|}{53}                                                                             & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{89.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.1}}                                    & \multicolumn{1}{c|}{56.5}                                                                            & \multicolumn{1}{c|}{61.3}                                                                           & \multicolumn{1}{c|}{56.4}                                                                                   & \multicolumn{1}{c|}{80.2}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{82.7}}                                    & \multicolumn{1}{c|}{53.6}                                                                            & \multicolumn{1}{c|}{58.5}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{82}                                                        & \cellcolor[HTML]{FFFFFF}\textbf{83.6}                                    \\ \hline
16,000                                                                                       & 4,000                                                                                     & \multicolumn{1}{c|}{51.6}                                                                            & \multicolumn{1}{c|}{65.1}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.5}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{58.3}                                                                            & \multicolumn{1}{c|}{59.1}                                                                           & \multicolumn{1}{c|}{56.1}                                                                                   & \multicolumn{1}{c|}{83}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84}}                                      & \multicolumn{1}{c|}{52.4}                                                                            & \multicolumn{1}{c|}{60.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.9}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.7}                                    \\ \hline
%16,000                                                                                       & 10000                                                                                    & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{74.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.3}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{90.5}}                                    & \multicolumn{1}{c|}{57.2}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.7}                                                                                   & \multicolumn{1}{c|}{81.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.7}}                                    & \multicolumn{1}{c|}{54.1}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{84.9}                                    \\ \hline
16,000                                                                                       & 12,213                                                                                    & \multicolumn{1}{c|}{47.3}                                                                            & \multicolumn{1}{c|}{58.4}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{90.4}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{91}}                                      & \multicolumn{1}{c|}{56.8}                                                                            & \multicolumn{1}{c|}{56.3}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.1}                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{83.5}}                                    & \multicolumn{1}{c|}{53.4}                                                                            & \multicolumn{1}{c|}{59.8}                                                                           & \multicolumn{1}{c|}{56.3}                                                                                   & \multicolumn{1}{c|}{82.8}                                                      & \cellcolor[HTML]{FFFFFF}\textbf{85}                                      \\ \hline
\end{tabular}

\end{table*}

==> tables/exp.tex <==

\begin{table}
\centering

\begin{tabular}{| l | c c | c | c c c c | c | c c c c | c | c c c c |}
\hline
 & \multirow{3}{*}{Source Labeled Data Size} & \multirow{3}{*}{TargetLabeledDataSize} & \multicolumn{15}{c}{Target Test Accuracy for Kirby(in \%)} \\
 &  &  & \multicolumn{5}{c}{Sensor 0} & \multicolumn{5}{c}{Sensor 1} & \multicolumn{5}{c}{Sensor 2} \\
0 &  &  & VanillaBase-lineSingleModel & VanillaBase-lineMultiModel & VanillaBase-lineFine-TunedModel & ICIT-ADV-DA & modi-fiedICIT-ADV-DA & VanillaBase-lineSingleModel & VanillaBase-lineMultiModel & VanillaBase-lineFine-TunedModel & ICIT-ADV-DA & modi-fiedICIT-ADV-DA & VanillaBase-lineSingleModel & VanillaBase-lineMultiModel & VanillaBase-lineFine-TunedModel & ICIT-ADV-DA & modi-fiedICIT-ADV-DA \\
0 & 2000 & 50 & 0.495 & 0.537 & 0.503 & \textbf{0.798} & 0.797 & 0.584 & 0.576 & 0.525 & 0.716 & \textbf{0.729} & 0.527 & 0.523 & 0.531 & 0.74 & \textbf{0.741} \\
\hline
1 & 2000 & 200 & 0.454 & 0.573 & 0.568 & 0.855 & \textbf{0.863} & 0.586 & 0.577 & 0.567 & 0.785 & \textbf{0.799} & 0.521 & 0.579 & 0.541 & \textbf{0.78} & 0.777 \\
\hline
2 & 2000 & 500 & 0.454 & 0.573 & 0.557 & \textbf{0.886} & 0.885 & 0.581 & 0.564 & 0.552 & 0.786 & \textbf{0.793} & 0.516 & 0.586 & 0.587 & 0.789 & \textbf{0.793} \\
\hline
3 & 2000 & 1000 & 0.441 & 0.606 & 0.592 & \textbf{0.888} & 0.885 & 0.564 & 0.589 & 0.563 & 0.772 & \textbf{0.799} & 0.528 & 0.558 & 0.564 & 0.784 & \textbf{0.786} \\
\hline
4 & 2000 & 4000 & 0.47 & 0.563 & 0.563 & \textbf{0.892} & 0.891 & 0.567 & 0.563 & 0.563 & 0.806 & \textbf{0.816} & 0.526 & 0.563 & 0.563 & 0.809 & \textbf{0.827} \\
\hline
5 & 2000 & 10000 & 0.445 & 0.563 & 0.563 & 0.9 & \textbf{0.919} & 0.577 & 0.563 & 0.563 & 0.798 & \textbf{0.828} & 0.527 & 0.56 & 0.56 & 0.806 & \textbf{0.843} \\
\hline
6 & 2000 & 16000 & 0.458 & 0.563 & 0.563 & 0.885 & \textbf{0.917} & 0.585 & 0.563 & 0.563 & 0.814 & \textbf{0.829} & 0.532 & 0.563 & 0.563 & 0.813 & \textbf{0.843} \\
\hline
7 & 5000 & 50 & 0.463 & 0.493 & 0.561 & 0.79 & \textbf{0.799} & 0.578 & 0.592 & 0.487 & \textbf{0.725} & 0.721 & 0.511 & 0.563 & 0.517 & 0.711 & \textbf{0.733} \\
\hline
8 & 5000 & 200 & 0.504 & 0.565 & 0.521 & 0.874 & \textbf{0.876} & 0.538 & 0.563 & 0.517 & 0.778 & \textbf{0.794} & 0.553 & 0.561 & 0.514 & 0.79 & \textbf{0.793} \\
\hline
9 & 5000 & 500 & 0.453 & 0.628 & 0.541 & \textbf{0.889} & 0.877 & 0.57 & 0.595 & 0.489 & 0.799 & \textbf{0.807} & 0.549 & 0.588 & 0.483 & 0.806 & \textbf{0.812} \\
\hline
10 & 5000 & 1000 & 0.51 & 0.711 & 0.562 & \textbf{0.892} & 0.876 & 0.554 & 0.595 & 0.562 & \textbf{0.805} & 0.764 & 0.554 & 0.572 & 0.563 & 0.807 & \textbf{0.814} \\
\hline
11 & 5000 & 4000 & 0.546 & 0.643 & 0.563 & \textbf{0.902} & 0.895 & 0.585 & 0.563 & 0.562 & 0.798 & \textbf{0.82} & 0.545 & 0.579 & 0.563 & 0.817 & \textbf{0.829} \\
\hline
12 & 5000 & 10000 & 0.465 & 0.564 & 0.563 & 0.888 & \textbf{0.917} & 0.563 & 0.563 & 0.563 & 0.805 & \textbf{0.841} & 0.535 & 0.563 & 0.563 & 0.808 & \textbf{0.841} \\
\hline
13 & 5000 & 16000 & 0.503 & 0.616 & 0.563 & 0.853 & \textbf{0.916} & 0.563 & 0.563 & 0.563 & 0.816 & \textbf{0.827} & 0.538 & 0.563 & 0.563 & 0.821 & \textbf{0.844} \\
\hline
14 & 8000 & 50 & 0.487 & 0.527 & 0.515 & \textbf{0.8} & 0.773 & 0.562 & 0.566 & 0.538 & 0.728 & \textbf{0.744} & 0.512 & 0.542 & 0.515 & 0.729 & \textbf{0.736} \\
\hline
15 & 8000 & 200 & 0.482 & 0.579 & 0.54 & 0.863 & \textbf{0.874} & 0.57 & 0.572 & 0.493 & \textbf{0.789} & 0.782 & 0.534 & 0.556 & 0.539 & \textbf{0.79} & 0.788 \\
\hline
16 & 8000 & 500 & 0.569 & 0.526 & 0.558 & 0.885 & \textbf{0.888} & 0.578 & 0.579 & 0.539 & \textbf{0.799} & 0.798 & 0.521 & 0.576 & 0.567 & 0.814 & \textbf{0.823} \\
\hline
17 & 8000 & 1000 & 0.486 & 0.598 & 0.562 & 0.893 & \textbf{0.897} & 0.572 & 0.595 & 0.563 & 0.815 & \textbf{0.828} & 0.541 & 0.583 & 0.563 & 0.817 & \textbf{0.834} \\
\hline
18 & 8000 & 4000 & 0.506 & 0.598 & 0.563 & 0.906 & \textbf{0.91} & 0.577 & 0.563 & 0.563 & 0.813 & \textbf{0.833} & 0.543 & 0.563 & 0.563 & 0.831 & \textbf{0.842} \\
\hline
19 & 8000 & 10000 & 0.481 & 0.599 & 0.563 & 0.9 & \textbf{0.919} & 0.562 & 0.56 & 0.563 & 0.807 & \textbf{0.825} & 0.519 & 0.562 & 0.565 & 0.814 & \textbf{0.844} \\
\hline
20 & 8000 & 16000 & 0.499 & 0.633 & 0.565 & 0.88 & \textbf{0.913} & 0.569 & 0.56 & 0.563 & 0.806 & \textbf{0.825} & 0.536 & 0.563 & 0.565 & 0.819 & \textbf{0.843} \\
\hline
21 & 10000 & 50 & 0.51 & 0.572 & 0.54 & 0.746 & \textbf{0.802} & 0.563 & 0.576 & 0.518 & \textbf{0.725} & 0.718 & 0.52 & 0.519 & 0.467 & 0.714 & \textbf{0.733} \\
\hline
22 & 10000 & 200 & 0.49 & 0.548 & 0.538 & \textbf{0.874} & \textbf{0.874} & 0.568 & 0.606 & 0.513 & 0.776 & \textbf{0.779} & 0.52 & 0.565 & 0.563 & 0.789 & \textbf{0.79} \\
\hline
23 & 10000 & 500 & 0.506 & 0.56 & 0.537 & 0.869 & \textbf{0.888} & 0.57 & 0.536 & 0.507 & \textbf{0.812} & 0.808 & 0.53 & 0.556 & 0.563 & \textbf{0.822} & 0.812 \\
\hline
24 & 10000 & 1000 & 0.517 & 0.57 & 0.563 & 0.898 & \textbf{0.905} & 0.578 & 0.6 & 0.562 & \textbf{0.807} & 0.805 & 0.544 & 0.58 & 0.562 & 0.827 & \textbf{0.831} \\
\hline
25 & 10000 & 4000 & 0.537 & 0.741 & 0.563 & 0.895 & \textbf{0.909} & 0.576 & 0.563 & 0.567 & \textbf{0.828} & 0.823 & 0.548 & 0.605 & 0.562 & 0.807 & \textbf{0.837} \\
\hline
26 & 10000 & 10000 & 0.506 & 0.614 & 0.563 & 0.907 & \textbf{0.923} & 0.567 & 0.563 & 0.563 & 0.817 & \textbf{0.83} & 0.542 & 0.56 & 0.563 & 0.817 & \textbf{0.846} \\
\hline
27 & 10000 & 16000 & 0.529 & 0.577 & 0.563 & 0.903 & \textbf{0.923} & 0.568 & 0.563 & 0.563 & 0.822 & \textbf{0.828} & 0.529 & 0.56 & 0.563 & 0.823 & \textbf{0.849} \\
\hline
28 & 16000 & 50 & 0.512 & 0.551 & 0.514 & 0.751 & \textbf{0.789} & 0.547 & 0.572 & 0.517 & \textbf{0.728} & 0.716 & 0.521 & 0.543 & 0.464 & 0.723 & \textbf{0.739} \\
\hline
29 & 16000 & 200 & 0.522 & 0.496 & 0.513 & 0.87 & \textbf{0.874} & 0.568 & 0.586 & 0.513 & \textbf{0.783} & 0.782 & 0.546 & 0.579 & 0.506 & 0.79 & \textbf{0.791} \\
\hline
30 & 16000 & 500 & 0.479 & 0.563 & 0.564 & 0.881 & \textbf{0.887} & 0.576 & 0.601 & 0.563 & \textbf{0.81} & 0.795 & 0.494 & 0.525 & 0.565 & 0.817 & \textbf{0.818} \\
\hline
31 & 16000 & 1000 & 0.529 & 0.53 & 0.563 & 0.894 & \textbf{0.901} & 0.565 & 0.613 & 0.564 & 0.802 & \textbf{0.827} & 0.536 & 0.585 & 0.567 & 0.82 & \textbf{0.836} \\
\hline
32 & 16000 & 4000 & 0.516 & 0.651 & 0.563 & 0.905 & \textbf{0.91} & 0.583 & 0.591 & 0.561 & 0.83 & \textbf{0.84} & 0.524 & 0.603 & 0.563 & 0.829 & \textbf{0.847} \\
\hline
33 & 16000 & 10000 & 0.534 & 0.743 & 0.563 & 0.903 & \textbf{0.905} & 0.572 & 0.563 & 0.567 & 0.814 & \textbf{0.837} & 0.541 & 0.563 & 0.563 & 0.828 & \textbf{0.849} \\
\hline
34 & 16000 & 16000 & 0.473 & 0.584 & 0.563 & 0.904 & \textbf{0.91} & 0.568 & 0.563 & 0.563 & 0.821 & \textbf{0.835} & 0.534 & 0.598 & 0.563 & 0.828 & \textbf{0.85} \\
\hline

\end{tabular}

\end{table}

\begin{table}
    \centering
    \begin{tabular}{cccccccccc}
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
         &  &  &  &  &  &  &  &  & \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
